Fun with Flags: Robust Principal Directions via Flag Manifolds

Principal component analysis (PCA), along with its extensions to manifolds and outlier contaminated data, have been indispensable in computer vision and machine learning. In this work, we present a unifying formalism for PCA and its variants, and introduce a framework based on the flags of linear subspaces, ie a hierarchy of nested linear subspaces of increasing dimension, which not only allows for a common implementation but also yields novel variants, not explored previously. We begin by generalizing traditional PCA methods that either maximize variance or minimize reconstruction error. We expand these interpretations to develop a wide array of new dimensionality reduction algorithms by accounting for outliers and the data manifold. To devise a common computational approach, we recast robust and dual forms of PCA as optimization problems on flag manifolds. We then integrate tangent space approximations of principal geodesic analysis (tangent-PCA) into this flag-based framework, creating novel robust and dual geodesic PCA variations. The remarkable flexibility offered by the 'flagification' introduced here enables even more algorithmic variants identified by specific flag types. Last but not least, we propose an effective convergent solver for these flag-formulations employing the Stiefel manifold. Our empirical results on both real-world and synthetic scenarios, demonstrate the superiority of our novel algorithms, especially in terms of robustness to outliers on manifolds.

==> content/old_versions/background_old.tex <==
\vspace{-1mm}\section{Preliminaries}\vspace{-1mm}\label{sec:bg}
%Before delving into the specifics of our contributions, we 
Let us start by briefly introducing Riemannian geometry, flag manifolds, and methods for finding principal directions.
%\subsection{Riemannian geometry \& Flag manifolds}
\begin{dfn}[Riemannian manifold~\cite{lee2006riemannian}]
A \emph{Riemannian manifold} $\Man$ is a smooth manifold with a positive definite inner product $\langle \cdot, \cdot \rangle: \TxM \times \TxM \to \R$ defined on the tangent space $\TxM$ at $\x \in \Man$.
\end{dfn}
\begin{dfn}[Geodesics \& Exp/Log-maps]
A \emph{geodesic} $\gamma : \R \to \Man$ parameterizes a path from $\gamma(0) = \x$ to $\gamma(1) = \y$. 
The \emph{exponential map} $\Exp_{\x}(\bv) : \TxM \to \Man$ maps a vector $\bv \in \TxM$ to the manifold in a length preserving fashion such that $\dot\gamma_{\bv}(0)=\bv$ and $\Exp_{\x}(\bv)=\y$. 
Its inverse, the \emph{logarithmic map} is $\Log_{\x}(\y) : \Man \to \TxM$ for $\x,\y \in \Man$ and computes the tangent direction from $\x$ to $\y$. Hence,  $\gamma(t) = \Exp_{\x}\left({\tau\Log_{\x}(\y)}\right)$ for $\tau \in \R$ is the geodesic curve. $\SubMan \in \Man$ is said to be a geodesic submanifold at $\x \in \Man$ if all geodesics through $\x$ in $\SubMan$ are geodesics in $\Man$. %Note that, . \tolga{say sth about matrix manifolds.}
\end{dfn}
% and computes the direction from $x$ to $y$\footnote{The logarithm map may not be defined everywhere on $M$.}.
% on the tangent space. This inner product defines a Riemannian metric on $M$ and is denoted  where $\x \in M$ and $\TxM$ is the tangent space to $M$ at $x$. Let $\bv \in \TxM$ be a tangent vector to $M$ at $x$. 
%  The \emph{logarithm map} is $\text{log}_x(y) : M \to \TxM$ for $x,y \in M$ and computes the direction from $x$ to $y$\footnote{The logarithm map may not be defined everywhere on $M$.}. 
%A \emph{geodesic} $\gamma : \R \to M$ parameterizes a path from $\gamma(0) = x$ to $\gamma(1) = y$. The geodesic can be written as $\gamma = \exp_x^{t\log_x(y)}$ for $t \in \R$. $H \in M$ is a geodesic submanifold at $x \in M$ if all geodesics passing through $x$ in $H$ are geodesics in $M$.

\begin{dfn}[Flag]\label{def:flagobj}
% \textcolor{blue}{Nate: Reword this}
A \emph{flag} is an nested sequence of subspaces of a finite dimensional vector space $\mathcal{V}$ of \emph{increasing} dimension, is the filtration $\{\emptyset \}=\mathcal{V}_0 \subset \mathcal{V}_1 \subset \ldots \subset \mathcal{V}_{k} \subset \mathcal{V}$ with $0=n_0<n_1<\ldots<n_k<n$ where $\mathrm{dim} \mathcal{V}_i=n_i$ and $\mathrm{dim} \mathcal{V}=n$.  The \emph{type} or \emph{signature} of this flag is $(n_1, \ldots ,n_k;n)$ or $(n_1, \ldots ,n_k)$.

% A \emph{flag} in a finite dimensional vector space $\mathcal{V}$ over a field is a sequence of nested subspaces with \emph{increasing} dimension, each containing its predecessor, \ie the filtration: $\{\emptyset \}=\mathcal{V}_0 \subset \mathcal{V}_1 \subset \ldots \subset \mathcal{V}_{k} \subset \mathcal{V}$ with $0=n_0<n_1<\ldots<n_k<n$ where $\mathrm{dim} \mathcal{V}_i=n_i$ and $\mathrm{dim} \mathcal{V}=n$. 
% We say this flag is of \emph{type} or \emph{signature} $(n_1, \ldots ,n_k;n)$. 
%A flag is called \emph{complete} if $d_i = i,\,\forall i$. Otherwise the flag is \emph{incomplete} or \emph{partial}. 

\noindent\textbf{\emph{Notation}:} We denote a flag using a point $\X$ on the Stiefel manifold~\cite{edelman1998geometry} $St(n_k, n) = \{\X \in \R^{n \times n_k} : \X^T \X = \I \}$. Given $\X \in St(n_k, n)$ and $\x_i$, $i^{\text{th}}$ column of $\X$, we define 
\begin{equation}\label{eq: Xi def}
\X_{i+1} = \begin{bmatrix} \x_{n_{i}+1} & \x_{n_{i}+2} & \cdots &  \x_{n_{i+1}} \end{bmatrix}  \in \R^{n \times m_{i+1}}.
\end{equation}
where $m_i = n_i-n_{i-1}$ for $i=1,2,\ldots, k$. $[\X_1, \ldots, \X_i]$ denotes the span of the columns of $\{ \X_1, \ldots, \X_i\}$. Then
\begin{equation}
     [ \X_1 ]  \subset [\X_1, \X_2] \subset \cdots \subset  [\X_1, \ldots, \X_k] = [\X] \subset \R^n. \nonumber
\end{equation}
is a flag of type $(n_1, \ldots , n_k;n)$ and is denoted $[\![\X]\!]$.


% A flag, $[\![\X]\!]$ of type $(n_1, \ldots , n_k; n)$, is represented by a truncated orthogonal matrix $\X \in \R^{n \times n_k}$. Let $m_i = n_i-n_{i-1}$ for $j=1,2,\ldots, k$, and 
% \begin{equation}\label{eq: Xi def}
% \X_i = [\x_{n_{i-1}+1},\x_{n_{i-1}+2}, \ldots, \x_{n_i}]  \in \R^{n \times m_i}
% \end{equation}
% for $i=1,2,\ldots, k$.
% %whose columns are the $n_{j-1}+1$ to $n_{j}$ columns of $\X$. 
% Let $[\X] := \text{col}(\X)$, then $[\![\X]\!]$ is
% \begin{equation}
%      [ \X_1 ]  \subset [\X_1, \X_2] \subset \cdots \subset  [\X_1, \ldots, \X_k] = [\X] \subset \R^n. \nonumber
% \end{equation}
\end{dfn}

\begin{dfn}[Flag manifold]
% \textcolor{blue}{Nate: Reword this}
The set of all flags of type $(n_1, \ldots, n_k; n)$ is called the flag manifold due to its manifold structure. We refer to this \emph{flag manifold} as $\flag(n_1, \ldots, n_k; n)$ or $\flag(n+1)$. Flags generalize Grassmann and Stiefel manifolds~\cite{edelman1998geometry} because $\flag(n_k; n)= Gr(n_k,n)$ and $\flag(1,\dots,n_k; n)=St(n_k,n)$. 
We denote flags in $\flag(n+1)$ using the fact from~\cite{ye2022optimization}:
\begin{equation*}
\flag(n+1) = St(n_k, n)/O(m_1) \times O(m_2) \times \cdots \times O(m_{k+1}).
\end{equation*}
\end{dfn}
\noindent Ye~\etal~\cite{ye2022optimization} equip $\flag(n+1)$ offer closed-form analytic expressions for some Riemannian operators needed for optimization by using extrinsic matrix coordinates.


% The aggregate of all flags of the same type, \ie a certain collection of ordered sets of vector subspaces, admits the structure of manifolds. We refer to this \emph{flag manifold} %with its dimension (type) 
% as $\flag(n_1, \ldots, n_k; n)$ or equivalently as $\flag(n+1)$. The points of $\flag(n+1)$
% %$\flag(d_1, \ldots, d_k; d)$ 
% parameterize all flags of type $(n_1, \ldots, n_k;n)$. 
% Flag manifolds generalize Grassmannians~\cite{edelman1998geometry} because $\flag(k; n)=\Gr(k,n)$. $\flag(n+1)$ can be thought of as a quotient of groups ~\cite{ye2022optimization}:
% \begin{equation*}
% \flag(n+1) = St(d_k, n)/O(m_1) \times O(m_2) \times \cdots \times O(m_{k+1}),
% \end{equation*}
% where
% $St(n_k, n) = \{\X \in \R^{n \times n_k} : \X^T \X = \I \} $ denotes the Stiefel manifold of $n_k$-frames.
% \end{dfn}
% \noindent Ye~\etal~\cite{ye2022optimization} equip $\flag(\cdot)$ with extrinsic matrix coordinates that, in turn, give closed-form analytic expressions for various Riemannian operators required for optimization.



==> content/old_versions/backup-pca.tex <==
\subsection{PCA and its robust variants}
Given a set of $k < n$ orthonormal vectors $\{\bu_i\}_{j=1}^k \subset \R^n$, define the matrix $\U = [\bu_1,\dots,\bu_k]$. The projection of $\x$ onto the subspace spanned by this basis (namely $S_\U$) is $\pi_{S_\U}(\x) := \U \U^T \x$.

Suppose we have $p$ samples (points) with $n$ random variables (features) $\mathcal{X} = \{ \x_i \}_{i=1}^p \subset \R^n$ with a sample mean of $0$. The directions found by PCA either maximize variance (\cref{eq: minpca}) or minimize reconstruction error (\cref{eq: minpca}).


\begin{dfn}[PCA~\cite{hotelling1933analysis}]
The $i$th principal direction is
\begin{equation}\label{eq: maxpca}
\mathbf{u}_{i} = \argmax_{\substack{\mathbf{u}^T \mathbf{u} = 1 \\ \mathbf{u} \in S_i^\perp }} \mathbb{E} \left[\|  \pi_{S_{\mathbf{u}}} (\x_j) \|_2^2 \right]
\end{equation}
\begin{equation}\label{eq: minpca}
\mathbf{u}_{i} = \argmin_{\substack{\mathbf{u}^T \mathbf{u} = 1 \\ \mathbf{u} \in S_{i-1}^\perp}} \mathbb{E} \left[\|  \bm{\x_j} - \pi_{S_{\mathbf{u}}} (\x_j) \|_2^2 \right]
\end{equation}
\end{dfn}
In general, PCA gives us a $k<n$ dimensional embedding of the data as the columns of $\U^T\X \in \R^{k \times p}$. We can approximately invert PCA by left multiplication by $\U$.

General formulations of the PCA optimization problem are~\cref{eq: maxpca_gen,eq: mindpca_gen}:
\begin{equation}\label{eq: maxpca_gen}
\argmax_{\mathbf{U}^T \mathbf{U} = \I} \mathbb{E} \left[\|  \pi_{S_{\mathbf{U}}} (\x_j) \|_p^q \right],
\end{equation}
\begin{equation}\label{eq: minpca_gen}
\argmin_{\mathbf{U}^T \mathbf{U} = \I } \mathbb{E} \left[\|  \bm{\x_j} - \pi_{S_{\mathbf{U}}} (\x_j) \|_p^q \right].
\end{equation}
Both problems recover PCA when $p=q=2$. 

If we instead formulate the general ``dual'' problems~\cref{eq: maxopca_gen,eq: minopca_gen}, we will recover the orthogonal compliment of the PCA directions found in~\cref{eq: maxpca_gen,eq: mindpca_gen}. We will refer to these formulations as versions of $\perp$PCA.
\begin{equation}\label{eq: maxopca_gen}
\argmax_{\mathbf{B}^T \mathbf{B} = \I} \mathbb{E} \left[\|  \pi_{S_{\mathbf{B}}} (\x_j) \|_p^q \right],
\end{equation}
\begin{equation}\label{eq: minopca_gen}
\argmin_{\mathbf{B}^T \mathbf{B} = \I } \mathbb{E} \left[\|  \bm{\x_j} - \pi_{S_{\mathbf{B}}} (\x_j) \|_p^q \right].
\end{equation}
Suppose we find the first $k$ principal directions using either of~\cref{eq: maxpca_gen,eq: mindpca_gen} and store them in $\U$. Then we find the first $n-k$ $\perp$ principal directions using either of~\cref{eq: maxopca_gen,eq: minopca_gen} and store them in $\B$. We can be sure that $[\U, \B] \in O(n)$. That is to say that $\B = \U^{\perp}$.

\paragraph{Robust PCA Formulations} Outliers of a dataset are generally considered data that significantly deviate from the general pattern of the dataset. Points in the dataset that are not outliers will be called inliers. If we have a dataset with many outlier points, the directions of maximum variance (detected by PCA) may represent these outliers than the actual dataset. Therefore, we seek methods for dimensionality reduction that capture a space containing only the dataset's inliers. 

There are two variants of Robust PCA in the literature: Robust PCA-L1 (RPCA-L1)~\cite{markopoulos2014optimal} solves~\cref{eq: maxpca_gen} for $p=q=1$ and Robust Weiszfeld PCA-L1 (WPCA-L1)~\cite{neumayer2020robust} solves~\cref{eq: minpca_gen} for $p=q=1$. We also propose two new formulations RPCA-L2 and WPCA-L2 which solve ~\cref{eq: maxpca_gen} and ~\cref{eq: minpca_gen} for $p=2,q=1$ respectively.



\paragraph{Dual PCA (DPCA)}
Our model for data with inliers and outliers is the data matrix with $p$ samples of $n$ features: $\X =  [\textbf{A}, \mathbf{B}] \mathbf{P}   \in \R^{n \times p}$. The columns of $\textbf{A}$ and $\mathbf{B}$ are inliers and outliers, respectively. We assume there are more inliers than outliers. $\mathbf{P}$ is a permutation matrix. We assume the samples live on the unit sphere, namely, $\{\x_1, \x_2,\dots, \x_p\} \in \mathbb{S}^{n-1}$. DPCA seeks a subspace $S_\ast = \text{span}\{ \vb_1,  \vb_2, \dots,  \vb_k\}$ so that $S_\ast^\perp$ contains the most inliers (e.g., columns of $\A$). So, we seek vectors, namely $\{\vb_1,  \vb_2, \dots,  \vb_k\}$, that are as orthogonal as possible to the span of the inliers. Classically, DPCA is a $0$-norm problem, but it is relaxed to a $1$-norm problem whose solution is called DPCP~\cite{vidal2018dpcp}. We will refer to this $1$-norm solution as DPCP-L1. One relaxed version of DPCP-L1 is called DPCP-L2 (refered to as DPCP-IRLS by~\cite{vidal2018dpcp}. In general, we can think of these optimization problems as~\cref{eq: mindpca_gen,eq: maxdpca_gen}:
\begin{equation}\label{eq: mindpca_gen}
\argmin_{\mathbf{B}^T \mathbf{B} = \I} \mathbb{E} \left[\|  \pi_{S_{\mathbf{B}}} (\x_j) \|_p^q \right],
\end{equation}
\begin{equation}\label{eq: maxdpca_gen}
\argmax_{\mathbf{B}^T \mathbf{B} = \I } \mathbb{E} \left[\|  \bm{\x_j} - \pi_{S_{\mathbf{B}}} (\x_j) \|_p^q \right].
\end{equation}
Using~\cref{eq: mindpca_gen}, we recover DPCP-L1 with $p=q=1$ and DPCP-L2 with $p=2,q=1$. Two new methods for Dual PCA are the Weiszfeld DPCPs (WDPCPs) which optimize ~\cref{eq: mindpca_gen}. They are called WDPCP-L1 with $p=q=1$ and WDPCP-L2 with $p=2,q=1$.


%%%%%% PGA


\subsection{PGA and its robust variants}

Let $\{x_i\}_{i=1}^p$ be a dataset on a Riemannian manifold $M$.\footnote{$M = \R^n$: $\langle \x, \y \rangle = \x^T\y$, $\text{exp}_x(v) = v-x$, and $\text{log}_x(y) = y-x$}

Given a distance $d(\cdot, \cdot)$ on $M$, an average $\mu$ on $M$ is
\begin{equation}\label{eq: manifold_mean}
    \mu = \argmin_{y \in M} \sum_{i=1}^p d(x_i, y)^q.
\end{equation}
When $d(\cdot, \cdot)$ is the geodesic distance and $q=2$, the Karcher mean~\cite{karcher1977riemannian} is the local minimizer of~\ref{eq: manifold_mean} and if there is a global minimizer of~\ref{eq: manifold_mean} we call it the Fr\'echet mean.

Define the $i$th subspace of $T_{\mu}(M)$ as
\begin{equation}
    S_i = \text{span}\{ \bu_1, \bu_2, \dots, \bu_i \}
\end{equation}
and $S_\bu = \text{span}\{ \bu\}$. The projection operator onto the geodesic subspace $\SubMan \in \Man$ is \footnote{$\pi_{H}$ can be any monotonically increasing function of distance.}
\begin{equation}\label{eq:projdef}
\pi_H(x) = \argmin_{z \in H } d(z, x).
\end{equation}
The geodesic subspace of $S \subset T_\mu(M)$ is
\begin{equation}
   H(S) = \{ \text{exp}_{\mu}(\bv) : \bv \in S\}.
\end{equation}
\textit{Note: In contrast to PCA, in PGA, we need to define $H(S)$ because the tangent space and manifold are distinct.}

\begin{dfn}[PGA~\cite{sommer2010manifold}]
The $i$th principal geodesic direction for (exact) PGA is defined as the geodesic starting at the mean with the tangent vector
\begin{equation}\label{eq:pga_max}
\bu_{i} = \argmax_{\substack{ \| \bu \| = 1 \\ \bu \in S_{i-1}^\perp}} \mathbb{E} \left[ d( \mu, \pi_{H(S_\bu)} (x_j))^q \right]
\end{equation}
for $q=2$.
\end{dfn}

As an alternative to maximizing variance~\cref{eq:pga_max}, we can formulate PGA as a minimizer of reconstruction errors (or unexplained variance) as 
\begin{equation}\label{eq:pga_min} 
\bu_{i} = \argmin_{\substack{ \| \bu \| = 1 \\ \bu \in S_{i-1}^\perp}} \mathbb{E} \left[ d( x_j, \pi_{H(S_\bu)} (x_j))^q \right]
\end{equation}
for $q=2$. In Euclidean space, maximizing variances is equivalent to minimizing residuals, but~\cref{eq:pga_max} and~\cref{eq:pga_min} are not equivalent on Riemannian manifolds~\cite{sommer2010manifold}. Notice that PGA results a flag of subspaces of the tangent space of signature $(1,2,\dots,k, \text{dim}(T_{\mu}(M))$:
\begin{equation}
    S_1 \subset S_2 \subset \cdots \subset S_k \subset T_{\mu}(M).
\end{equation}

Again, we can formulate weighted versions of these algorithms with weights $\{w_j\}_{j=1}^p \in \R$. For example, weighted PGA solves
\begin{equation}\label{eq:wt_pga_max}
\bu_{i} = \argmax_{\substack{ \| \bu \| = 1 \\ \bu \in S_{i-1}^\perp}} \mathbb{E} \left[ w_j d( \mu, \pi_{H(S_\bu)} (x_j))^q \right]
\end{equation}
% Using the minimize distortion definition~\cref{eq:pga_min} and inspiration from Tabaghi~\etal~\cite{tabaghi2023principal}, we say PGA finds a geodesic submanifold of $M$ at $\mu$
% \begin{equation}
%     H_\ast = \argmax_{H \subset M} \mathbb{E} \left[ d( \mu, \pi_{H} (x_j))^2 \right].
% \end{equation}
% Similarly, the maximizing variance definition~\cref{eq:pga_max} results in
% \begin{equation}
%     H_\ast = \argmin_{H \subset M} \mathbb{E} \left[ d( x_j, \pi_{H} (x_j))^2 \right].
% \end{equation}

Let $\w_j = \text{log}_{\mu} x_j$ for $j=1,2,\dots, p$. Fletcher~\etal~\cite{fletcher2004principal} define the $i$th principal geodesic direction from tangent-PGA as the $i$th principal component of $\{\w_j \}_{j=1}^p$. Tangent-PCA is a somewhat reversable transformation. Given $\U = [\bu_{1},\bu_{2}, \dots , \bu_{k}]$ and $\W = [\w_1, \w_2, \dots, \w_p]$, we find the principal components in the tangent space as $ \hat{\W}= \U^T \W $. Then, we approximate the inverse transform as $\U \hat{\W}$ and take $\text{exp}_{\mu}$ to map the columns of this matrix back to the manifold.



\paragraph{Robust PGA (RPGA)}
Novel Riemannian manifold versions of the RPCA variants RPCA and WPCA are \cref{eq:pga_max} and \cref{eq:pga_min} with $q=1$ and called RPGA and WPGA respectively. Given a manifold valued dataset, we approximate these problems by preforming RPCA and WPCA in the tangent space to the Karcher mean. We will refer to these tangent space algorithms as tangent RPCA (tRPCA) and tangent WPCA (tWPCA).

\paragraph{Dual PGA (DPGA)}
Given a Riemannian manifold valued dataset, let us compute the Karcher mean, then move the data such that it is all a unit distance from the Karcher mean. Denote such a normalized dataset as $\{x_i\}_{i=1}^p \subset M$, Then the Riemannian manifold versions of the DPCA variants DPCP and WDPCP are minimizing are~\cref{eq:dpga_min} and \cref{eq:dpga_max} respectively.
\begin{equation}\label{eq:dpga_min}
\bu_{i} = \argmin_{\substack{ \| \bu \| = 1 \\ \bu \in S_{i-1}^\perp}} \mathbb{E} \left[ d( \mu, \pi_{H(S_\bu)} (x_j)) \right]
\end{equation}
\begin{equation}\label{eq:dpga_max} 
\bu_{i} = \argmax_{\substack{ \| \bu \| = 1 \\ \bu \in S_{i-1}^\perp}} \mathbb{E} \left[ d( x_j, \pi_{H(S_\bu)} (x_j)) \right]
\end{equation}
We call~\cref{eq:dpga_min} DPGP and \cref{eq:dpga_max} WDPGP. Again, we can approximate these problems by preforming DPCP and WDPCP in the tangent space. We refer to these tangent space algorithms as  tangent DPCP (tDPCP) and tangent WDPCP (tWDPCP).




==> content/old_versions/conclusion_old.tex <==
\section{Conclusion}
Having fun-with-flags, we have presented a unifying flag-manifold-based framework for computing robust principal directions of Euclidean and non-Euclidean data. Covering PCA, Dual-PCA and their tangent versions in the same framework has given us a generalization power to develop novel, manifold-aware outlier detection and dimensionality reduction algorithms, either by modifying flag-type or by altering norms. We further devised practical algorithms on Stiefel manifolds to efficiently compute these robust directions without requiring direct optimization on the flag manifold. 
Our experimental evaluations revealed that new variants of robust and dual \PCA/tangent \PCA~discovered in our framework can be useful in a variety of applications.

% szwagier2023rethinking,nguyen2022closed
\paragraph{Limitations \& future Work}
% Our algorithm is dependent upon the accuracy and speed of the Riemannian retractions on flag manifolds. 
%Coming up with better \& faster retractions is an ongoing research~\cite{szwagier2023rethinking,nguyen2022closed}.
We cannot handle \emph{non-linear flags}~\cite{haller2023weighted} and hence cannot cover nested spheres/hyperbolic spaces~\cite{dryden2019principal,jung2012analysis,fan2022nested}.
We have also not included Barycentric subspaces~\etal~\cite{pennec2018barycentric}. We leave these for a future study.
% In the future, we will also investigate the approximate invertability of flagified algorithms.
\begin{comment}
Barycentric subspaces~\etal~\cite{pennec2018barycentric}, which we have not covered in this work, solve this problem and can be potentially used to generate more robust versions of Dual-PGA. 
Finally, treating nested-manifolds such as nested spheres~\cite{dryden2019principal,jung2012analysis} or hyperbolic spaces~\cite{fan2022nested} in our framework requires working with \emph{non-linear flags}~\cite{haller2023weighted,nonline}
In the future, we will also investigate the approximate invertibility of flagified algorithms.

We still have problems with the cut locus of the mean on a Riemannian manifold for defining geodesic submanifolds for each of these manifold dimensionality reduction algorithms. Barycentric subspaces, by Pennec~\etal~\cite{pennec2018barycentric}, solve this problem and can be potentially used to generate more robust Riemannian manifold versions of algorithms like DPCP-IRLS.

In the future, 
A nonlinear flag is a finite sequence of nested closed submanifold

Partial least squares has been realized as an algorithm on Riemannian manifolds~\cite{ryan2023riemannian}. Many other dimensionality reduction algorithms can also be realized as Riemannian manifolds. Specifically, future work could port the numerous algorithms for solving DPCP in Euclidean space to the Riemannian manifold setting.

Mention principal nested manifolds and non-linear flags as sequences of nested manifolds.

Mention applications to earth system sciences.

There might be a way to do the known robust PCA and DPCP algorithms with a weiszfeld-type step. We could alternate between the tangent space and the manifold and do weighted centroid and weighted tangent space PCA as nested loops or in the same iteration.



Having invertible transforms is key to understanding what the transform is doing, quantifying uncertainties and distortions of the mapping. Employing invertible nonlinear feature transformations offers advantages such as interpretability, feature engineering, regularization, reversibility, data augmentation, and lossless compression. Other cool applications of invertible transformations are in privacy preservation, representation learning, or solving inverse problems, since they ensuring stability, and facilitate transfer learning. Invertibility allows for data recovery, probably more efficient optimization algorithms, and numerical stability. Therefore we are interested in investigating approximate invertability of algorithms like Flagified PCA, PGA, and Flagified PGA. In fact, it would be interested to investigate the invertibility of most of the published dimensionality reduction algorithms on Riemannian manifolds.

\paragraph{Summary}

\begin{itemize}
    \item \TDPCP:  is good for manifold outlier classification
    \item \TRPCA, \TWPCA: are good for reconstruction in the presence of outliers
    \item \TWPCA does better with very out of distribution outliers whereas \TRPCA does better when the outliers are closer to being in-distribution
\end{itemize}


% fRPCA(1,2,...,k) = L_1-RPCA 
% fWPCA(1,2,...,k) = L_1-WPCA 
% fDPCP(1,2,...,k) = L_1-DPCP 


\end{comment}

==> content/old_versions/intro_old.tex <==
%\vspace{-4mm}
\section{Introduction}\label{sec:intro}

Dimensionality reduction is at the heart of machine learning, statistics and computer vision. Principal Component Analysis (PCA)~\cite{pearson1901liii,hotelling1933analysis} is a well-known technique for reducing the dimensionality of a dataset by linearly transforming the data into a new coordinate system where (most of) the variation in the data can be described with fewer dimensions than the initial data.
Thanks to its simplicity, effectiveness and versatility, PCA has quickly been extended to nonlinear transforms~\cite{scholkopf1997kernel,awate2014kernel,neumayer2020robust}, Riemannian manifolds~\cite{laparra2012nonlinearities,pennec2020advances,fletcher2004principal} or to unknown number of subspaces~\cite{vidal2005generalized}. These have proven indispensable for extracting meaningful information from complex datasets. 

In this paper, we present a unifying framework marrying a large family of PCA variants such as robust PCA~\cite{markopoulos2014optimal,polyak2017robust,kwak2013principal}, dual PCA~\cite{vidal2018dpcp}, PGA~\cite{sommer2010manifold} or tangent PCA~\cite{fletcher2004principal} specified by the norms and powers in a common objective function. Being able to accommodate all these different versions into the same framework allows us to innovate novel ones, for example, \emph{tangent dual PCA}, which poses a strong method for outlier filtering on manifolds. We further enrich the repertoire of available techniques by representing the space of eigenvectors as `flags'~\cite{alekseevsky1997flag}, a hierarchy of nested linear subspaces, in a vein similar to~\cite{pennec2018barycentric}. This `flagification' paves the way to a common computational basis, and we show how all these formulations can be efficiently implemented via a single algorithm which performs Riemannian optimization on Stiefel manifolds~\cite{boumal2023intromanifolds}.
This algorithm additionally contributes to the landscape of optimization techniques for dimensionality reduction, and we prove its convergence for the particular case of dual PCA.

\noindent In summary, \textbf{our contributions are}:
\begin{itemize}[itemsep=0.1pt,leftmargin=*,topsep=1pt]
    \item Generalization of PCA, PGA, and their robust versions leading to new novel variants of these principal directions
    \item A unifying flag manifold-based framework for computing principal directions of Euclidean and non-Euclidean data yielding novel (tangent) PCA formulations between $L_1$ and $L_2$ robust and dual principal directions controlled by flag types
    \item Novel weighting schemes, not only weighting the directions but also the subspaces composed of these directions.
    \item A practical way to optimize objectives on flags by mapping the problems into Stiefel-optimization, which removes the need to convey optimization on flag manifolds, an issue remaining open to date~\cite{ye2022optimization,szwagier2023rethinking}
\end{itemize}
Our theoretical exposition translates to excellent and remarkable findings, validating the usefulness of our novel toolkit in several application examples, from outlier prediction to shape analysis. 
The implementation can be found at \url{https://github.com/nmank/FunWithFlags}.
%will be made available upon publication.
%\tolga{A teaser might come, I'm leaving space for this.}
%
%In conclusion, our proposed flag-based framework represents a paradigm shift in PCA, overcoming the limitations of traditional methods and offering a versatile toolkit for tackling outliers and non-linear structures. The presented algorithms, empowered by the 'flagification' concept, provide a robust and flexible approach to dimensionality reduction, contributing significantly to the advancement of computer vision methodologies.

\iffalse
\tolga{not written yet.}

% Code for this project can be found at this \href{https://github.com/nmank/FlagDimensionalityReduction}{git repo}.

Subspace analysis is an indispensable component of machine learning as various forms of data and parameter sets admit a compact representation as a subspace of a high-dimensional vector space.


Principal component analysis~\cite{pearson1901liii,hotelling1933analysis}.

The modern formalism of PCA goes back to the work of Hotelling~\cite{hotelling1933analysis}.

Given a set of multivariate data points, principal component analysis (PCA) finds new orthogonal basis vectors so that different individual components of the data in the new coordinate system become uncorrelated and the leading basis vectors carry the largest projected variance of the data — compared to any other orthogonal coordinate system.

PCA is a statistical technique for reducing the dimensionality of a datase by linearly transforming the data into a new coordinate system where (most of) the variation in the data can be described with fewer dimensions than the initial data.

In dimensionality reduction, time series analysis, pattern recognition, clustering, exploratory data analysis, image and motion analysis, interpretation, and visualization [21].
\fi



==> content/old_versions/method_least_old.tex <==

\begin{table}[t]
    \centering
    \begin{tabular}{@{\:}c@{\:}|@{\:}c@{\:}|@{\:}c@{\:}||@{\:}c@{\:}c@{\:}c@{\:}}
        & & $(p,q)$ & Variance & Rec. Err. & $\flag(\cdot;n)$\\
        \toprule
        \multirow{6}{*}{\rotatebox[origin=c]{90}{Euclidean}} & \multirow{3}{*}{\rotatebox[origin=c]{90}{Primal}} & $(2,2)$ & \PCA~\cite{hotelling1933analysis} & \PCA~\cite{hotelling1933analysis} & $(1,2,...,k)$\\
        & & $(2,1)$ &  \LtwoRPCA ~\cite{polyak2017robust} & \LtwoWPCA~\cite{ding2006r} & $(k)$\\
        & & $(1,1)$ & \LoneRPCA~\cite{markopoulos2014optimal} & \LoneWPCA~\cite{neumayer2020robust} & $(1,2,...,k)$\\
        \cmidrule{2-6}
        & \multirow{3}{*}{\rotatebox[origin=c]{90}{Dual}} & $(2,2)$ & \OPCA~\cite{vidal2018dpcp} & \OPCA~\cite{vidal2018dpcp} & $(1,2,...,k)$\\
        & & $(2,1)$ &  \LtwoDPCP~\cite{vidal2018dpcp} & \textcolor{blue}{\LtwoWDPCP} & $(k)$\\
        & & $(1,1)$ & \LoneDPCP~\cite{vidal2018dpcp} & \textcolor{blue}{\LoneWDPCP} & $(1,2,...,k)$\\
        \midrule
        \multirow{6}{*}{\rotatebox[origin=c]{90}{Manifold}} & \multirow{3}{*}{\rotatebox[origin=c]{90}{Primal}} & $(2,2)$ & \TPCA~\cite{fletcher2004principal} & \TPCA~\cite{fletcher2004principal} & $(1,2,...,k)$\\
        & & $(2,1)$ &  \textcolor{blue}{\LtwoTRPCA} & \textcolor{blue}{\LtwoTWPCA} & $(k)$\\
        & & $(1,1)$ & \textcolor{blue}{\LoneTRPCA} & \textcolor{blue}{\LoneTWPCA} & $(1,2,...,k)$\\
        \cmidrule{2-6}
        & \multirow{3}{*}{\rotatebox[origin=c]{90}{Dual}} & $(2,2)$ & \textcolor{blue}{\OTPCA} & \textcolor{blue}{\OTPCA} & $(1,2,...,k)$\\
        & & $(2,1)$ &  \textcolor{blue}{\LtwoTDPCP} & \textcolor{blue}{\LtwoTWDPCP} & $(k)$\\
        & & $(1,1)$ & \textcolor{blue}{\LoneTDPCP} & \textcolor{blue}{\LoneTWDPCP} & $(1,2,...,k)$\\
        \bottomrule
    \end{tabular}
    \caption{A summary of variants of \PCA, robust \PCA~and tangent \PCA. The new \PCA~variants introduced in this paper are highlighted in \textcolor{blue}{blue}. For robust variants of \PCA: optimizing over $\flag(1,2,\dots,k;n) = St(k,n)$ recovers $L_1$ and optimizing over $\flag(k;n) = Gr(k,n)$ recovers $L_2$ formulations. Optimizing for any other flag type will provide a collection of novel algorithms between $L_1$ and $L_2$ versions.}
    \label{tab:pca_summary}
\end{table}

%\newpage
%\vspace{-1mm}
\section{Flagifying PCA and Its Robust Variants}\vspace{-1mm}\label{sec:method}
% \subsection{Flagification of PCA and its robust variants}
We now re-interpret PCA in Euclidean spaces as an optimization on flags of linear subspaces. This flagification will later enable us to introduce more variants and algorithms.
    
% We state a generalization of PCA, which optimizes over flags of a given type. Notice that this is the same objective function as PCA. 
\begin{dfn}[Flagified (weighted-)PCA (fPCA)~\cite{pennec2018barycentric}]
A (weighted-)flag of principal components is the solution to:
    \begin{equation}\label{eq:wflagpca}
         [\![\U]\!]^\star=\argmax_{[\![\U]\!] \in \flag(n+1)}  \mathbb{E}_j \left[ \sum_{i=1}^k w_{ij}\| \pi_{\U_i} (\x_j)\|_2^2 \right].
    \end{equation}
    where $w_{ij}$ denote the weights.
    We refer to a weighted flag PCA algorithm optimized over $\flag(n_1,n_2,\dots,n_k;n)$ as $\mathrm{weighted-fPCA}(n_1,n_2,\dots,n_k;n)$. When $w_{ij}=1 \,\forall i,j$, we recover $\mathrm{fPCA}$.
    % Similarly, a flag of weighted PCs is the solution to:
    %\begin{equation}\label{eq:wflagpca}
    %     [\![\U]\!]^\star=\argmax_{[\![\U]\!] \in \flag(n+1)}  \mathbb{E} \left[ \sum_{i=1}^k w_{ij}\| \pi_{\U_i} (\x_j)\|_2^2 \right]
    %\end{equation}
\end{dfn}

\begin{remark}
The solution to~\cref{eq: pca_opt_rot} is only unique up to rotation, and PCA is unique (up to column signs) because we order by eigenvalues. This ordering imposes a flag structure. Interpreting this optimization problem over a flag emphasizes the nested structure of principal subspaces~\cite{damon2014backwards} and provides a slight loosening of the strict eigenvalue ordering scheme from PCA. Also note that the joint optimization over the whole flag of subspaces (instead of optimizing each subspace independently) poses a computational challenge, preventing~\cite{pennec2018barycentric} from a practical implementation. This gap is filled via a manifold optimization in~\cite{ye2022optimization} by characterizing the Riemannian geometry of $\flag(\cdot)$. We provide further details in the supplementary.
% As we show in our supplementary, PCA is only unique up to an orthogonal transformation, which is the reason why practical implementations sort the eigenspace based on the eigenvalues. Yet, the flag of subspaces which is generated in~\cref{eq:flagpca} is more unique. This is thanks to leveraging the nested structure of principal subspaces~\cite{damon2014backwards}, an important yet overlooked property. Also note that the joint optimization over the whole flag of subspaces (instead of optimizing each subspace independently) poses a computational challenge, preventing~\cite{pennec2018barycentric} from a practical implementation. This gap is filled via a manifold optimization in~\cite{ye2022optimization} by characterizing the Riemanian geometry of $\flag(\cdot)$. 
\end{remark}

\noindent Building off of these, we now flagify the robust variants of PCA before introducing new dimensionality reduction algorithms and moving onto the principal geodesic.

%\begin{remark}
%Although flagification appears to add little information to PCA, it provides a general interpretation of the principal components where we impose only a nested structure of principal subspaces in which the subspace dimension increases depending on flag type. Overall, flagification is a process that allows us to go ahead and generalize other dimensionality reduction algorithms that provide us with a sequence of nested subspaces.    
%\end{remark}


\paragraph{Flagified Robust (Dual-)PCA variants}
To respect the nested structure of flags, we must embed the flag structure into the optimization problem. Generalized versions of robust PCA in~\cref{eq: flagRPCAmax} and Dual PCA in~\cref{eq: flagDPCAmin} change the objective function value and the space over which we optimize. 
We state these flagified formulations below.
\begin{dfn}[Flagified (Dual-)PCA]
In the sequel, we define flagified (f) \RPCA~/ \WPCA~/ \DPCP~/ \WDPCP:
\begin{align}\label{eq: flagRPCAmax}
&[\![\U]\!]^\star = \\
&\begin{cases}
        \argmax\limits_{[\![\U]\!] \in \flag(n+1)}  \mathbb{E}_j \left[ \sum_{i=1}^k\| \pi_{\U_i} (\x_j)\|_2 \right], & \mathrm{(fRPCA)}\\
        \argmin\limits_{[\![\U]\!] \in \flag(n+1)} \mathbb{E}_j \left[ \sum_{i=1}^k \| \x_j  -\pi_{\U_i} (\x_j)\|_2 \right], & \mathrm{(fWPCA)}
        \end{cases}\nonumber\\
&\nonumber\\
&[\![\B]\!]^\star = \label{eq: flagDPCAmin}\\
&\begin{cases}
        \argmin\limits_{[\![\B]\!] \in \flag(n+1)} \mathbb{E}_j \left[ \sum_{i=1}^k\| \pi_{\B_i} (\x_j)\|_2 \right], & \mathrm{(fDPCP)}\\
        \argmax\limits_{[\![\B]\!] \in \flag(n+1)} \mathbb{E}_j \left[ \sum_{i=1}^k \| \x_j  -\pi_{\B_i} (\x_j)\|_2 \right], & \mathrm{(fWDPCP)}
        \end{cases}\nonumber
\end{align}
where $\U_i$ and $\B_i$ as $\X_i$ is defined using~\cref{eq: Xi def}.
\end{dfn}
\begin{remark}
    Formulating these flagified robust PCAs over $\flag(1,2,\dots,k;n)$ recovers $L_1$ formulations and over $\flag(k;n)$ recovers $L_2$ of robust PCA and \DPCP~formulations. This fact is enforced in~\cref{tab:pca_summary}. 
\end{remark}
Inspired by Mankovich and Birdal~\cite{Mankovich_2023_ICCV}, we now show how to implement these robust variants by showing equivalent optimization problems on the Stiefel manifold~\cite{edelman1998geometry}.
We start by viewing weighted \fPCA~in~\cref{eq:wflagpca} as a Stiefel optimization problem in~\cref{prop:wfPCA}. For the rest of this section, we will slightly abuse notation and use $[\![\U ] \!]$ for flags of both primal  
 and dual principal directions, discarding $\B$. We will provide the necessary proofs in our supplementary material.
\begin{prop}[Stiefel optimization of (weighted) fPCA]\label{prop:wfPCA}
    Suppose we have weights $\{w_{ij}\}_{i=1,j=1}^{i=k,j=p}$ for a dataset $\{ \x_j \}_{j=1}^p \subset \R^n$ along with a flag type $(n_1,n_2,\dots, n_k; n)$. We store the weights in the diagonal weight matrices $\{\W_i\}_{i=1}^k$ with diagonals $(\W_i)_{jj} = w_{ij}$. If
    \begin{equation}\label{eq:wflag_pca}
        \U^\ast  = \argmax_{\U \in St(n_k,n)} \sum_{i=1}^k \tr \left( \U^T \X \W_i \X^T \U \I_i \right)
    \end{equation}
    where $\I_i$ is determined as a function of the flag signature. For example, for $\flag(n+1)$: 
    \begin{equation}\label{eq: Ii}
    (\I_i)_{l,s} = 
    \begin{cases}
        1, & l = s \in \{ n_{i-1} + 1, 
 n_{i-1} + 2, \dots, n_i\} \\
        0, &\mathrm{ otherwise}\nonumber\\
    \end{cases}    
\end{equation}
    Then $[\![\U^\ast ]\!] = [\![\U ]\!]^\ast$ is the weighted fPCA of the data with the given weights (e.g., solves~\cref{eq:wflagpca}) as long as we restrict ourselves to a region on $\flag(n+1)$ and $St(n_k,n)$ where (weighted)~\fPCA~is convex.
\end{prop}
\begin{proof}[Sketch of the proof]
Our proof, whose details are in the supp. material, closely follows~\cite{Mankovich_2023_ICCV}.
\end{proof}
We propose an algorithm for finding (weighted)~\fPCA~using Stiefel Conjugate Gradient Descent (Stiefel-CGD)~\cite{hager2006survey,sato2022riemannian} in the supplementary.

Next, we translate the flagified robust PCA optimizations in~\cref{eq: flagRPCAmax,eq: flagDPCAmin} to problems over the Stiefel manifold with diagonal weight matrices
    \begin{align}\label{eq: max_weights}
    (\mathbf{W}_i^+([\![\U]\!]))_{jj}  &= \max \left\{ \| \U \I_i \U^T\x_j\|_2, \epsilon \right\}^{-1},\\
    (\mathbf{W}_i^-([\![\U]\!]))_{jj} &= \max \left\{ \|\x_j -\U \I_i \U^T\x_j\|_2, \epsilon \right\}^{-1},\label{eq: min_weights}
\end{align}
chosen according to the robust \fPCA~optimization of concern, as outlined in~\cref{tab:weight_org}.
% Different robust \fPCA~optimizations correspond to different weights, these correspondences are outlined in~\cref{tab:weight_org}.
\begin{table}[t]
    \centering
    \begin{tabular}{c||c|c}
        \PCA~Variant & \fRPCA~/ \fDPCP & \fWPCA~/ \fWDPCP\\
        \midrule
        Weight & $\mathbf{W}_i^+$ from~\cref{eq: max_weights} & $\mathbf{W}_i^-$ from~\cref{eq: min_weights}
    \end{tabular}
    \caption{Weight matrix assignment according to the flagified robust PCA formulation.\vspace{-3mm}}
    \label{tab:weight_org}
\end{table}


\begin{prop}[Stiefel optimization for flagified Robust (Dual-)PCAs]\label{prop:fPCA_all}
   We can formulate \fRPCA, \fWPCA, \fDPCP, and \fWDPCP~as optimization problems over the Stiefel manifold using $[\![ \U ] \!]^\ast = [\![\U^\ast] \!]$ and the following: 
    \begin{align}\label{eq: stRPCAmax}
    &\U^\star = \\
    &\begin{cases}
            \argmax\limits_{\U \in St(n, n_k)}  \sum_{i=1}^k \tr \left(  \U^T \Pm_i^+\U \I_i  \right), & \mathrm{(fRPCA)}\\
            \argmin\limits_{\U \in St(n, n_k)}\sum_{i=1}^k \tr \left(\Pm_i^- -  \U^T \Pm_i^-\U \I_i  \right), & \mathrm{(fWPCA)}
            \end{cases}\nonumber\\
    &\nonumber\\
    &\U^\star = \label{eq: stDPCAmin}\\
    &\begin{cases}
            \argmin\limits_{\U \in St(n, n_k)} \sum_{i=1}^k \tr \left(  \U^T \Pm_i^+ \U \I_i  \right), & \mathrm{(fDPCP)}\\
            \argmax\limits_{\U \in St(n, n_k)} \sum_{i=1}^k\tr \left(\Pm_i^- -  \U^T \Pm_i^-\U \I_i  \right) & \mathrm{(fWDPCP)}
            \end{cases}\nonumber
    \end{align}
    where $\Pm^-=\X \W^-_i([\![\U]\!]) \X^T$, $\Pm^+=\X \W^+_i([\![\U]\!]) \X^T$ and $\W^-_i([\![\U]\!])$, $\W^+_i([\![\U]\!])$ are defined in~\cref{tab:weight_org} as long as we restrict ourselves to a region on $\flag(n+1)$ and $St(n_k,n)$ where flag robust and dual PCAs are convex.
\end{prop}

% \begin{prop}[Stiefel Optimization for \fDPCP]\label{prop: obj_fn}
%     An iterate $[\![\U]\!]$ of~\cref{alg: flagified pca} for fDPCP will decrease the objective function in~\cref{eq: flagDPCAmin} as long as the weighted fDPCP optimization problem in~\cref{eq: stDPCAmin} can be solved using~\cref{alg: weighted flagified pca} and $\| \U \I_i \U^T \x_j\|_2 \geq \epsilon$ for all $i,j$.
% \end{prop}

~\cref{eq: stRPCAmax,eq: stDPCAmin} offer natural iterative re-weighted optimization schemes on the Stiefel manifold for obtaining flagified robust PCA variants, where we calculate a weighted flagified PCA at each iteration with weights defined in~\cref{tab:weight_org}. This is similar to~\cite{busam2017camera}. We summarize these algorithms in~\cref{alg: flagified pca}.
We further establish the convergence guarantee for the case of \fDPCP~\cref{cor: fdpcp converges} and leave other convergence results to future work.

%\textit{Alg 1. for \fDPCP~converges to $[\![ \U ] \! ]^* \in \flag(n+1)$ when iterates (1) remain in a region on $\flag(n+1)$ and $St(n_k,n)$ where the least squares objective ($f^+$) is convex and (2) adhere to the condition $\| \U \I_i \U^T \x_j\|_2 \geq \epsilon$ for all $i = 1,2,\dots,k$ and $j=1,2,\dots p$.} 
\begin{prop}[Convergence of \cref{alg: flagified pca} for \fDPCP]\label{cor: fdpcp converges}
    \cref{alg: flagified pca} for \fDPCP~converges as long as $\| \U \I_i \U^T \x_j\|_2 \geq \epsilon$ $\forall i,j$ as long as we restrict ourselves to a region on $\flag(n+1)$ and $St(n_k,n)$ where \fDPCP~is convex.
\end{prop}
\begin{proof}[Sketch of the proof]
 Let $f^+: \flag(n+1) \times \flag(n+1) \rightarrow \R$ denote the \fDPCP~objective function and $T: \flag(n+1) \rightarrow \flag(n+1)$ denote an iteration of~\cref{alg: flagified pca}. Similar to~\cite{Mankovich_2023_ICCV,mankovich2023subspace}, we first show that an iteration of~\cref{alg: flagified pca} decreases the \fDPCP~objective value. Then we notice that the real sequence with terms $f^+(T([\![\U^{(m-1)}]\!])) = f^+([\![\U^{(m)}]\!])$ is bounded below by $0$ and is decreasing. %So it converges as $m  \rightarrow \infty$.
 % Let $\lambda_1$ be the largest eigenvalue of $\X \X^T$ with the eigenvector $\bv$. So for any unit vector $\y$, we have $\sqrt{\y^T \X \X^T \y} \leq \sqrt{\lambda_i}$ For fRPCA notice that the real sequence with terms $f([\![\Y_r]\!]) \in \R$ is bounded above by $\sum_{i=1}^k \sum{l=1}^{m_i} \lambda_l$ and is increasing by ~\cref{prop: obj_fn}. So it converges as $r \rightarrow \infty$. 
\end{proof}

% \begin{prop}\label{prop: obj_fn}
%     An iteration of~\cref{alg: flagified pca} will produce a further optimal objective function as long as the weights satisfy for all $i,j$ either (1) $\| \Y \I_i \Y^T \x_j\|_2 \geq \epsilon$ for RPCA and DPCP; or (2) $\| \x_j - \Y \I_i \Y^T \x_j\|_2 \geq \epsilon$ for WPCA.
% \end{prop}
% Proof of this is in~\cref{sec:fPCAconv}.

% \begin{prop}[Convergence for fDPCP and fWPCA]\label{cor: flagirls obj converges}
% Let $[\![\Y_m]\!] \in \flag(n+1)$ be an iterate of ~\cref{alg: flagified pca} and $f:\flag(d+1) \rightarrow \R$ denote the objective value. $f([\![\Y_m]\!])$ converges as $m \rightarrow \infty$ as long as the weights satisfy for all $i,j$ either $\| \Y \I_i \Y^T \x_j\|_2 \geq \epsilon$ for DPCP or $\| \x_j - \Y \I_i \Y^T \x_j\|_2 \geq \epsilon$ for WPCA.
% % Let $[\![\Y_m]\!] \in \flag(n+1)$ be an iterate of ~\cref{alg: flagified pca} and $f:\flag(d+1) \rightarrow \R$ denote the objective value (e.g., fRPCA in~\cref{eq: flagRPCAmax}). $f([\![\Y_m]\!])$ converges as $m \rightarrow \infty$ as long as the weights satisfy for all $i,j$ either (1) $\| \Y \I_i \Y^T \x_j\|_2 \geq \epsilon$ for RPCA and DPCP; or (2) $\| \x_j - \Y \I_i \Y^T \x_j\|_2 \geq \epsilon$ for WPCA.
% \end{prop}

% \begin{proof}
%  For fDPCP and fWPCA notice that the real sequence with terms $f([\![\Y_r]\!]) \in \R$ is bounded below by $0$ and is decreasing by ~\cref{prop: obj_fn}. So it converges as $r \rightarrow \infty$.

%  % Let $\lambda_1$ be the largest eigenvalue of $\X \X^T$ with the eigenvector $\bv$. So for any unit vector $\y$, we have $\sqrt{\y^T \X \X^T \y} \leq \sqrt{\lambda_i}$ For fRPCA notice that the real sequence with terms $f([\![\Y_r]\!]) \in \R$ is bounded above by $\sum_{i=1}^k \sum{l=1}^{m_i} \lambda_l$ and is increasing by ~\cref{prop: obj_fn}. So it converges as $r \rightarrow \infty$. 
% \end{proof}



% Similar propositions apply for~\cref{eq: flagRPCAmin,eq: flagDPCAmin,eq: flagDPCAmax} with only a small change in the weight matrices $\W_i$ and are listed in the appendix. 



% Varying convergence reliability for these algorithms for all flagified PCA versions is summarized in~\cref{tab:summary}. Notice that an iteration of~\cref{alg: flagified pca} using $f$-objective for fRPCA is weighted fPCA.

% \nate{Figure out wording of this section to introduce \fRPCA~and \fWPCA}

% \paragraph{Finding \fRPCA and \fWPCA}
% Disheartened by the ineffectiveness of iterative weighted flagified PCAs for finding \fRPCA, \fWPCA, and \fWDPCP, we propose a new objective function to be optimized at each iteration in~\cref{prop: A_opt}.
% \begin{prop}[Alternative Stiefel optimization for fWPCA, fRPCA]\label{prop: A_opt}
%     Fixing $\{\W_i\}_{i=1}^k$, optimizing $E^+(\U)$ and  $E^-(\U)$ is the same as optimizing
%     \begin{equation}\label{eq: A_obj}
%      \tr\left(  \mathbf{A}([\![\U]\!]) \U \right)
%     \end{equation}
%     using the matrix
%     \begin{equation}\label{eq:A}
%         \mathbf{A}([\![\U]\!]) = \sum_{i=1}^k  \I_i \U^T \X \W_i \X^T.
%     \end{equation}
% \end{prop}
% The proof of this is in the supplementary material. We use~\cref{prop: A_opt} to form another iterative optimization scheme for finding \fRPCA, \fWPCA, and \fWDPCP. We update our weights as before, but optimize~\cref{eq: A_obj} at each iteration rather than weighted flag PCA. In our experiments we find that this scheme does not converge for \fWDPCP, but does converge for \fRPCA and \fWPCA. This is likely due to the fact that we are optimizing a linear objective function using CGD on the Stiefel manifold at each iteration and we can only descend on one direction. Therefore we offer an algorithm for finding both \fRPCA~ and \fWPCA~ using~\cref{eq: A_obj} in~\cref{alg: flagified pca}. Proof of convergence of this algorithm for \fRPCA~ and \fWPCA~ is future work.

% First, we define $\mathbf{A}$ as a function of $[\![\U]\!]$:
% \begin{equation}\label{eq:A}
%     \mathbf{A}([\![\U]\!]) = \sum_{i=1}^k  \I_i \U^T \X \W_i \X^T.
% \end{equation}
% $\mathbf{A}$ is to be assigned differently depending on our variant of PCA according to changing diagonal weight matrices $\W_i$ defined in~\cref{eq: max_weights,eq: min_weights}. We use $\mathbf{A}([\![\Z]\!])$ to re-write fRPCA/ fWPCA/ fWDPCP  weighted flag PCA objective in~\cref{eq:wflag_pca} as
% \begin{equation}\label{eq: A_obj}
%  \tr\left(  \mathbf{A}([\![\U]\!]) \U \right).
% \end{equation}

% So we run experiments where we iteratively optimize~\cref{eq: A_obj} for fRPCA/ fWPCA/ fWDPCP. In our experiments we find that this scheme does not converge for fWDPCP, but does converge for fRPCA/ fWPCA. Therefore we offer an algorithm for finding both fRPCA/ fWPCA using~\cref{eq: A_obj} in~\cref{alg: flagified pca}.


\begin{algorithm}[t]
\setstretch{1.13}
\caption{\fRPCA, \fWPCA, \fDPCP}\label{alg: flagified pca}
 \textbf{Input}: {Data $\{\x_j \in \R^n\}_{j=1}^p $, flag type $(n+1)$, $\epsilon>0$}\\
 \textbf{Output}: Flagified principal directions $[\![\U]\!]^\ast $ \\[0.25em] %\in \flag(n+1)
 Initialize $[\![\U]\!]$\\
 \While{(not converged)}
 {
     \vspace{.1cm}
    \textbf{Assign weights:}\\
    \Case{fRPCA or fDPCP}{
        Assign $\{\mathbf{W}_i^+([\![\U]\!])\}_{i=1}^k$ using~\cref{eq: max_weights}
            }
    \Case{fWPCA}{
        Assign $\{\mathbf{W}_i^-([\![\U]\!])\}_{i=1}^k$  using~\cref{eq: min_weights}
            }
    \vspace{.1cm}
    \textbf{Update estimate:}\\
    \Case{fRPCA} {
            $\mathbf{A}^+ \gets \sum_{i=1}^k  \I_i \U^T \X \W_i^+ \X^T$ \\
            $\U \gets \argmax_{\Z \in St(k,n)} \mathbf{A}^+ ( [\![ \U ]\!] ) \Z$
           }
    \Case{fWPCA}{
            $\mathbf{A}^- \gets \sum_{i=1}^k  \I_i \U^T \X \W_i^- \X^T$ \\
            $\U \gets \argmin_{\Z \in St(k,n)} \mathbf{A}^- ( [\![ \U ]\!] ) \Z$
            }
    \Case{fDPCP}{
        Assign $\U$ using~\cref{eq: stDPCAmin} with $\{\mathbf{W}_i^+([\![\U]\!])\}$
           }
}
$[\![\U]\!]^\ast \gets [\![\U]\!]$
\end{algorithm}
\vspace{-4mm}







% \begin{table}[H]    \centering
%     \begin{tabular}{c|cccc}
%            & fRPCA & fWPCA & fWDPCP & fDPCP \\
%            \hline
%         $f_{[\![ \Y ]\!]}$ & - & + & - & +\\
%         $g_{[\![ \Y ]\!]}$ & + & + & - & -
%     \end{tabular}
%     \label{tab:summary}
%     \caption{Convergence: reliable  is +, unreliable is -. \tolga{What is a convergence reliability? :) We have proofs?} \nate{I made this table as a note to keep track of what I've observed in my experiments so far. Perhaps we can back this up with proofs!}}
% \end{table}

\begin{remark}[Flagifying PGA or Tangent-PCA]
    True flagification of exact PGA is a difficult task. 
    While~\cref{eq: tangent_flag} resembles a flag structure, this is not the case for the nonlinear submanifolds in~\cref{eq:subman_flag}~\cite{haller2020nonlinear,haller2023weighted,ciuclea2023shape}.
    Instead, we will focus on its tangent approximations, where we map the data to the tangent space of the mean and perform (weighted) \fPCA~along with \fRPCA, \fWPCA, and \fDPCP~in the tangent space, just like in \TPCA~(\cref{rem:TPCA}).
    % To do this, all we do is preform weighted \fPCA~along with \fRPCA, \fWPCA, and \fDPCP~in the tangent space using inner products. This results in flagified tangent versions of \fPCA, \fRPCA, \fWPCA~and \fDPCP~called \fTPCA, \fTRPCA, \fTWPCA, and \fTDPCP~respectively and offer an algorithm to find these in~\cref{alg: tPDs}.
\end{remark}

\begin{remark}[Computational Complexity (CC)]
    \cref{alg: flagified pca} for \fRPCA, \fWPCA, and \fDPCP~ has a CC of $O(N_oM)$ and~\cref{alg: flagified pca} in $\TxM$ for \fTRPCA, \fTWPCA, and \fTDPCP~has a CC of $O(N_{\mu}pn n_k^2) + O(N_oM)$, where $N_o$ is the number of iterations of the outer loop, $N_{\mu}$ is the number of iterations of the Karcher median, $M$ is the CC of Stiefel CGD, $p$ is the number of points, and the flag is of type $(n_1,n_2,\dots,n_k;n)$.
\end{remark}


\begin{remark}[Flagifying Tangent (Dual)-PCA]
All these flagified PCA formulations can be run in the tangent space of a manifold centroid, producing a corresponding \emph{tangent} version. Following the same convention, we dub these \fTPCA, \fTRPCA, \fTWPCA, and \fTDPCP~and propose an algorithm for their computation in the supplementary.
\end{remark}
\setlength{\textfloatsep}{8pt}%\vspace{-20mm}
\begin{remark}[Even further fPCA variants]
As summarized in~\cref{tab:fl_type}, optimizing over $\flag(1,2,\dots,k;n)$ recovers $L_1$ versions of robust PCA while $\flag(k;n)$ recovers $L_2$ versions, in particular \RPCA, \WPCA, and \DPCP.
Naturally, one can employ other flag types recovering robust PCAs ``in between'' $L_1$ and $L_2$ that differ from $L_p$, $1<p<2$. Moreover, these flagified PCA formulations can be run in the tangent space of a manifold centroid to recover tangent robust $L_1$ and $L_2$ principal directions, and even ones in between. These generalizations immediately produce a plethora of novel dimensionality reduction algorithms. 
While we glimpse their potential advantages in~\cref{sec:eucPD}, we leave their thorough investigation for a future study.
%, which we cannot cover in the scope of work. 
% We plan to address these more in depth in a future study.
\end{remark}



% 
% \paragraph{Summary}
% In this section we proposed new flagified robust PCA variants. We offer \cref{alg: flagified pca} as a general algorithm which can be used to find \fRPCA, fWPCA, and fDPCP. Certainly, one could further optimize the weight matrices in~\cref{eq: max_weights,eq: min_weights} according to~\cite{peng2022global} but we consider this line of work as a future project. Finally, this algorithm generalizes other formulations of robust PCA because certain flag types recover $L_1$ and $L_2$ formulations of \RPCA, \WPCA, and \DPCP (see~\cref{tab:pca_summary}) and all other flag types recover robust PCA ``in between'' $L_1$ and $L_2$ robust PCAs. We emphasize this in~\cref{tab:flags_rule}.

% Additionally, running these flagified PCA formulations in the tangent space to a manifold centroid immediately produces a plethora of novel dimensionality reduction algorithms: \fTPCA, \fTRPCA, \foneTWPCA, and \fTDPCP. Again, we can use these methods to recover tangent robust $L_1$ and $L_2$ principal directions and discover new tangent robust principal directions by simply changing the flag type.


==> content/old_versions/method_less_old.tex <==
\vspace{-1mm}\section{Methods}\vspace{-1mm}\label{sec:method}



\begin{dfn}[Riemannian Manifold~\cite{lee2006riemannian}]
A \emph{Riemannian manifold} $M$ is a smooth manifold with a positive definite inner product on the tangent space. This inner product defines a Riemannian metric on $M$ and is denoted $\langle \cdot, \cdot \rangle : T_x(M) \times T_x(M) \rightarrow \R$ where $x \in M$ and $T_x(M)$ is the tangent space to $M$ at $x$. Let $\bv \in T_x(M)$ be a tangent vector to $M$ at $x$. The \emph{exponential map} is $\text{exp}_x(\bv) : T_x(M) \rightarrow M$. The \emph{logarithm map} is $\text{log}_x(y) : M \rightarrow T_x(M)$ for $x,y \in M$ and computes the direction from $x$ to $y$\footnote{The logarithm map may not be defined everywhere on $M$.}. A \emph{geodesic} $\gamma : \R \rightarrow M$ parameterizes a path from $\gamma(0) = x$ to $\gamma(1) = y$. The geodesic can be written as $\gamma = \exp_x^{t\log_x(y)}$ for $t \in \R$. $H \in M$ is a geodesic submanifold at $x \in M$ if all geodesics passing through $x$ in $H$ are geodesics in $M$.
\end{dfn}

\begin{dfn}[Flag]\label{def:flagobj}
A \emph{flag} in a finite dimensional vector space $\mathcal{V}$ over a field is a sequence of nested subspaces with \emph{increasing} dimension, each containing its predecessor, \ie the filtration: $\{\emptyset \}=\mathcal{V}_0 \subset \mathcal{V}_1 \subset \dots \subset \mathcal{V}_{k} \subset \mathcal{V}$ with $0=n_0<n_1<\dots<n_k<n_{k+1} = n$ where $\mathrm{dim} \mathcal{V}_i=n_i$ and $\mathrm{dim} \mathcal{V}=n$. We say this flag is of \emph{type} or \emph{signature} $(d_1, \dots ,d_k,d)$. 
%A flag is called \emph{complete} if $d_i = i,\,\forall i$. Otherwise the flag is \emph{incomplete} or \emph{partial}. 

\noindent\textbf{\emph{Notation}:} A flag, $[\![\X]\!]$ of type $(n_1, \dots ,n_k, n)$, is represented by a truncated orthogonal matrix $\X \in \R^{n \times n_k}$. Let $m_j = n_j-n_{j-1}$ for $j=1,2,\dots, k+1$, and $\X_j  \in \R^{n \times m_j}$ for $j=1,2,\dots, k$ whose columns are the $n_{j-1}+1$ to $n_{j}$ columns of $\X$. $[\![\X]\!]$ is
\begin{equation}
     [ \X_1 ]  \subset [\X_1, \X_2] \subset \cdots \subset  [\X_1, \dots, \X_k] = [\X] \subset \R^n. \nonumber
\end{equation}
\end{dfn}

\begin{dfn}[Flag manifold]
The aggregate of all flags of the same type, \ie a certain collection of ordered sets of vector subspaces, admits the structure of manifolds. We refer to this \emph{flag manifold} %with its dimension (type) 
as $\flag(n_1, ..., n_k; n)$ or equivalently as $\flag(n+1)$. The points of $\flag(n+1)$
%$\flag(d_1, ..., d_k; d)$ 
parameterize all flags of type $(n_1, ..., n_k,n)$. 
Flag manifolds generalize Grassmannians~\cite{edelman1998geometry} because $\flag(k; n)=\Gr(k,n)$. $\flag(n+1)$ can be thought of as a quotient of groups ~\cite{ye2022optimization}:
\begin{equation*}
\flag(d+1) = St(d_k, n)/O(m_1) \times O(m_2) \times \cdots \times O(m_{k+1}),
\end{equation*}
where
$St(d_k, n) = \{\X \in \R^{n \times d_k} : \X^T \X = \I \} $ is a Stiefel manifold.
\end{dfn}


\subsection{PCA and its robust variants}
Given a set of $k < n$ orthonormal vectors $\{\bu_i\}_{j=1}^k \subset \R^n$, define the matrix $\U = [\bu_1,\dots,\bu_k]$. The projection of $\x$ onto the subspace spanned by this basis (namely $S_\U$) is $\pi_{S_\U}(\x) := \U \U^T \x$.

Suppose we have $p$ samples (points) with $n$ random variables (features) $\mathcal{X} = \{ \x_i \}_{i=1}^p \subset \R^n$ with a sample mean of $0$. The directions found by PCA either maximize variance (\cref{eq: minpca}) or minimize reconstruction error (\cref{eq: minpca}).


\begin{dfn}[PCA~\cite{hotelling1933analysis}]
The $i$th principal direction is
The $i$th principal direction is
\begin{equation}\label{eq: maxpca}
\mathbf{u}_{i} = \argmax_{\substack{\mathbf{u}^T \mathbf{u} = 1 \\ \mathbf{u} \in S_i^\perp }} \mathbb{E} \left[\|  \pi_{S_{\mathbf{u}}} (\x_j) \|_2^2 \right]
\end{equation}
\begin{equation}\label{eq: minpca}
\mathbf{u}_{i} = \argmin_{\substack{\mathbf{u}^T \mathbf{u} = 1 \\ \mathbf{u} \in S_{i-1}^\perp}} \mathbb{E} \left[\|  \bm{\x_j} - \pi_{S_{\mathbf{u}}} (\x_j) \|_2^2 \right]
\end{equation}
\end{dfn}
In general, PCA gives us a $k<n$ dimensional embedding of the data as the columns of $\U^T\X \in \R^{k \times p}$. We can approximately invert PCA by left multiplication by $\U$.

\paragraph{Robust PCA (RPCA)}

Outliers of a dataset are generally considered data that significantly deviate from the general pattern of the dataset. Points in the dataset that are not outliers will be called inliers. If we have a dataset with many outlier points, the directions of maximum variance (detected by PCA) may represent these outliers than the actual dataset. Therefore, we seek methods for dimensionality reduction that capture a space containing only the dataset's inliers. There are four variants of robust PCA (RPCA):

\begin{dfn}[PCA-L1~\cite{markopoulos2014optimal}]
The $i$th L1 principal direction is
\begin{equation}\label{eq: maxpcal1}
\mathbf{u}_{i} = \argmax_{\substack{\mathbf{u}^T \mathbf{u} = 1 \\ \mathbf{u} \in S_{i-1}^\perp}} \mathbb{E} \left[\|  \pi_{S_{\mathbf{u}}} (\x_j) \|_2 \right]
\end{equation}
\end{dfn}

\begin{dfn}[WPCA~\cite{neumayer2020robust}]
The $i$th Weiszfeld principal direction is
\begin{equation}\label{eq: minpcal1}
\mathbf{u}_{i} = \argmin_{\substack{\mathbf{u}^T \mathbf{u} = 1 \\ \mathbf{u} \in S_{i-1}^\perp}} \mathbb{E} \left[\|  \x_j - \pi_{S_{\mathbf{u}}} (\x_j) \|_2 \right]
\end{equation}
\end{dfn}

Both~\cref{eq: maxpcal1} and~\cref{eq: minpcal1} also solve respective the $1$-norm optimization problems
\begin{equation}
    \U = \argmax_{\U^T \U = \I} \mathbb{E} \left[ \|  \pi_{S_{\U}} (\x_j) \|_1 \right]
\end{equation}
\begin{equation}
    \U = \argmax_{\U^T \U = \I} \mathbb{E} \left[ \|  \x_j - \pi_{S_{\mathbf{U}}} (\x_j) \|_1 \right]
\end{equation}

\begin{dfn}[\textcolor{red}{PCA-L2 cite}]
\begin{equation}\label{eq: maxpcal2}
\U = \argmax_{\U^T \U = \I} \mathbb{E} \left[ \|  \pi_{S_{\U}} (\x_j) \|_2 \right]
\end{equation}
\end{dfn}

\begin{dfn}[\textcolor{red}{WPCA-L2 cite}]
\begin{equation}\label{eq: minpcal2}
\U = \argmin_{\U^T \U = \I}  \mathbb{E} \left[\|  \x_j - \pi_{S_{\mathbf{U}}} (\x_j) \|_2 \right]
\end{equation}
\end{dfn} 

\paragraph{Dual PCA (DPCA)}

Our model for data with inliers and outliers is the data matrix with $p$ samples of $n$ features: $\X =  [\textbf{A}, \mathbf{B}] \mathbf{P}   \in \R^{n \times p}$. The columns of $\textbf{A}$ and $\mathbf{B}$ are inliers and outliers, respectively. We assume there are more inliers than outliers. $\mathbf{P}$ is a permutation matrix. We assume the samples live on the unit sphere, namely, $\{\x_1, \x_2,\dots, \x_p\} \in \mathbb{S}^{n-1}$. DPCA seeks a subspace $S_\ast = \text{span}\{ \vb_1,  \vb_2, \dots,  \vb_k\}$ so that $S_\ast^\perp$ contains the most inliers (e.g., columns of $\A$). So, we seek vectors, namely $\{\vb_1,  \vb_2, \dots,  \vb_k\}$, that are as orthogonal as possible to the span of the inliers.

\begin{dfn}[DPCA~\cite{vidal2018dpcp}]
    Let $S_i = \text{span} \{ \vb_1,  \vb_2, \dots,  \vb_i \}$. The $i$th dual principal component is
    \begin{equation}
        \vb_{i} =  \argmin_{\substack{\| \vb \| = 1 \\ \vb \in S_{i-1}^\perp}} \| \X^T \vb \|_0.
    \end{equation}
\end{dfn}

\begin{dfn}[Dual Principal Component Pursuit~\cite{vidal2018dpcp}]
    Let $\{\x_i\}_{i=1}^p \subset \R^n$ be unit vectors. dual principal component pursuit (DPCP) is
    \begin{equation}\label{eq: dpcp}
        \vb_{i} = \argmin_{\substack{ \| \vb \| = 1 \\ \vb \in S_{i-1}^\perp}}  \mathbb{E} \left[\|  \pi_{S_{\mathbf{b}}} (\x_j) \|_2 \right]
    \end{equation}
\end{dfn}

\begin{dfn}[DPCP-IRLS~\cite{vidal2018dpcp}]
    DPCP-IRLS (Iteratively Reweighted Least Squares) approximates DPCP: 
    \begin{equation}\label{eq: dpcpirls}
        \B = \argmin_{\B^T \B = \I} \mathbb{E} \left[ \|  \pi_{S_{\B}} (\x_j) \|_2 \right]
    \end{equation}
\end{dfn}
DPCP-IRLS is solved by running an IRLS algorithm~\cite{vidal2018dpcp}. A general Grassmannian realization of DPCP-IRLS, along with a ``flagified'' version of this realization, is in~\cref{sec:grassdpcp}.

Following what was done for robust PCA formulations, we introduce two more forms for Dual PCA.
\begin{dfn}[\textcolor{red}{DPCP-Max cite}]
    \begin{equation}\label{eq: dpcpmax}
        \vb_{i} = \argmax_{\substack{ \| \vb \| = 1 \\ \vb \in S_{i-1}^\perp}}  \mathbb{E} \left[\|  \x_j - \pi_{S_{\mathbf{b}}} (\x_j) \|_2 \right]
    \end{equation}
\end{dfn}

\begin{dfn}[\textcolor{red}{DPCP-IRLS-Max cite}]
    \begin{equation}\label{eq: dpcpirlsmax}
        \B = \argmax_{\B^T \B = \I} \mathbb{E} \left[ \| \x_j  -\pi_{S_{\B}} (\x_j) \|_2 \right]
    \end{equation}
\end{dfn}

Similarly to RPCA formulations, we can write~\cref{eq: dpcp,eq: dpcpmax} as $1$-norm optimizations.

\paragraph{Summary}

The different formulations for PCA and Dual PCA are summarized in~\cref{tab:summary}. We can traverse between the $1$ and $2$-norm formulations using $1<p<2$ norms.

\begin{table}[H]    \centering
    \begin{tabular}{c|cccc}
           & \multicolumn{2}{c}{RPCA} & \multicolumn{2}{c}{DPCA} \\
           & Max & Min & Max & Min \\
           \hline
        L1 & \cref{eq: maxpcal1} & \cref{eq: minpcal1} & \cref{eq: dpcpmax} & \cref{eq: dpcp}\\
        L2 & \cref{eq: maxpcal2} & \cref{eq: minpcal2} & \cref{eq: dpcpirlsmax} & \cref{eq: dpcpirls}
    \end{tabular}
    \label{tab:summary}
    \caption{A taxonomy of RPCA and DPCA formulations.}
\end{table}





\subsection{Flagification of PCA and its robust variants}

We now generalize PCA and its variants using flags by grouping eigenvectors using the flag type. The PCA optimization problem is naturally an optimization problem on the Stiefel manifold, $St(k,n) := \{ \Y \in \R^{k \times n} \: : \: \Y^T \Y = \I\}$. Suppose $\U = [\bu_1, \bu_2, \dots, \bu_k] \in St(k,n)$ are the $k<n$ principal components of a data matrix $\X$. These are naturally ordered according to their decreasing associated objective function values\footnote{The objective function values are also referred to as explained variances, eigenvalues and squared singular values}. This results in the nested subspace structure
\begin{equation}
    [\![ \U ]\!] = [\bu_1] \subset [\bu_1, \bu_2] \subset \cdots \subset [\bu_1, \bu_2, \dots, \bu_k] \subset \R^n.
\end{equation}
So also can think of $\U \in \flag(1,2,\dots,k; n)$, and consequently, reformulate PCA as an optimization problem over $\flag(1,2,\dots,k; n)$. 
%In fact, it is known that $\flag(1,2,\dots,k; n) \cong St(k,n)$\nate{CITE}. 
Thinking of $\U$ as $[\![ \U ]\!]$ emphasizes the nested subspace structure of the principal components according to their associated objective function values.

What if we have multiple principal components with the same objective function value? In other words, suppose we have at least one eigenvalue of $\X \X^T$ with a geometric multiplicity greater than $1$? For example, assume our dataset has a large variance on some $2$-plane, and all other directions orthogonal to that plane have smaller, unequal variance. Then, the first two principal components, $\bu_1$ and $\bu_2$, will have the same objective function value in~\cref{eq: maxpca}. Any rotation of the two vectors within the plane $\text{span}(\bu_1, \bu_2)$ will still produce the same objective function values. So,~\cref{eq: maxpca} is no longer a convex optimization problem over $St(k,n)$ because the first two principal components are not unique. However, if we remove $[\bu_1] \subset [\bu_1, \bu_2]$ from the nested subspace structure and consider $[\![ \U ]\!] \in \flag(2,3,\dots, k;n)$ as
\begin{equation}
    [\![ \U ]\!] = [\bu_1, \bu_2] \subset [\bu_1, \bu_2, \bu_3] \subset \cdots \subset [\bu_1, \dots, \bu_k]\subset \R^n.
\end{equation}
Then we have a unique solution to~\cref{eq: maxpca} over $\flag(2,3,\dots, k;n)$ in place of $St(k,n)$. In practice, it is unlikely that we will have two eigenvectors with the same eigenvalue. However, we can consider two eigenvalues the same as long as $|\lambda_i - \lambda_j| < \epsilon$ for some $\epsilon > 0$.

\begin{exmp}
Suppose we sample points $\{\x^{(i)}\}_{i=1}^{5000} \subset \R^4$ with coordinates sampled as $\x^{(i)}_1, \x^{(i)}_2 \sim \mathcal{N}(0,1)$, $\x^{(i)}_3 \sim \mathcal{N}(0,0.5)$, and $\x^{(i)}_4 \sim \mathcal{N}(0,0.1)$ where $\mathcal{N}(\mu,\sigma)$ is a normal distribution with mean $\mu$ and standard deviation $\sigma$. \cref{fig:why_flag_pca1} emphasizes that the first two principal components of these data and the first two coordinates of these data are rotations of one another. \cref{fig:why_flag_pca2} shows nearly identical explained variance for the first two principal components and~\cref{fig:why_flag_pca3} shows the first two PCs are identically $0$ for the first two coordinates of the data. Overall, we should preform PCA on $\flag(2,3,4;5)$ instead of $\flag(1,2,3,4;5)$.
% \begin{figure}[H]
%     \centering
%     \includegraphics{figures/flag_exp_gaussian.pdf}
%     \caption{Mapping the data onto $\mathbf{e}_1 = [1,0,0,0]^T$ and $\mathbf{e}_1 = [0,1,0,0]^T$. Any basis vectors orthogonal to $\text{span}(\mathbf{e}_3, \mathbf{e}_4)$ will work for the first two principle components of our data.}
%     \label{fig:why_flag_pca0}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics{figures/flag_exp_2pcs.pdf}
%     \caption{Mapping the data onto the first two principle components. Any basis vectors orthogonal to $\text{span}(\mathbf{e}_3, \mathbf{e}_4)$ will work for the first two principle components of our data.}
%     \label{fig:why_flag_pca1}
% \end{figure}

\begin{figure}[t]
  \centering
  \subfloat{
    \includegraphics[width=0.22\textwidth]{figures/flag_exp_gaussian.pdf}
    % \label{fig:subfig1}
  }
  \hfill
  \subfloat{
    \includegraphics[width=0.22\textwidth]{figures/flag_exp_2pcs.pdf}
    % \label{fig:subfig2}
  }
  \caption{Mapping the data onto $\mathbf{e}_1 = [1,0,0,0]^T$ and $\mathbf{e}_1 = [0,1,0,0]^T$ (left) and the first two principle components (right). Any basis vectors orthogonal to $\text{span}(\mathbf{e}_3, \mathbf{e}_4)$ will produce a rotated version of the same plots so in this case, PCA is not unique on $\flag(1,2,3;4)$.}
  \label{fig:why_flag_pca1}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width =\linewidth]{figures/flag_exp_evr.pdf}
    \caption{The explained variances (objective function values) for the PCs.}
    \label{fig:why_flag_pca2}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width =\linewidth]{figures/flag_exp_pcs.pdf}
    \caption{The principal directions.}
    \label{fig:why_flag_pca3}
\end{figure}
\end{exmp}

Motivated by this example, we state a generalization of PCA, which optimizes over flags of a given type.
\begin{dfn}[Flagified PCA (fPCA)~\cite{pennec2018barycentric}]
A flag of principal components is the solution to:
    \begin{equation}\label{eq:flagpca}
         \argmax_{[\![\U]\!] \in \flag(n+1)}  \mathbb{E} \left[ \sum_{i=1}^k\| \pi_{\U_i} (\x_j)\|_2^2 \right]
    \end{equation}
\end{dfn}
Ye~\etal find a solution~\cref{eq:flagpca} using Newton's method on the flag manifold ~\cite{ye2022optimization} and Nguyen offers a method for solving such a problem using RTR on flag manifolds~\cite{nguyen2022closed}. These algorithms produce the same basis vectors for flags regardless of flag type. These basis vectors are different than those found using standard PCA. But, for $[\![ \U ]\!] \in \flag(n_1,n_2,\dots,n_k,n)$ that solves~\cref{eq:flagpca} using either Newton's method or RTR, the column space of $\U_{:,:n_k}$ is the same as the span of the first $n_k$ principal components. This is because the objective function in~\cref{eq:flagpca} is invariant to ordering the columns of $\Y$.

Variants on flagified PCA that maximize $\tr(\Y^T\X\X^T \Y)^q$ over $\flag(n+1)$ are coined ``nonlinear eigenflags'' and are difficult to solve for $q=2$~\cite{ye2022optimization}. Yet, methods from Mankovich~\etal can be adapted to solve such problems, especially for $q = 1/2$. Another variant of fPCA is weighted fPCA where we assume a weight for each subspace dimension in the flag $i$ and each data point $j$ as $w_{ij} \in \R$. 

\begin{dfn}[Weighted fPCA]
A flag of principal components is the solution to:
    \begin{equation}\label{eq:flagpca}
         \argmax_{[\![\U]\!] \in \flag(n+1)}  \mathbb{E} \left[ \sum_{i=1}^k w_{ij}\| \pi_{\U_i} (\x_j)\|_2^2 \right]
    \end{equation}
\end{dfn}

Although flagification appears to add little information to PCA, it provides a general interpretation of the principal components where we impose only a nested structure of principal subspaces in which the subspace dimension increases depending on flag type. Overall, flagification is a process that allows us to go ahead and generalize other dimensionality reduction algorithms that provide us with a sequence of nested subspaces.


\paragraph{Flagified RPCA}
For Flagified PCA to respect the nested structure of flags, we must embed the flag structure into the optimization problem. RPCA allows us to do this.
\begin{dfn}[fPCA-L1]
    \begin{equation}\label{eq: flagRPCAmax}
        \argmax_{[\![\U]\!] \in \flag(n+1)}  \mathbb{E} \left[ \sum_{i=1}^k\| \pi_{\U_i} (\x_j)\|_2 \right].
    \end{equation}
\end{dfn}

\begin{dfn}[fWPCA]
    \begin{equation}\label{eq: flagRPCAmin}
        \argmin_{[\![\U]\!] \in \flag(n+1)} \mathbb{E} \left[ \sum_{i=1}^k \| \x_j  -\pi_{\U_i} (\x_j)\|_2 \right].
    \end{equation}
\end{dfn}


% \nate{Check convexity. Over reals and flag.}

% \footnote{We can generalize this to $\| \cdot \|_2^q$ for $q \in (0,2)$}
% Let $\widehat{\x}_j = \x_j/\| \x_j \|_2$. Then a similar optimization problem is
% \begin{equation}\label{eq:medianflagPCA}
%     \argmin_{[\![\Y]\!] \in \flag(n+1)} \sum_{j=1}^p \sum_{i=1}^k \sqrt{1-\widehat{\x}_j^T \Y_i \Y_i^T \widehat{\x}_j}.
% \end{equation}
% If $\widetilde{\x}_j = \widehat{\x}_j$ for all $j$, then these problems have the same optimizers. Otherwise, the optimizers are not necessarily the same. \cref{eq:realflagPCA} is the most natural version of Flagified PCA, whereas~\cref{eq:medianflagPCA} resembles the chordal flag median from~\cite{mankovich2023chordal}.

% We can approximate~\cref{eq:realflagPCA} with an IRLS (Iteratively Reweighted Least Squares) framework where an iteration solves a weighted Stiefel manifold optimization problem. The optimization problem in~\cref{eq:realflagPCA} and algorithm derived from~\cref{prop:IRLSPCA} provides a generalization of a problem similar to what is investigated in Weiszfeld-PCA~\cite{neumayer2020robust}. We can consider a flagified version of Weiszfeld-PCA
% \begin{equation}
%     \argmin_{[\![\Y]\!] \in \flag(n+1)} \sum_{j=1}^p \sum_{i=1}^k \| (\I-\Y_i\Y_i^T)\widetilde{\x}_j\|_2.
% \end{equation}

% Define the matrix $\A$ as
% \begin{equation}\label{eq:A}
%     \A([\![\Y]\!])=  \begin{bmatrix}
%                 \Y_1^T \widetilde{\X}^T \mathbf{W}_1([\![\Y]\!]) \widetilde{\X}\\
%                 \Y_2^T \widetilde{\X}^T \mathbf{W}_2([\![\Y]\!]) \widetilde{\X}\\
%                 \vdots\\
%                 \Y_{n_k}^T \widetilde{\X}^T \mathbf{W}_{n_k}([\![\Y]\!]) \widetilde{\X}
%         \end{bmatrix}.
% \end{equation}
% $\mathbf{W}_i([\![\Y]\!])$ is a diagonal matrix whose $j$th diagonal entry is
% \begin{equation}\label{eq: irls weights}
%     (\mathbf{W}_i([\![\Y]\!]))_{jj} = \frac{1}{\max \left( \| \Y_i^T \widetilde{\x}_j\|_2, \epsilon \right)},
% \end{equation}
% with $\epsilon = 10^{-8}$.
% \nate{Try different functions for weights...}

% \begin{prop}\label{prop:IRLSPCA}
%     Suppose $[\![\Y]\!] \in \flag(n+1)$ solves~\cref{eq:realflagPCA} and $\| \Y_i^T \x_j\|_2 \geq \epsilon$ for all $i$ and $j$. Then $\Y \in St(n_k,n)$ must also solve
%     \begin{equation}\label{eq:STrealflagPCA}
%         \argmax_{\Y \in St(n_k,n)} \tr \left( \A([\![\Y]\!]) \Y \right)
%     \end{equation}
%     where $\A$ is defined in~\cref{eq:A}.
% \end{prop}

% \begin{proof}
%     First, we will translate~\cref{eq:realflagPCA} into a problem over $St(n_k,n)$. We begin by defining the matrices
%     \begin{equation}\label{eq: Ii}
%         (\I_i)_{l,s} = 
%         \begin{cases}
%             1, & l = s \in \{ n_{j-1} + 1, 
%      n_{j-1} + 2, \dots, n_j\} \\
%             0, &\text{ otherwise}\nonumber \\
%         \end{cases}, 
%     \end{equation}
%     \begin{equation}\label{eq: Jj}
%         \text{and }(\mathbf{J}_j)_{l,s} = 
%         \begin{cases}
%             1, & l = s = j \\
%             0, &\text{ otherwise}\nonumber \\
%         \end{cases}.
%     \end{equation}
%     This allows us to rephrase the optimization problem in~\cref{eq:realflagPCA} as
%     \begin{equation}
%         \argmax_{\Y \in St(n_k,n)} \sum_{j=1}^p \sum_{i=1}^k \sqrt{\tr\left( \widetilde{\X} \mathbf{J}_j \widetilde{\X}^T \Y \I_i \Y \right)}.
%     \end{equation}

%     Now, we can write the Lagrangian for this problem with the symmetric matrix of Lagrange multipliers $\bm{\Lambda}$ as
%     \begin{equation}
%         \mathcal{L} (\Y) = \sum_{j=1}^p \sum_{i=1}^k \sqrt{\tr\left( \widetilde{\X} \mathbf{J}_j \widetilde{\X}^T \Y \I_i \Y \right)} + \bm{\Lambda}(\I - \Y^T \Y ).
%     \end{equation}

%     Then, we collect our gradients in the following equations
%     \begin{align*}
%     \begin{aligned}%\label{eq: lagrangian grad}
%         \nabla_{\Y} \mathcal{L}
%         &=  \sum_{j=1}^p \sum_{i=1}^k \frac{\widetilde{\X} \mathbf{J}_j \widetilde{\X}^T \Y \I_i}{\sqrt{\tr \left( \widetilde{\X} \mathbf{J}_j \widetilde{\X}^T \Y \I_i \Y \right)}} - \bm{\Lambda} \Y\\
%          \nabla_{\bm{\Lambda}} \mathcal{L} &=  \I - \Y^T \Y.
%     \end{aligned}
%     \end{align*}

%     With some algebraic manipulation along with the definition of $\mathbf{A}$, we can use $\nabla \mathcal{L} = 0$ to arrive at

%     \begin{equation}
%         \tr(\bm{\Lambda}) \propto \tr \left( \A([\![\Y]\!]) \Y \right).
%     \end{equation}

%     Finally we notice that maximizing $\tr(\bm{\Lambda})$ will maximize~\cref{eq:realflagPCA}.

%     \nate{The final steps in this proof need some polishing.}
    
% \end{proof}

% We now use \cref{prop:IRLSPCA} to define~\cref{alg:realflagPCA}.

% \begin{algorithm}[t]%\label{alg:train}
% \setstretch{1.13}
% \caption{Flagified Robust PCA.}\label{alg:realflagPCA}
%  \textbf{Input}: {Mean centered dataset $\{\widetilde{\x}_j\}_{j=1}^p$}\\
%  \textbf{Output}: Flagified PCA weights $[\![\U]\!] \in \flag(n+1)$ \\[0.25em]
%  Initialize $[\![\U]\!]$\\
%  \While{(not converged)}
%  {
%     Assign $\mathbf{W}_i([\![\U]\!])$ using~\cref{eq: irls weights} (with $\epsilon>0$)\\
%     Update $[\![\U]\!]$ as the solution to~\cref{eq:STrealflagPCA} with $\A([\![\U]\!])$ using Stiefel Riemannian Trust Regions (RTR).
%  }
% \end{algorithm}




% \begin{prop}
%     \nate{Write down DPCP-IRLS in terms of only inner products. I'm looking for an analogous version of~\cref{def: linpga}}
% \end{prop}
% \begin{proof}
%     \nate{Then we have to prove it!}
% \end{proof}

\paragraph{Flagified DPCA}
We flagify the formulations of DPCP to approximate Flagified DPCA.
\begin{dfn}[fDPCP]
    \begin{equation}\label{eq: flagDPCAmin}
        \argmin_{[\![\B]\!] \in \flag(n+1)} \mathbb{E} \left[ \sum_{i=1}^k\| \pi_{\B_i} (\x_j)\|_2 \right].
    \end{equation}
\end{dfn}

\begin{dfn}[fDPCP-Max]
    \begin{equation}\label{eq: flagDPCAmax}
        \argmax_{[\![\B]\!] \in \flag(n+1)} \mathbb{E} \left[ \sum_{i=1}^k \| \x_j  -\pi_{\B_i} (\x_j)\|_2 \right].
    \end{equation}
\end{dfn}


% We have seen that DPCP-IRLS is a procedure that approximates DPCP and consequently provides an approximation of the dual principal components from Dual-PCA. Again, notice that this procedure results in a nested sequence of dual principal components as columns of the matrix $\B = [\vb_1,\vb_2, \dots, \vb_m] \in St(m,n)$ with increasing objective function values. Therefore, we have the nested subspace structure according to the increasing objective function values
% \begin{equation}
%     [\![\B]\!] = [\vb_1] \subset [\vb_1,\vb_2] \subset \cdots \subset [\vb_1,\vb_2, \dots, \vb_m] \subset \R^n.
% \end{equation}
% We can think of DPCP-IRLS, and Dual-PCA in general, as an optimization problem over $ [\![\B]\!] \in \flag(1,2,\dots,m; n)$.



% \begin{dfn}[Flagified DPCP-IRLS]
%     Suppose $\B = [\B_1,\B_2,\dots, \B_k]$ where $\B_i \in \R^{n \times m_i}$.
%     \begin{equation}
%         \argmin_{[\![ \B ]\!] \in \flag(n+1)} \sum_{j=1}^p \sum_{i=1}^k \| \B_i^T \x_j\|_2 .
%     \end{equation}
% \end{dfn}

% Suppose we have two dual principal components with the same objective value, for example, $\vb_1$ and $\vb_2$, then we would like to optimize over $ [\![\B]\!] \in \flag(2,\dots,m; n)$. So, it is worthwhile to generalize our optimization problem for DPCP-IRLS to a concern over the flag manifold of an arbitrary type. In this arena, we can choose the flag type rather than being restricted to $\flag(1,2,\dots,m; n)$.

% We can find an approximation to the flag of dual principal components by solving the ``flagified'' version of DPCP-IRLS. This perspective generalizes Dual PCA by relaxing the nested subspace structure of the dual principal components.
% \begin{equation}
%     \argmin_{[\![ \B ]\!] \in \flag(n+1)} \| \X^T \B \|_{1,2}.
% \end{equation}
% As with flagified PCA, this objective function value is invariant to ordering the columns of $\B$.

% \nate{explain relation to DPCP-IRLS}
% \begin{dfn}[Flagified DPCP-IRLS]
%     Suppose $\B = [\B_1,\B_2,\dots, \B_k]$ where $\B_i \in \R^{n \times m_i}$.
%     \begin{equation}
%         \argmin_{[\![ \B ]\!] \in \flag(n+1)} \sum_{j=1}^p \sum_{i=1}^k \| \B_i^T \x_j\|_2 .
%     \end{equation}
% \end{dfn}
% We can approximate the weights for Flagified DPCP-IRLS using~\cref{alg:realflagDPCP-IRLS}.

% \begin{algorithm}[t]%\label{alg:train}
% \setstretch{1.13}
% \caption{Flagified DPCP-IRLS.}\label{alg:realflagDPCP-IRLS}
%  \textbf{Input}: {Mean centered dataset $\{\widetilde{\x}_j\}_{j=1}^p$}\\
%  \textbf{Output}: Flagified DPCA weights $[\![\B]\!] \in \flag(n+1)$ \\[0.25em]
%  Initialize $[\![\B]\!]$\\
%  \While{(not converged)}
%  {
%     Assign $\mathbf{W}_i([\![\B]\!])$ using~\cref{eq: irls weights} (with $\epsilon>0$)\\
%     Update $[\![\B]\!]$ as the solution to \emph{minimizing the objective function in~\cref{eq:STrealflagPCA}} with $\A([\![\B]\!])$ using Stiefel Riemannian Trust Regions (RTR).
%  }
% \end{algorithm}

\paragraph{Algorithms}
Optimizing over $\flag(1,2,\dots,k;n) = St(k,n)$ recovers L$1$ formulations and optimizing over $\flag(k;n) = Gr(k,n)$ recovers L$2$ formulations.
\begin{table}[H]    \centering
    \begin{tabular}{c|cccc}
           & \multicolumn{2}{c}{RPCA} & \multicolumn{2}{c}{DPCA} \\
           & Max & Min & Max & Min \\
           \hline
        Name & fPCA-L1 & fWPCA & fDPCP-Max & fDPCP\\
        Opt & \cref{eq: flagRPCAmax} & \cref{eq: flagRPCAmin} & \cref{eq: flagDPCAmax} & \cref{eq: flagDPCAmin}
    \end{tabular}
    \label{tab:summary}
    \caption{Flagification of RPCA and DPCA formulations.}
\end{table}

Define the projection matrix $\mathbf{P}([\![\Y]\!], \epsilon)$ as
\begin{equation}\label{eq:P}
    \mathbf{P}([\![\Y]\!], \epsilon)=  \X \W_i \X^T.
\end{equation}
Also define the matrix
\begin{equation}\label{eq:A}
    \mathbf{A}([\![\Y]\!], \epsilon) = \sum_{i=1}^k  \mathbf{P}([\![\Y]\!], \epsilon) \Y \I_i.
\end{equation}
using identity matrices as a function of the flag signature
\begin{equation}\label{eq: Ii}
    (\I_i)_{l,s} = 
    \begin{cases}
        1, & l = s \in \{ n_{j-1} + 1, 
 n_{j-1} + 2, \dots, n_j\} \\
        0, &\text{ otherwise}\nonumber \\
    \end{cases}.
\end{equation}
$\mathbf{P}$ and $\mathbf{A}$ are different depending on our variant of RPCA or DPCA according to changing diagonal weight matrices $\W_i$. For PCA-L1 and DPCP-Max (\cref{eq: flagRPCAmax,eq: flagDPCAmax}) we use
\begin{equation}\label{eq: max_weights}
    (\mathbf{W}_i([\![\Y]\!]))_{jj}  = \max \left( \| \Y_i^T \x_j\|_2, \epsilon \right)^{-1}
\end{equation}
and for WPCA and DPCP (\cref{eq: flagRPCAmin,eq: flagDPCAmin}) we use
\begin{equation}\label{eq: min_weights}
    (\mathbf{W}_i([\![\Y]\!]))_{jj} = \max \left( \| \x_j - \Y_i^T \x_j\|_2, \epsilon \right)^{-1}.
\end{equation}
Certainly, one could optimize these weight functions according to~\cite{peng2022global}.


Now define the functions $f$ and $g$ as
\begin{equation}\label{eq: irls_f}
    f_{[\![\Y]\!], \epsilon}(\Z) = \sum_{i=1}^k \tr\left( \Z^T \mathbf{P}([\![\Y]\!], \epsilon) \Z \I_i  \right),
\end{equation}
\begin{equation}\label{eq: irls_g}
    g_{[\![\Y]\!], \epsilon}(\Z) = \tr\left( \Z^T \mathbf{A}([\![\Y]\!], \epsilon)  \right).
\end{equation}



\begin{prop}\label{prop:IRLSPCA}
    Suppose $[\![\Y]\!] \in \flag(n+1)$ solves~\cref{eq: flagRPCAmax} and $\| \Y_i^T \x_j\|_2 \geq \epsilon$ for all $i$ and $j$. Then $\Y \in St(n_k,n)$ must also solve
    \begin{equation}\label{eq:STrealflagPCA}
        \argmax_{\Z \in St(n_k,n)} f_{[\![\Y]\!], \epsilon}(\Z) 
    \end{equation}
    where $f_{[\![\Y]\!], \epsilon}$ is defined in~\cref{eq: irls_f} and $\W_i$ is defined using~\cref{eq: max_weights}.
\end{prop}
\begin{proof}
    See appendix.
\end{proof}

Similar propositions apply for~\cref{eq: flagRPCAmin,eq: flagDPCAmin,eq: flagDPCAmax} with only a small change in the weight matrices $\W_i$ and are listed in the appendix. For fWPCA and fDPCP (\cref{eq: flagRPCAmin,eq: flagDPCAmin}) we minimize and for fRPCA and fDPCP-Max (\cref{eq: flagRPCAmax,eq: flagDPCAmax}) we maximize. An algorithm to find fWPCA and fDPCP is~\cref{alg: flagified pca f} and an algorithm to find fPCA-L1 and fWPCA is~\cref{alg: flagified pca g}. Varying convergence reliability for these algorithms is summarized in~\cref{tab:summary}. Notice that an iteration of f-IRLS~\cref{alg: flagified pca f} for PCA-L$1$ is weighted fPCA.

\begin{algorithm}[t]
\setstretch{1.13}
\caption{f-IRLS}
\label{alg: flagified pca f}
 \textbf{Input}: {Dataset $\{\x_j\}_{j=1}^p$}\\
 \textbf{Output}: Principal Directions $[\![\Y]\!] \in \flag(n+1)$ \\[0.25em]
 Initialize $[\![\Y]\!]$\\
 \While{(not converged)}
 {
    Assign $\mathbf{W}_i([\![\Y]\!])$ (with $\epsilon>0$)\\
    Update $[\![\Y]\!]$ as optimizer of $f_{[\![\Y]\!], \epsilon}(\Z)$ over $\Z \in St(k,n)$ using Stiefel RTR.
 }
\end{algorithm}

\begin{algorithm}[t]
\setstretch{1.13}
\caption{g-IRLS}
\label{alg: flagified pca g}
 \textbf{Input}: {Dataset $\{\x_j\}_{j=1}^p$}\\
 \textbf{Output}: Principal Directions $[\![\Y]\!] \in \flag(n+1)$ \\[0.25em]
 Initialize $[\![\Y]\!]$\\
 \While{(not converged)}
 {
    Assign $\mathbf{W}_i([\![\Y]\!])$ (with $\epsilon>0$)\\
    Update $[\![\Y]\!]$ as optimizer of $g_{[\![\Y]\!], \epsilon}(\Z)$ over $\Z \in St(k,n)$ using Stiefel Steepest Descent.
 }
\end{algorithm}

\begin{table}[H]    \centering
    \begin{tabular}{c|cccc}
           & fPCA-L1 & fWPCA & fDPCP-Max & fDPCP \\
           \hline
        $f_{[\![ \Y ]\!], \epsilon}$ & - & + & - & +\\
        $g_{[\![ \Y ]\!], \epsilon}$ & + & + & - & -
    \end{tabular}
    \label{tab:summary}
    \caption{Convergence: reliable  is +, unreliable is -.}
\end{table}


\paragraph{Summary} In summary, we use flagification to offer a unified algorithms whose parameters can be changed to solve RPCA and DPCA variants including novel flag versions that traverse between the L$1$ and L$2$ formulations. In general, we find that optimizing $g$ using steepest descent is faster than optimizing $f$ using RTR. 


\subsection{PGA and its robust variants}

Let $\{x_i\}_{i=1}^p$ be a dataset on a Riemannian manifold $M$.\footnote{$M = \R^n$: $\langle \x, \y \rangle = \x^T\y$, $\text{exp}_x(v) = v-x$, and $\text{log}_x(y) = y-x$}

Given a distance $d(\cdot, \cdot)$ on $M$, an average $\mu$ on $M$ is
\begin{equation}\label{eq: manifold_mean}
    \mu = \argmin_{y \in M} \sum_{i=1}^p d(x_i, y)^q.
\end{equation}
When $d(\cdot, \cdot)$ is the geodesic distance and $q=2$, the Karcher mean~\cite{karcher1977riemannian} is the local minimizer of~\ref{eq: manifold_mean} and if there is a global minimizer of~\ref{eq: manifold_mean} we call it the Fr\'echet mean.

Define the $i$th subspace of $T_{\mu}(M)$ as
\begin{equation}
    S_i = \text{span}\{ \bu_1, \bu_2, \dots, \bu_i \}
\end{equation}
and $S_\bu = \text{span}\{ \bu\}$. The projection operator onto the geodesic subspace $H \in M$ is \footnote{$\pi_{H}$ can be any monotonically increasing function of distance.}
\begin{equation}\label{eq:projdef}
\pi_H(x) = \argmin_{z \in H } d(z, x).
\end{equation}
The geodesic subspace of $S \subset T_\mu(M)$ is
\begin{equation}
   H(S) = \{ \text{exp}_{\mu}(\bv) : \bv \in S\}.
\end{equation}
\textit{Note: In contrast to PCA, in PGA, we need to define $H(S)$ because the tangent space and manifold are distinct.}

\begin{dfn}[PGA~\cite{sommer2010manifold}]
The $i$th principal geodesic direction for (exact) PGA is defined as the geodesic starting at the mean with the tangent vector
\begin{equation}\label{eq:pga_max}
\bu_{i} = \argmax_{\substack{ \| \bu \| = 1 \\ \bu \in S_{i-1}^\perp}} \mathbb{E} \left[ d( \mu, \pi_{H(S_\bu)} (x_j))^q \right]
\end{equation}
for $q=2$.
\end{dfn}

As an alternative to maximizing variance~\cref{eq:pga_max}, we can formulate PGA as a minimizer of reconstruction errors (or unexplained variance) as 
\begin{equation}\label{eq:pga_min} 
\bu_{i} = \argmin_{\substack{ \| \bu \| = 1 \\ \bu \in S_{i-1}^\perp}} \mathbb{E} \left[ d( x_j, \pi_{H(S_\bu)} (x_j))^q \right]
\end{equation}
for $q=2$. In Euclidean space, maximizing variances is equivalent to minimizing residuals, but~\cref{eq:pga_max} and~\cref{eq:pga_min} are not equivalent on Riemannian manifolds~\cite{sommer2010manifold}. Notice that PGA results a flag of subspaces of the tangent space of signature $(1,2,\dots,k, \text{dim}(T_{\mu}(M))$:
\begin{equation}
    S_1 \subset S_2 \subset \cdots \subset S_k \subset T_{\mu}(M).
\end{equation}
% Using the minimize distortion definition~\cref{eq:pga_min} and inspiration from Tabaghi~\etal~\cite{tabaghi2023principal}, we say PGA finds a geodesic submanifold of $M$ at $\mu$
% \begin{equation}
%     H_\ast = \argmax_{H \subset M} \mathbb{E} \left[ d( \mu, \pi_{H} (x_j))^2 \right].
% \end{equation}
% Similarly, the maximizing variance definition~\cref{eq:pga_max} results in
% \begin{equation}
%     H_\ast = \argmin_{H \subset M} \mathbb{E} \left[ d( x_j, \pi_{H} (x_j))^2 \right].
% \end{equation}

Let $\w_j = \text{log}_{\mu} x_j$ for $j=1,2,\dots, p$. Fletcher~\etal~\cite{fletcher2004principal} define the $i$th principal geodesic direction from tangent-PGA as the $i$th principal component of $\{\w_j \}_{j=1}^p$. Tangent-PCA is a somewhat reversable transformation. Given $\U = [\bu_{1},\bu_{2}, \dots , \bu_{k}]$ and $\W = [\w_1, \w_2, \dots, \w_p]$, we find the principal components in the tangent space as $ \hat{\W}= \U^T \W $. Then, we approximate the inverse transform as $\U \hat{\W}$ and take $\text{exp}_{\mu}$ to map the columns of this matrix back to the manifold.



\paragraph{Robust PGA (RPGA)}
The Riemannian manifold versions of the RPCA variants PCA-L1 and WPCA are \cref{eq:pga_max} and \cref{eq:pga_min} with $q=1$ and called PGA-L1 and WPGA respectively. Given a manifold valued dataset, we approximate these problems by preforming PCA-L1 and WPCA in the tangent space to the Karcher mean. We will refer to these as tangent space algorithms as Tangent-PCA-L1 and Tangent-WPCA.

\paragraph{Dual PGA (DPGA)}
Given a Riemannian manifold valued dataset, let us compute the Karcher mean, then move the data such that it is all a unit distance from the Karcher mean. Denote such a normalized dataset as $\{x_i\}_{i=1}^p$, Then the Riemannian manifold versions of the DPCA variants DPCP and DPCP-Max are minimizing are~\cref{eq:dpga_min} and \cref{eq:dpga_max} respectively.
\begin{equation}\label{eq:dpga_min}
\bu_{i} = \argmin_{\substack{ \| \bu \| = 1 \\ \bu \in S_{i-1}^\perp}} \mathbb{E} \left[ d( \mu, \pi_{H(S_\bu)} (x_j)) \right]
\end{equation}
\begin{equation}\label{eq:dpga_max} 
\bu_{i} = \argmax_{\substack{ \| \bu \| = 1 \\ \bu \in S_{i-1}^\perp}} \mathbb{E} \left[ d( x_j, \pi_{H(S_\bu)} (x_j)) \right]
\end{equation}
We call~\cref{eq:dpga_min} DPGP and \cref{eq:dpga_max} DPCP-Max. Again, we can approximate these problems by preforming DPCP and DPCP-Max in the tangent space. We refer to these tangent space algorithms as Tangent-DPCP and Tangent-DPCP-Max.


\paragraph{Flagification of PGA and its robust variants}
True flagification of PGA is a difficult task. Instead we will focus on Flagifying the tangent approximations of the true PGA algorithms. To do this, all we do is preform RPCA and DPCA variants in the tangent space using inner products. This results in Tangent-Flagified versions of PCA-L1, WPCA, DPCP, and DPCP-Max called T-fPCA-L1, T-fWPCA, T-fDPCP, and T-fDPCP-Max.




\begin{comment}
\begin{prop}\label{prop:fRPCA}
    Suppose $[\![\Y]\!] \in \flag(n+1)$ solves~\cref{eq: flagRPCAmax} and $\| \Y_i^T \x_j\|_2 \geq \epsilon$ for all $i$ and $j$. Then $\Y \in St(n_k,n)$ must also solve both of
    \begin{equation}\label{eq:fMax}
        \argmax_{\Z \in St(n_k,n)} \left(\sum_{i=1}^k \tr\left( \Z^T \mathbf{P}([\![\Y]\!]) \Z \I_i  \right) \vcentcolon= f_{[\![\Y]\!]}(\Z) \right)
    \end{equation}
    \begin{equation}\label{eq:gMax}
        \argmax_{\Z \in St(n_k,n)} \Big( \tr\left( \Z^T \mathbf{A}([\![\Y]\!])  \right) \vcentcolon= g_{[\![\Y]\!]}(\Z)\Big)
    \end{equation}
    where $\W_i$ is defined using~\cref{eq: max_weights} and $\epsilon = 0$.
\end{prop}


\begin{proof}
    Suppose $[\![\Y]\!] \in \flag(n+1)$ solves~\cref{eq: flagRPCAmax} and $\| \Y_i^T \x_j\|_2 \geq \epsilon$ for all $1\leq i \leq k$ and $1 \leq j \leq p$. Then
    \begin{align}
        \mathbb{E} \left[ \sum_{i=1}^k\| \pi_{\U_i} (\x_j)\|_2 \right] &= \sum_{j=1}^p \sum_{i=1}^k\| \pi_{\U_i} (\x_j)\|_2,\\
        &= \sum_{j=1}^p \sum_{i=1}^k\sqrt{\tr \left( \x_j^T \U_i \U_i^T  \x_j \right)},\\
        &\sum_{j=1}^p \sum_{i=1}^k \sqrt{\tr \left( \U_i^T \x_j  \x_j^T \U_i\right)},\\
        &\sum_{j=1}^p \sum_{i=1}^k \sqrt{\tr \left( \U^T \x_j  \x_j^T \U \I_i \right)}.
    \end{align}
    Now, we can write the Lagrangian for this problem with the symmetric matrix of Lagrange multipliers $\bm{\Lambda}$ as
    \begin{equation}
        \mathcal{L} (\U) = \sum_{j=1}^p \sum_{i=1}^k \sqrt{\tr\left( \x_j \x_j^T \U \I_i \U \right)} + \bm{\Lambda}(\I - \U^T \U ).
    \end{equation}
    Then, we collect our gradients in the following equations
    \begin{align*}
    \begin{aligned}%\label{eq: lagrangian grad}
        \nabla_{\U} \mathcal{L}
        &=  \sum_{j=1}^p \sum_{i=1}^k \frac{\x_j \x_j^T \U \I_i}{\sqrt{\tr \left( \x_j \x_j^T \U \I_i \U \right)}} - \bm{\Lambda} \U\\
         \nabla_{\bm{\Lambda}} \mathcal{L} &=  \I - \U^T \U.
    \end{aligned}
    \end{align*}
    Setting these gradients equal to $0$ results in
\begin{align}
    \sum_{j=1}^p \sum_{i=1}^k \frac{\x_j \x_j^T \U \I_i}{\sqrt{\tr \left( \x_j \x_j^T \U \I_i \U \right)}} &=  \bm{\Lambda} \U, \\
    \sum_{j=1}^p \sum_{i=1}^k \frac{\U^T \x_j \x_j^T \U \I_i}{\sqrt{\tr \left(\x_j \x_j^T \U \I_i \U \right)}} &=  \bm{\Lambda}, \\
    \sum_{j=1}^p \sum_{i=1}^k (\W_i)_{jj} \U^T \x_j \x_j^T \U \I_i &=  \bm{\Lambda}, \\
    \tr\left(\sum_{i=1}^k \U^T \left( \sum_{j=1}^p (\W_i)_{jj} \x_j \x_j^T \right)  \U \I_i\right) &=  \tr(\bm{\Lambda}), \\
    \sum_{i=1}^k \tr\left(\U^T \left( \sum_{j=1}^p (\W_i)_{jj} \x_j \x_j^T \right)  \U \I_i\right) &=  \sum_{i=1}^k\lambda_i, \\
    \sum_{i=1}^k \tr(\U^T \left( \X \W_i \X^T \right)  \U \I_i) &=  \sum_{i=1}^k\lambda_i, \\
    \sum_{i=1}^k \tr(\U^T \mathbf{P}([\![\U]\!])  \U \I_i) &=  \sum_{i=1}^k\lambda_i,\\
    \sum_{i=1}^k \tr(\left( \U^T \A([\![\U]\!])\right) &=  \sum_{i=1}^k\lambda_i.
\end{align}
\nate{Now say something about the optimization.}
\end{proof}

\begin{prop}\label{prop:fWPCA}
    Suppose $[\![\Y]\!] \in \flag(n+1)$ solves fWPCA in~\cref{eq: flagRPCAmax} and $\| \Y_i^T \x_j\|_2 \geq \epsilon$ for all $i$ and $j$. Then $\Y \in St(n_k,n)$ must also solve
     and solve both of~\cref{eq:gMin,eq:fMin}:
    \begin{equation}\label{eq:fMin}
        \argmin_{\Z \in St(n_k,n)} f_{[\![\Y]\!]}(\Z),
    \end{equation}
    \begin{equation}\label{eq:gMin}
        \argmin_{\Z \in St(n_k,n)} g_{[\![\Y]\!]}(\Z),
    \end{equation}
    where $\W_i$ is defined using~\cref{eq: min_weights}.
\end{prop}
\begin{proof}
    \nate{add this}
\end{proof}

\begin{prop}\label{prop:fDPCP}
    Suppose $[\![\Y]\!] \in \flag(n+1)$ solves fWPCA in~\cref{eq: flagRPCAmax} and $\| \Y_i^T \x_j\|_2 \geq \epsilon$ for all $i$ and $j$. Then $\Y \in St(n_k,n)$ must also solve both of~\cref{eq:gMin,eq:fMin} where $g_{[\![\Y]\!]}$ is defined in~\cref{eq: irls_g} and $\W_i$ is defined using~\cref{eq: max_weights}.
\end{prop}
\begin{proof}
    \nate{add this}
\end{proof}

\begin{prop}\label{prop:fWDPCP}
    Suppose $[\![\Y]\!] \in \flag(n+1)$ solves fWPCA in~\cref{eq: flagRPCAmax} and $\| \Y_i^T \x_j\|_2 \geq \epsilon$ for all $i$ and $j$. Then $\Y \in St(n_k,n)$ must also solve both of~\cref{eq:gMax,eq:fMax} where $g_{[\![\Y]\!]}$ is defined in~\cref{eq: irls_g} and $\W_i$ is defined using~\cref{eq: min_weights}.
\end{prop}
\begin{proof}
    \nate{add this}
\end{proof}
\end{comment}



% \begin{algorithm}[t]
% \setstretch{1.13}
% \caption{tRPCA Variants}
% \label{alg: tPDs}
%  \textbf{Input}: {Dataset $\{x_j\}_{j=1}^p \subset M$}\\
%  \textbf{Output}: Robust principal directions $\{\bu_i\}_{i=1}^k \in T_{\mu}(M)$ \\[0.25em]
%  $\mu \leftarrow \text{KarcherMedian}\left(\{x_j\}_{j=1}^p\right)$\\
%  $\w_j \leftarrow \exp_{\mu}(x_j)$\\
 
%  $\{\bu_i\}_{i=1}^k \leftarrow \text{RPCA}\left(\{ \w_j\}_{j=1}^p \right)$\\
% \end{algorithm}


% \begin{algorithm}[t]
% \setstretch{1.13}
% \caption{tWPCA}
% \label{alg: tPDs}
%  \textbf{Input}: {Dataset $\{\x_j\}_{j=1}^p \subset \Man$}\\
%  \textbf{Output}: Weiszfeld principal geodesic directions $\{\bu_i\}_{i=1}^k \in T_{\mu}(\Man)$ \\[0.25em]
%   Initialize $\y \in \Man$\\
%   \While{(not converged)}
%   {
%      $\mu \leftarrow \text{KarcherMedian}\left(\{\x_j\}_{j=1}^p\right)$\\
%      $\w_j \leftarrow \exp_{\mu}(x_j)$\\
%      $\{\bu_i\}_{i=1}^k \leftarrow \text{WPCA}\left(\{ \w_j\}_{j=1}^p \right)$\\
% \end{algorithm}

% \begin{algorithm}[t]
% \setstretch{1.13}
% \caption{tWPCA-L1}
% \label{alg: tWPCA-L1}
%  \textbf{Input}: {Dataset $\{x_j\}_{j=1}^p \subset M$}\\
%  \textbf{Output}: Weiszfeld principal directions $\{\bu_i\}_{i=1}^k \in T_{\mu}(M)$ \\[0.25em]
%  $\mu \leftarrow \text{KarcherMean}\left(\{x_j\}_{j=1}^p\right)$\\
%  $\w_j \leftarrow \exp_{\mu}(x_j)$\\
%  $\{\bu_i\}_{i=1}^k  \leftarrow \text{WPCA}\left(\{ \w_j\}_{j=1}^p \right)$\\
% \end{algorithm}

% \begin{algorithm}[t]
% \setstretch{1.13}
% \caption{tDPCP-L2}
% \label{alg: tDPCP-L2}
%  \textbf{Input}: {Dataset $\{x_j\}_{j=1}^p \subset M$}\\
%  \textbf{Output}: DPCP directions $\{\bu_i\}_{i=1}^k \in T_{\mu}(M)$ \\[0.25em]
%  $\mu \leftarrow \text{KarcherMean}\left(\{x_j\}_{j=1}^p\right)$\\
%  $\w_j \leftarrow \exp_{\mu}(x_j)$\\
%  $\hat{\w_j} \leftarrow \w_j/\|\w_j\|$\\
%  $\{\bu_i\}_{i=1}^k  \leftarrow \text{DPCP-L2}\left(\{ \hat{\w_j}\}_{j=1}^p \right)$\\
% \end{algorithm}

% \begin{algorithm}[t]
% \setstretch{1.13}
% \caption{weighted ftPCA}
% \label{alg: ftPCA}
%  \textbf{Input}: {Dataset $\{x_j\}_{j=1}^p \subset M$, flag signature $(n_1,n_2,\dots, n_k)$}\\
%  \textbf{Output}: Principal Directions $\{\bu_i\}_{i=1}^k \in T_{\mu}(M)$ \\[0.25em]
%  $\mu \leftarrow \text{KarcherMean}\left(\{x_j\}_{j=1}^p\right)$\\
%  $\w_j \leftarrow \exp_{\mu}(x_j)$\\
%  $\{\bu_i\}_{i=1}^k  \leftarrow \text{fPCA}\left(\{ \w_j\}_{j=1}^p, (n_1,n_2,\dots, n_k) \right)$ using \\
% \end{algorithm}


% \begin{algorithm}[t]
% \setstretch{1.13}
% \caption{weighted ftRPCA}
% \label{alg: ftRPCA}
%  \textbf{Input}: {Dataset $\{x_j\}_{j=1}^p \subset M$, flag signature $(n_1,n_2,\dots, n_k)$}\\
%  \textbf{Output}: Principal Directions $\{\bu_i\}_{i=1}^k \in T_{\mu}(M)$ \\[0.25em]
%  $\mu \leftarrow \text{KarcherMean}\left(\{x_j\}_{j=1}^p\right)$\\
%  $\w_j \leftarrow \exp_{\mu}(x_j)$\\
%  $\{\bu_i\}_{i=1}^k  \leftarrow \text{fRPCA}\left(\{ \w_j\}_{j=1}^p, (n_1,n_2,\dots, n_k) \right)$\\
% \end{algorithm}

% \begin{algorithm}[t]
% \setstretch{1.13}
% \caption{weighted ftWPCA}
% \label{alg: ftWPCA}
%  \textbf{Input}: {Dataset $\{x_j\}_{j=1}^p \subset M$, flag signature $(n_1,n_2,\dots, n_k)$}\\
%  \textbf{Output}: Principal Directions $\{\bu_i\}_{i=1}^k \in T_{\mu}(M)$ \\[0.25em]
%  $\mu \leftarrow \text{KarcherMean}\left(\{x_j\}_{j=1}^p\right)$\\
%  $\w_j \leftarrow \exp_{\mu}(x_j)$\\
%  $\{\bu_i\}_{i=1}^k  \leftarrow \text{fRPCA}\left(\{ \w_j\}_{j=1}^p, (n_1,n_2,\dots, n_k) \right)$\\
% \end{algorithm}

% \begin{algorithm}[t]
% \setstretch{1.13}
% \caption{weighted ftDPCP}
% \label{alg: ftDPCP}
%  \textbf{Input}: {Dataset $\{x_j\}_{j=1}^p \subset M$, flag signature $(n_1,n_2,\dots, n_k)$}\\
%  \textbf{Output}: Principal Directions $\{\bu_i\}_{i=1}^k \in T_{\mu}(M)$ \\[0.25em]
%  $\mu \leftarrow \text{KarcherMean}\left(\{x_j\}_{j=1}^p\right)$\\
%  $\w_j \leftarrow \exp_{\mu}(x_j)$\\
%  $\hat{\w_j} \leftarrow \w_j/\|\w_j\|$\\
%  $\{\bu_i\}_{i=1}^k  \leftarrow \text{ftDPCP}\left(\{ \w_j\}_{j=1}^p, (n_1,n_2,\dots, n_k) \right)$\\
% \end{algorithm}

==> content/old_versions/method_old.tex <==
\vspace{-1mm}\section{Methods}\vspace{-1mm}\label{sec:method}



\begin{dfn}[Riemannian Manifold~\cite{lee2006riemannian}]
A \emph{Riemannian manifold} $M$ is a smooth manifold with a positive definite inner product on the tangent space. This inner product defines a Riemannian metric on $M$ and is denoted $\langle \cdot, \cdot \rangle : T_x(M) \times T_x(M) \rightarrow \R$ where $x \in M$ and $T_x(M)$ is the tangent space to $M$ at $x$. Let $\bv \in T_x(M)$ be a tangent vector to $M$ at $x$. The \emph{exponential map} is $\text{exp}_x(\bv) : T_x(M) \rightarrow M$. The \emph{logarithm map} is $\text{log}_x(y) : M \rightarrow T_x(M)$ for $x,y \in M$ and computes the direction from $x$ to $y$\footnote{The logarithm map may not be defined everywhere on $M$.}. A \emph{geodesic} $\gamma : \R \rightarrow M$ parameterizes a path from $\gamma(0) = x$ to $\gamma(1) = y$. The geodesic can be written as $\gamma = \exp_x^{t\log_x(y)}$ for $t \in \R$. $H \in M$ is a geodesic submanifold at $x \in M$ if all geodesics passing through $x$ in $H$ are geodesics in $M$.
\end{dfn}

\begin{dfn}[Flag]\label{def:flagobj}
A \emph{flag} in a finite dimensional vector space $\mathcal{V}$ over a field is a sequence of nested subspaces with \emph{increasing} dimension, each containing its predecessor, \ie the filtration: $\{\emptyset \}=\mathcal{V}_0 \subset \mathcal{V}_1 \subset \dots \subset \mathcal{V}_{k} \subset \mathcal{V}$ with $0=n_0<n_1<\dots<n_k<n_{k+1} = n$ where $\mathrm{dim} \mathcal{V}_i=n_i$ and $\mathrm{dim} \mathcal{V}=n$. We say this flag is of \emph{type} or \emph{signature} $(d_1, \dots ,d_k,d)$. 
%A flag is called \emph{complete} if $d_i = i,\,\forall i$. Otherwise the flag is \emph{incomplete} or \emph{partial}. 

\noindent\textbf{\emph{Notation}:} A flag, $[\![\X]\!]$ of type $(n_1, \dots ,n_k, n)$, is represented by a truncated orthogonal matrix $\X \in \R^{n \times n_k}$. Let $m_j = n_j-n_{j-1}$ for $j=1,2,\dots, k+1$, and $\X_j  \in \R^{n \times m_j}$ for $j=1,2,\dots, k$ whose columns are the $n_{j-1}+1$ to $n_{j}$ columns of $\X$. $[\![\X]\!]$ is
\begin{equation}
     [ \X_1 ]  \subset [\X_1, \X_2] \subset \cdots \subset  [\X_1, \dots, \X_k] = [\X] \subset \R^n. \nonumber
\end{equation}
\end{dfn}

\begin{dfn}[Flag manifold]
The aggregate of all flags of the same type, \ie a certain collection of ordered sets of vector subspaces, admits the structure of manifolds. We refer to this \emph{flag manifold} %with its dimension (type) 
as $\flag(n_1, ..., n_k; n)$ or equivalently as $\flag(n+1)$. The points of $\flag(n+1)$
%$\flag(d_1, ..., d_k; d)$ 
parameterize all flags of type $(n_1, ..., n_k,n)$. 
Flag manifolds generalize Grassmannians~\cite{edelman1998geometry} because $\flag(k; n)=\Gr(k,n)$. $\flag(n+1)$ can be thought of as a quotient of groups ~\cite{ye2022optimization}:
\begin{equation*}
\flag(d+1) = St(d_k, n)/O(m_1) \times O(m_2) \times \cdots \times O(m_{k+1}),
\end{equation*}
where
$St(d_k, n) = \{\X \in \R^{n \times d_k} : \X^T \X = \I \} $ is a Stiefel manifold.
\end{dfn}


\subsection{Principal Component Analysis (PCA)}


Suppose we have $p$ samples (points) with $n$ random variables (features) $\mathcal{X} = \{ \x_i \}_{i=1}^p \subset \R^n$ with a sample mean of $0$. Principal component analysis either maximizes 

\begin{dfn}[PCA~\cite{hotelling1933analysis}]
Define $S_i  = \text{span} (  \mathbf{u}_1, \mathbf{u}_2, \dots, \mathbf{u}_i)$ and  $S_{\mathbf{u}}  = \text{span} \left(  S_{i-1} \cup \{\mathbf{u} \}\right)$. The $i$th principal component is
\begin{equation}\label{eq: generalpca}
\mathbf{u}_{i} = \argmax_{\substack{\mathbf{u}^T \mathbf{u} = 1 \\ \mathbf{u} \in S_{i-1}^\perp}} \mathbb{E} \left[\|  \bm{\x_j} - \pi_{S_{\mathbf{u}}} (\x_j) \|_2^2 \right]
\end{equation}
for $q=2$. Set $q=1$ for the $i$th ``robust'' principal component.
\end{dfn}



\begin{dfn}[PCA~\cite{hotelling1933analysis}]
Define $S_i  = \text{span} (  \mathbf{u}_1, \mathbf{u}_2, \dots, \mathbf{u}_i)$ and  $S_{\mathbf{u}}  = \text{span} \left(  S_{i-1} \cup \{\mathbf{u} \}\right)$. The $i$th principal component is
\begin{equation}\label{eq: generalpca}
\mathbf{u}_{i} = \argmin_{\substack{\mathbf{u}^T \mathbf{u} = 1 \\ \mathbf{u} \in S_{i-1}^\perp}} \mathbb{E} \left[\|  \bm{\mu} - \pi_{S_{\mathbf{u}}} (\x_j) \|_2^2 \right]
\end{equation}
for $q=2$. Set $q=1$ for the $i$th ``robust'' principal component.
\end{dfn}


\begin{dfn}[PCA~\cite{hotelling1933analysis}]
The first $k$ \emph{principal components}\footnote{ These are sometimes called the principal component weights or Empirical Orthogonal Functions.} of $\mathcal{X}$ are the columns of
\begin{equation}\label{eq:pca_opt}
\U = \argmax_{\Y^T \Y = \I} \tr(\Y^T \widetilde{\X} \widetilde{\X}^T \Y).
\end{equation}
\end{dfn}
PCA has been kernelized to improve performance when $p << n$ and better represent non-linear structures in data~\cite{scholkopf1997kernel}. In general, PCA gives us a $k<n$ dimensional embedding of the data as the columns of $\U^T\widetilde{\X} \in \R^{k \times p}$. We can approximately invert PCA by left multiplication by $\U$.

\begin{remark}
    The solution for PCA is the first $k$ left singular vectors of $\widetilde{\X}$, or equivalently, the first $k$ eigenvectors of the mean-centered covariance matrix.  It is standard to order the columns of $\U$ according to their associated explained variances (eigenvalues) $\lambda_i = \bu^T \widetilde{\X} \widetilde{\X}^T \bu_i$. Specifically, we order the principal components as $\lambda_{i} \geq \lambda_{i+1}$. But, in~\cref{eq:pca_opt}, there is no restriction on the ordering of the columns of the matrix $\Y$ because
    \begin{equation}
        \tr(\Y^T \widetilde{\X} \widetilde{\X}^T \Y) = \sum_{i=1}^k \y_i^T \widetilde{\X} \widetilde{\X}^T \y_i.
    \end{equation}
    Since the objective function in~\cref{eq:pca_opt} is invariant to ordering the columns of $\Y$, it is an objective function defined over a Grassmannian.
    
    % The PCA objective function is essentially the sum of the first $k$ eigenvalues of the matrix $\widetilde{\X}\widetilde{\X}^T$. This sum is invariant to the permutations of the columns of $\U$ (eigenvectors) because these permutations only change the order of the eigenvalues of the sum and addition is commutative. Therefore, in this formulation, any ordering of the columns of $\U$ produces the same objective function values. \nate{Elaborate on this and formalize mathematically.}
\end{remark}

\paragraph{Formalizing PCA}
Define the projection operator onto the subspace $H \subset \R^n$ as
\begin{equation}
\pi_H(\x) = \argmin_{\z \in H } d(\z, \x)^2.
\end{equation}
Suppose $H$ has the orthonormal basis $\{u_1,u_2,\dots, u_k\}$ and construct $\U = [u_1,u_2,\dots, u_k]$. Let $\x \in \R^n$ and $d(\z, \x) = \| \z - \x\|$. Then $\pi_H(\x) = \U \U^T(x)$.
% Note: there is no need to distinguish between a geodesic subspace and a subspace of the tangent space. 


\begin{prop}\label{prop: pcaexp}
Define $S_i  = \text{span} (  \mathbf{u}_1, \mathbf{u}_2, \dots, \mathbf{u}_i)$ and  $S_{\mathbf{u}}  = \text{span} \left(  S_{i-1} \cup \{\mathbf{u} \}\right)$. The $i$th principal component is
\begin{equation}\label{eq: generalpca}
\mathbf{u}_{i} = \argmax_{\substack{\mathbf{u}^T \mathbf{u} = 1 \\ \mathbf{u} \in S_{i-1}^\perp}} \mathbb{E} \left[\|  \bm{\mu} - \pi_{S_{\mathbf{u}}} (\x_j) \|^q \right]
\end{equation}
for $q=2$. Set $q=1$ for the $i$th ``robust'' principal component.
\end{prop}
The above definition uses $x^q$ as the function of the distance. We can generally replace $x^q$ with any monotonic function from $\R^+$ to $\R$. Neumayer~\etal~\cite{neumayer2020robust} noted this fact and proposed a provably convergent algorithm for computing robust PCA ($q=1$). Other notions of robust PCA have also been considered~\cite{candes2011robust, vidal2018dpcp}.

\begin{proof}
    See Appendix.
\end{proof}

%\begin{align}
%&\sum_{j=1}^p \x_j^T\mathbf{U}_i \mathbf{U}_i^T \x_j  - 2\bm{\mu}^T \mathbf{U}_i \mathbf{U}_i^T  \x_j \\
%&= \sum_{j=1}^p \x_j^T\mathbf{U}_i \mathbf{U}_i^T \x_j  - 2\bm{\mu}^T \mathbf{U}_i \mathbf{U}_i^T  \x_j 
%\end{align}
%So, this is equivalent to INSERT TANGENT PGA NOTATION.


%\begin{align}
%&\sum_{j=1}^n \x_j^T \mathbf{u}_i \mathbf{u}_i^T \x_j  - 2\bm{\mu}^T \mathbf{u}_i \mathbf{u}_i^T \x_j \\
%&=\tr \left( \mathbf{u}_i^T \left( \sum_{j=1}^n \x_j^T \x_j  - 2\bm{\mu}^T  \x_j \right) \mathbf{u}_i^T \right) \\
%&=\tr \left( \mathbf{u}_i^T \left( \sum_{j=1}^n  -\x_j^T\bm{\mu}   \x_j^T \x_j  - \bm{\mu}^T  \x_j \right) \mathbf{u}_i^T \right) \\
%&=\tr \left( \mathbf{u}_i^T \left( \sum_{j=1}^n (\x_j-\bm{\mu})^T (\x_j  - \bm{\mu})^T \right) \mathbf{u}_i^T \right) 
%\end{align}


\begin{prop}
    Suppose $\{w_j\}_{j=1}^p \subset \R^n$ is a mean centered dataset. Then the $i$th principal component of this dataset is
    \begin{equation}
        u_{i} =\argmax_{\substack{ \| u \| = 1 \\ u \in S_i^\perp}}  \sum_{j=1}^p \left( \langle w_j, u \rangle^2 + \sum_{l=1}^{i-1} \langle w_j, u_l \rangle^2 \right).
    \end{equation}
\end{prop}

\begin{proof}
    See Appendix.
\end{proof}

\subsection{Flagified-PCA}
\nate{I think this makes the utility of Flagified-PCA a bit clearer... Let me know what you think. Please add to the discussion}


We now generalize PCA using flags by grouping eigenvectors using the flag type. The PCA optimization problem~\cref{eq:pca_opt} is naturally an optimization problem on the Stiefel manifold, $St(k,n) := \{ \Y \in \R^{k \times n} \: : \: \Y^T \Y = \I\}$. Suppose $\U = [\bu_1, \bu_2, \dots, \bu_k] \in St(k,n)$ are the $k<n$ principal components of a data matrix $\X$. These are naturally ordered according to their decreasing associated objective function values\footnote{The objective function values are also referred to as explained variances, eigenvalues and squared singular values} in~\cref{prop: pcaexp}. This results in the nested subspace structure
\begin{equation}
    [\![ \U ]\!] = [\bu_1] \subset [\bu_1, \bu_2] \subset \cdots \subset [\bu_1, \bu_2, \dots, \bu_k] \subset \R^n.
\end{equation}
So also can think of $\U \in \flag(1,2,\dots,k; n)$, and consequently, reformulate~\cref{eq:pca_opt} as an optimization problem over $\flag(1,2,\dots,k; n)$. In fact, it is known that $\flag(1,2,\dots,k; n) \cong St(k,n)$\nate{CITE}. However, thinking of $\U$ as $[\![ \U ]\!]$ clearly emphasizes the nested subspace structure of the principal components according to their associated objective function values.

What if we have multiple principal components with the same objective function value? In other words, suppose we have at least one eigenvalue of $\widetilde{\X} \widetilde{\X}^T$ with a geometric multiplicity greater than $1$? For example, assume our dataset has a large variance on some $2$-plane, and all other directions orthogonal to that plane have smaller, unequal variance. Then, the first two principal components, $\bu_1$ and $\bu_2$, will have the same objective function value in~\cref{eq: generalpca}. Any rotation of the two vectors within the plane $\text{span}(\bu_1, \bu_2)$ will still produce the same objective function values. So,~\cref{eq:pca_opt} is no longer a convex optimization problem over $St(k,n)$ because the first two principal components are not unique. However, if we remove $[\bu_1] \subset [\bu_1, \bu_2]$ from the nested subspace structure and consider $[\![ \U ]\!] \in \flag(2,3,\dots, k;n)$ as
\begin{equation}
    [\![ \U ]\!] = [\bu_1, \bu_2] \subset [\bu_1, \bu_2, \bu_3] \subset \cdots \subset [\bu_1, \dots, \bu_k]\subset \R^n.
\end{equation}
Then we have a unique solution to~\cref{eq:pca_opt} over $\flag(2,3,\dots, k;n)$ in place of $St(k,n)$. An example of this is in the Appendix. In practice, it is unlikely that we will have two eigenvectors with the same eigenvalue. However, we can consider two eigenvalues the same as long as $|\lambda_i - \lambda_j| < \epsilon$ for some $\epsilon > 0$.

Motivated by this example, we state a generalization of PCA, which optimizes over flags of a given type.
\begin{dfn}[Flagified-PCA~\cite{pennec2018barycentric}]
A flag of principal components is $[\![ \U ]\!]$:
    \begin{equation}\label{eq:flagpca}
         \argmax_{[\![ \Y ]\!] \in \flag(n+1)} \tr(\Y^T\widetilde{\X}\widetilde{\X}^T \Y).
    \end{equation}
\end{dfn}
Ye~\etal find a solution~\cref{eq:flagpca} using Newton's method on the flag manifold ~\cite{ye2022optimization} and Nguyen offers a method for solving such a problem using RTR on flag manifolds~\cite{nguyen2022closed}. These algorithms produce the same basis vectors for flags regardless of flag type. These basis vectors are different than those found using standard PCA. But, for $[\![ \U ]\!] \in \flag(n_1,n_2,\dots,n_k,n)$ that solves~\cref{eq:flagpca} using either Newton's method or RTR, the column space of $\U_{:,:n_k}$ is the same as the span of the first $n_k$ principal components. This is because the objective function in~\cref{eq:flagpca} is invariant to ordering the columns of $\Y$.

Variants on flagified PCA that maximize $\tr(\Y^T\widetilde{\X}\widetilde{\X}^T \Y)^q$ over $\flag(n+1)$ are coined ``nonlinear eigenflags'' and are difficult to solve for $q=2$~\cite{ye2022optimization}. Yet, methods from Mankovich~\etal can be adapted to solve such problems, especially for $q = 1/2$.

Although flagification appears to add little information to PCA, it provides a general interpretation of the principal components where we impose only a nested structure of principal subspaces in which the subspace dimension increases depending on flag type. Overall, flagification is a process that allows us to go ahead and generalize other dimensionality reduction algorithms that provide us with a sequence of nested subspaces.


% We now generalize PCA using flags. ~\cite{pennec2018barycentric} has shown that PCA can be seen as an optimization on flag manifolds. However, Pennec lacked an algorithm to perform this optimization. This gap has been filled by ~\cite{ye2022optimization}. 

% \paragraph{Making PCA an actual flag problem.}
% We can change this function into an actual problem over the flag manifold if we require the objective function to be dependent on the columns of $\Y$. We do this as one of the following optimization problem
% \begin{equation}
%      \argmax_{[\![ \Y ]\!] \in \flag(n+1)} \sum_{j=1}^k \sqrt{\tr(\Y_j^T\widetilde{\X}\widetilde{\X}^T \Y_j)}.
% \end{equation}

% If we remove the square roots from either problem, we recover the standard Flagified PCA problem. This is almost robust PCA by Neumayer~\etal~\cite{neumayer2020robust} and is very close to the chordal flag median optimization problem \nate{CITE}.


% \nate{This method is a silly idea because it is costly and could just be accomplished by multiplying a matrix of PCs by a block diagonal matrix with $i$ blocks in $SO(m_i)$.}
% \tolga{Yes, but it gives us a 'perspective' to go ahead and flagify other things, which would be useful. We can mention that although silly, this is an important stepping stone.}
% \nate{I re-structured this section and added a last paragraph about the flagification perspective. Let me know what you think. }

\paragraph{Flagified Robust PCA}

For flagified PCA to respect the nested structure of flags, we must embed the flag structure into the optimization problem. As a maximization problem, we have
\begin{equation}\label{eq:realflagPCA}
    \argmax_{[\![\Y]\!] \in \flag(n+1)} \sum_{j=1}^p \sum_{i=1}^k \| \Y_i^T \widetilde{\x}_j\|_2.
\end{equation}
\nate{Check convexity. Over reals and flag.}

\footnote{We can generalize this to $\| \cdot \|_2^q$ for $q \in (0,2)$}
Let $\widehat{\x}_j = \x_j/\| \x_j \|_2$. Then a similar optimization problem is
\begin{equation}\label{eq:medianflagPCA}
    \argmin_{[\![\Y]\!] \in \flag(n+1)} \sum_{j=1}^p \sum_{i=1}^k \sqrt{1-\widehat{\x}_j^T \Y_i \Y_i^T \widehat{\x}_j}.
\end{equation}
If $\widetilde{\x}_j = \widehat{\x}_j$ for all $j$, then these problems have the same optimizers. Otherwise, the optimizers are not necessarily the same. \cref{eq:realflagPCA} is the most natural version of Flagified PCA, whereas~\cref{eq:medianflagPCA} resembles the chordal flag median from~\cite{mankovich2023chordal}.

We can approximate~\cref{eq:realflagPCA} with an IRLS (Iteratively Reweighted Least Squares) framework where an iteration solves a weighted Stiefel manifold optimization problem. The optimization problem in~\cref{eq:realflagPCA} and algorithm derived from~\cref{prop:IRLSPCA} provides a generalization of a problem similar to what is investigated in Weiszfeld-PCA~\cite{neumayer2020robust}. We can consider a flagified version of Weiszfeld-PCA
\begin{equation}
    \argmin_{[\![\Y]\!] \in \flag(n+1)} \sum_{j=1}^p \sum_{i=1}^k \| (\I-\Y_i\Y_i^T)\widetilde{\x}_j\|_2.
\end{equation}

Define the matrix $\A$ as
\begin{equation}\label{eq:A}
    \A([\![\Y]\!])=  \begin{bmatrix}
                \Y_1^T \widetilde{\X}^T \mathbf{W}_1([\![\Y]\!]) \widetilde{\X}\\
                \Y_2^T \widetilde{\X}^T \mathbf{W}_2([\![\Y]\!]) \widetilde{\X}\\
                \vdots\\
                \Y_{n_k}^T \widetilde{\X}^T \mathbf{W}_{n_k}([\![\Y]\!]) \widetilde{\X}
        \end{bmatrix}.
\end{equation}
$\mathbf{W}_i([\![\Y]\!])$ is a diagonal matrix whose $j$th diagonal entry is
\begin{equation}\label{eq: irls weights}
    (\mathbf{W}_i([\![\Y]\!]))_{jj} = \frac{1}{\max \left( \| \Y_i^T \widetilde{\x}_j\|_2, \epsilon \right)},
\end{equation}
with $\epsilon = 10^{-8}$.
\nate{Try different functions for weights...}

\begin{prop}\label{prop:IRLSPCA}
    Suppose $[\![\Y]\!] \in \flag(n+1)$ solves~\cref{eq:realflagPCA} and $\| \Y_i^T \x_j\|_2 \geq \epsilon$ for all $i$ and $j$. Then $\Y \in St(n_k,n)$ must also solve
    \begin{equation}\label{eq:STrealflagPCA}
        \argmax_{\Y \in St(n_k,n)} \tr \left( \A([\![\Y]\!]) \Y \right)
    \end{equation}
    where $\A$ is defined in~\cref{eq:A}.
\end{prop}

\begin{proof}
    First, we will translate~\cref{eq:realflagPCA} into a problem over $St(n_k,n)$. We begin by defining the matrices
    \begin{equation}\label{eq: Ii}
        (\I_i)_{l,s} = 
        \begin{cases}
            1, & l = s \in \{ n_{j-1} + 1, 
     n_{j-1} + 2, \dots, n_j\} \\
            0, &\text{ otherwise}\nonumber \\
        \end{cases}, 
    \end{equation}
    \begin{equation}\label{eq: Jj}
        \text{and }(\mathbf{J}_j)_{l,s} = 
        \begin{cases}
            1, & l = s = j \\
            0, &\text{ otherwise}\nonumber \\
        \end{cases}.
    \end{equation}
    This allows us to rephrase the optimization problem in~\cref{eq:realflagPCA} as
    \begin{equation}
        \argmax_{\Y \in St(n_k,n)} \sum_{j=1}^p \sum_{i=1}^k \sqrt{\tr\left( \widetilde{\X} \mathbf{J}_j \widetilde{\X}^T \Y \I_i \Y \right)}.
    \end{equation}

    Now, we can write the Lagrangian for this problem with the symmetric matrix of Lagrange multipliers $\bm{\Lambda}$ as
    \begin{equation}
        \mathcal{L} (\Y) = \sum_{j=1}^p \sum_{i=1}^k \sqrt{\tr\left( \widetilde{\X} \mathbf{J}_j \widetilde{\X}^T \Y \I_i \Y \right)} + \bm{\Lambda}(\I - \Y^T \Y ).
    \end{equation}

    Then, we collect our gradients in the following equations
    \begin{align*}
    \begin{aligned}%\label{eq: lagrangian grad}
        \nabla_{\Y} \mathcal{L}
        &=  \sum_{j=1}^p \sum_{i=1}^k \frac{\widetilde{\X} \mathbf{J}_j \widetilde{\X}^T \Y \I_i}{\sqrt{\tr \left( \widetilde{\X} \mathbf{J}_j \widetilde{\X}^T \Y \I_i \Y \right)}} - \bm{\Lambda} \Y\\
         \nabla_{\bm{\Lambda}} \mathcal{L} &=  \I - \Y^T \Y.
    \end{aligned}
    \end{align*}

    With some algebraic manipulation along with the definition of $\mathbf{A}$, we can use $\nabla \mathcal{L} = 0$ to arrive at

    \begin{equation}
        \tr(\bm{\Lambda}) \propto \tr \left( \A([\![\Y]\!]) \Y \right).
    \end{equation}

    Finally we notice that maximizing $\tr(\bm{\Lambda})$ will maximize~\cref{eq:realflagPCA}.

    \nate{The final steps in this proof need some polishing.}
    
\end{proof}

We now use \cref{prop:IRLSPCA} to define~\cref{alg:realflagPCA}.

\begin{algorithm}[t]%\label{alg:train}
\setstretch{1.13}
\caption{Flagified Robust PCA.}\label{alg:realflagPCA}
 \textbf{Input}: {Mean centered dataset $\{\widetilde{\x}_j\}_{j=1}^p$}\\
 \textbf{Output}: Flagified PCA weights $[\![\U]\!] \in \flag(n+1)$ \\[0.25em]
 Initialize $[\![\U]\!]$\\
 \While{(not converged)}
 {
    Assign $\mathbf{W}_i([\![\U]\!])$ using~\cref{eq: irls weights} (with $\epsilon>0$)\\
    Update $[\![\U]\!]$ as the solution to~\cref{eq:STrealflagPCA} with $\A([\![\U]\!])$ using Stiefel Riemannian Trust Regions (RTR).
 }
\end{algorithm}








\subsection{Dual-PCA (DPCA)}
\tolga{I would write here sth about what outliers are, why treating them is important, and why this particularly chosen way is useful. Or outliers can sit at the heart of our paper and deserve a seat in the intro.} \nate{I added some words and did light editing. See the paragraphs below.}
Outliers of a dataset are generally considered data that significantly deviate from the general pattern of the dataset. Points in the dataset that are not outliers will be called inliers. If we have a dataset with many outlier points, the directions of maximum variance (detected by PCA) may represent these outliers than the actual dataset. Therefore, we seek methods for dimensionality reduction that capture a space containing only the dataset's inliers.

Our model for data with inliers and outliers is the data matrix with $p$ samples of $n$ features: $\X =  [\textbf{A}, \mathbf{B}] \mathbf{P}   \in \R^{n \times p}$. The columns of $\textbf{A}$ and $\mathbf{B}$ are inliers and outliers, respectively. We assume there are more inliers than outliers. $\mathbf{P}$ is a permutation matrix. We assume the samples live on the unit sphere, namely, $\{\x_1, \x_2,\dots, \x_p\} \in \mathbb{S}^{n-1}$. DPCA seeks a subspace $S_\ast = \text{span}\{ \vb_1,  \vb_2, \dots,  \vb_k\}$ so that $S_\ast^\perp$ contains the most inliers (e.g., columns of $\A$). So, we seek vectors, namely $\{\vb_1,  \vb_2, \dots,  \vb_k\}$, that are as orthogonal as possible to the span of the inliers.

\begin{dfn}[DPCA~\cite{vidal2018dpcp}]
    Let $S_i = \text{span} \{ \vb_1,  \vb_2, \dots,  \vb_i \}$. The $i$th dual principal component is
    \begin{equation}
        \vb_{i} =  \argmin_{\substack{\| \vb \| = 1 \\ \vb \in S_{i-1}^\perp}} \| \X^T \vb \|_0.
    \end{equation}
\end{dfn}

\begin{dfn}[Dual Principal Component Pursuit~\cite{vidal2018dpcp}]
    Dual Principal Component Pursuit (DPCP) is a relaxation of Dual PCA.
    \begin{equation}
        \vb_{i} =  \argmin_{\substack{\| \vb \| = 1 \\ \vb \in S_{i-1}^\perp}} \| \X^T \vb \|_1.
    \end{equation}
\end{dfn}
This is the dual formulation of principal component pursuit from robust PCA~\cite{candes2011robust}.


\begin{prop}\label{prop:dpcphopes}
    % \nate{We need some sort of proposition that relates Dual PCA to expected values or a linearized version.}\\
    Let $\{\x_i\}_{i=1}^p \subset \R^n$ and $\hat{\x}_i =  \x_i / \| \x_i \|$. DPCP is equivalent to
    \begin{equation}
        \vb_{i} = \argmin_{\substack{ \| \vb \| = 1 \\ \vb \in S_{i-1}^\perp}}  \mathbb{E}  \left[ \langle  \hat{\x}_i, \pi_{S_b} (\hat{\x}_i) \rangle^{1/2} \right].
    \end{equation}
\end{prop}
\begin{proof}
    See appendix.
\end{proof}


\begin{dfn}[DPCP-IRLS~\cite{vidal2018dpcp}]
    DPCP-IRLS (Iteratively Reweighted Least Squares) solves an approximation of DPCP: 
    \begin{equation}
        \argmin_{\B^T \B = \I } \| \X^T \B \|_{1,2}.
    \end{equation}
    $\| \X^T \B \|_{1,2}$ denotes the sum of the Euclidean norms of the rows of $\X^T \B$. 
\end{dfn}
DPCP-IRLS is solved by running an IRLS algorithm~\cite{vidal2018dpcp}. A general Grassmannian realization of DPCP-IRLS, along with a ``flagified'' version of this realization, is in~\cref{sec:grassdpcp}.

\tolga{should we introduce $1\leq q\leq 2$ and minimize $\|\cdot\|_q$ instead? Of course, this slightly deviates from the original problem definition.} \nate{I think it makes the most sense to add a note about other matrix norms rather than change the definition for DPCP-IRLS. See my note below.}

Other matrix norms, e.g., $\| \X^T \B \|_{1,q}$ for any $q \in [1,2]$, can be considered. Specifically, $\| \X^T \B \|_{1,1}$ recovers the optimization for the first $k$ dual principal components for DPCP.

% \begin{prop}
%     \nate{Write down DPCP-IRLS in terms of only inner products. I'm looking for an analogous version of~\cref{def: linpga}}
% \end{prop}
% \begin{proof}
%     \nate{Then we have to prove it!}
% \end{proof}


\subsection{Flagified-Dual-PCA} 
We have seen that DPCP-IRLS is a procedure that approximates DPCP and consequently provides an approximation of the dual principal components from Dual-PCA. Again, notice that this procedure results in a nested sequence of dual principal components as columns of the matrix $\B = [\vb_1,\vb_2, \dots, \vb_m] \in St(m,n)$ with increasing objective function values. Therefore, we have the nested subspace structure according to the increasing objective function values
\begin{equation}
    [\![\B]\!] = [\vb_1] \subset [\vb_1,\vb_2] \subset \cdots \subset [\vb_1,\vb_2, \dots, \vb_m] \subset \R^n.
\end{equation}
We can think of DPCP-IRLS, and Dual-PCA in general, as an optimization problem over $ [\![\B]\!] \in \flag(1,2,\dots,m; n)$.

Suppose we have two dual principal components with the same objective value, for example, $\vb_1$ and $\vb_2$, then we would like to optimize over $ [\![\B]\!] \in \flag(2,\dots,m; n)$. So, it is worthwhile to generalize our optimization problem for DPCP-IRLS to a concern over the flag manifold of an arbitrary type. In this arena, we can choose the flag type rather than being restricted to $\flag(1,2,\dots,m; n)$.

We can find an approximation to the flag of dual principal components by solving the ``flagified'' version of DPCP-IRLS. This perspective generalizes Dual PCA by relaxing the nested subspace structure of the dual principal components.
\begin{equation}
    \argmin_{[\![ \B ]\!] \in \flag(n+1)} \| \X^T \B \|_{1,2}.
\end{equation}
As with flagified PCA, this objective function value is invariant to ordering the columns of $\B$.

\nate{explain relation to DPCP-IRLS}
\begin{dfn}[Flagified DPCP-IRLS]
    Suppose $\B = [\B_1,\B_2,\dots, \B_k]$ where $\B_i \in \R^{n \times m_i}$.
    \begin{equation}
        \argmin_{[\![ \B ]\!] \in \flag(n+1)} \sum_{j=1}^p \sum_{i=1}^k \| \B_i^T \x_j\|_2 .
    \end{equation}
\end{dfn}
We can approximate the weights for Flagified DPCP-IRLS using~\cref{alg:realflagDPCP-IRLS}.

\begin{algorithm}[t]%\label{alg:train}
\setstretch{1.13}
\caption{Flagified DPCP-IRLS.}\label{alg:realflagDPCP-IRLS}
 \textbf{Input}: {Mean centered dataset $\{\widetilde{\x}_j\}_{j=1}^p$}\\
 \textbf{Output}: Flagified DPCA weights $[\![\B]\!] \in \flag(n+1)$ \\[0.25em]
 Initialize $[\![\B]\!]$\\
 \While{(not converged)}
 {
    Assign $\mathbf{W}_i([\![\B]\!])$ using~\cref{eq: irls weights} (with $\epsilon>0$)\\
    Update $[\![\B]\!]$ as the solution to \emph{minimizing the objective function in~\cref{eq:STrealflagPCA}} with $\A([\![\B]\!])$ using Stiefel Riemannian Trust Regions (RTR).
 }
\end{algorithm}






\subsection{Principal Geodesic Analysis (PGA)}
\tolga{In this paper, we follow a gradual-flagification philosophy built on top of earlier definitions. Currently, this cumulative progress is not visible, but we can make it visible. It would be important to keep this in mind while writing.} \nate{Hmmm. I hear you, but I'm not sure its totally clear to me what you mean by this. Perhaps just add more exposition to tie the story together? Maybe this will make more sense once we add an introduction, flush out the related work section, and get .}

Let $\{x_i\}_{i=1}^p$ be a dataset on a Riemannian manifold $M$.\footnote{$M = \R^n$: $\langle \x, \y \rangle = \x^T\y$, $\text{exp}_x(v) = v-x$, and $\text{log}_x(y) = y-x$}

Let $\mu$ be the average of $\{x_i\}_{i=1}^p$ on $M$.\footnote{$\mu$ does not have to be a mean. Any base point on $M$ will do.} Given a distance $d(\cdot, \cdot)$ on $M$, an average is
\begin{equation}
    \mu = \argmin_{y \in M} \sum_{i=1}^p d(x_i, y)^q.
\end{equation}
We generally take $q\in \{1,2\}$. The Karcher mean~\cite{karcher1977riemannian} is the ``canonical'' mean on Riemannian manifolds and provides a recipe for computing the average with respect to the squared geodesic distance. For a table of known manifold means and distances, see~\cref{sec:manmeans} \nate{Actually make this table in the appendix}. 

Define the $i$th subspace of $T_{\mu}(M)$ as
\begin{equation}
    S_i = \text{span}( \bu_1, \bu_2, \dots, \bu_i)
\end{equation}
and $S_\bu = \text{span}\left(  S_{i-1}\cup \{ \bu\} \right) $. The projection operator onto the geodesic subspace $H \in M$ is \footnote{$\pi_{H}$ can be any monotonically increasing function of distance.}
\begin{equation}\label{eq:projdef}
\pi_H(x) = \argmin_{z \in H } d(z, x).
\end{equation}
The geodesic subspace of $S \subset T_\mu(M)$ is
\begin{equation}
   H(S) = \{ \text{exp}_{\mu}(\bv) : \bv \in S\}.
\end{equation}
\textit{Note: In contrast to PCA, in PGA, we need to define $H(S)$ because the tangent space and manifold are distinct.}
\begin{dfn}[PGA~\cite{sommer2010manifold}]
The $i$th principal geodesic direction for (exact) PGA is defined as the geodesic starting at the mean with the tangent vector
\begin{equation}\label{eq:pga_max}
\bu_{i} = \argmax_{\substack{ \| \bu \| = 1 \\ \bu \in S_{i-1}^\perp}} \mathbb{E} \left[ d( \mu, \pi_{H(S_\bu)} (x_j))^q \right]
\end{equation}
for $q=2$. Set $q=1$ for the $i$th ``robust'' principal geodesic.
\end{dfn}
% \nate{Is this transformation reversible in some sense? Is there an inverse to $\pi_H$?}
% \tolga{Hmmm, I'm pesimistic here. Why do we need this? (I mean $\exp$ is reversible, of course, but not the projection onto a vector in the tangent space.}
% \nate{A coworker in Gustau's lab suggested this. I think the idea is as follows: In PCA, we can find the principal components. Project onto them. Then, do an analysis with the principal components. Then, go back to the original high-dimensional space. The question is- can we do the same sort of thing with variations on manifold PCA (e.g., PGA).}


As an alternative to maximizing variance~\cref{eq:pga_max}, we can formulate PGA as a minimizer of reconstruction errors (or unexplained variance) as \tolga{vectors bold or not? May I demand sticking to the notation? otherwise I quickly get confused ;)} \nate{Hehe. All vectors are boldface :)}
\begin{equation}\label{eq:pga_min} 
\bu_{i} = \argmin_{\substack{ \| \bu \| = 1 \\ \bu \in S_{i-1}^\perp}} \mathbb{E} \left[ d( x_j, \pi_{H(S_\bu)} (x_j))^2 \right].
\end{equation}
In Euclidean space, maximizing variances is equivalent to minimizing residuals, but~\cref{eq:pga_max} and~\cref{eq:pga_min} are not equivalent on Riemannian manifolds~\cite{sommer2010manifold}.

Using the minimize distortion definition~\cref{eq:pga_min} and inspiration from Tabaghi~\etal~\cite{tabaghi2023principal}, we say PGA finds a geodesic submanifold of $M$ at $\mu$
\begin{equation}
    H_\ast = \argmax_{H \subset M} \mathbb{E} \left[ d( \mu, \pi_{H} (x_j))^2 \right].
\end{equation}
Similarly, the maximizing variance definition~\cref{eq:pga_max} results in
\begin{equation}
    H_\ast = \argmin_{H \subset M} \mathbb{E} \left[ d( x_j, \pi_{H} (x_j))^2 \right].
\end{equation}




\begin{dfn}[Tangent-PCA]\label{def: linpga}
\tolga{name this as tangent-pca or tangent-pcd ? :)} \nate{changed}
    Let $\w_j = \text{log}_{\mu} x_i$ for $i=1,2,\dots, p$. Fletcher~\etal~\cite{fletcher2004principal} define the $i$th principal geodesic direction from linearized (a.k.a. tangent) PGA is
    \begin{equation}\label{eq:linpga}
    \bu_{i} =\argmax_{\substack{ \| \bu \| = 1 \\ \bu \in S_{
    i-1}^\perp}}  \sum_{j=1}^p \left( \langle \w_j, \bu \rangle^2 + \sum_{l=1}^{i-1} \langle \w_j, \bu_l \rangle^2 \right).
    \end{equation}
\end{dfn}

\textit{Note: Tangent-PCA is invertible because it is essentially PCA on the tangent space. Given $\U = [\bu_{1},\bu_{2}, \dots , \bu_{k}]$ and $\W = [\w_p, \w_p, \dots, \w_p]$, we find the principal components in the tangent space as $ \hat{\W}= \U^T \W $. Then, we approximate the inverse transform as $\U \hat{\W}$ and take $\text{exp}_{\mu}$ to map the columns of this matrix back to the manifold.}


PGA results in nested subspaces of the tangent space and nested geodesic submanifolds:
\begin{equation}
    S_1 \subset S_2 \subset \cdots \subset S_k \subset T_{\mu}(M),
\end{equation}
\begin{equation}
    H(S_1) \subset H(S_2) \subset \cdots \subset H(S_k) \subset M.
\end{equation}

\paragraph{Flagifyied PGA} \nate{Details on the mapping h. Is this the Riemannian metric tensor?} Define $\w_i$ as in~\cref{def: linpga} and let $h: T_\mu(M)\rightarrow \R^N$ be the invertible mapping.
%defined by the Riemannian metric tensor. 
Define the matrix 
\begin{equation}
    \mathbf{H} = [h(\w_1), h(\w_2), \dots, h(\w_p)],
\end{equation}
and the optimization problem
\begin{equation}
[\z_1, \z_2, \dots, \z_k] = \argmax_{\Y^T \Y = \I} \tr(\Y^T \mathbf{H}\mathbf{H}^T \Y).
\end{equation}
This approximates the principle geodesic directions $\{\vb_i\}_{i=1}^k \approx \{ h^{-1}(\z_i)\}_{i=1}^k$. We can also optimize this problem over $\flag(n+1)$:
\begin{equation}
    [\![\z_1, \z_2, \dots, \z_k]\!] = \argmax_{[\![ \Y ]\!] \in \flag(n+1)} \tr(\Y^T \mathbf{H}\mathbf{H}^T \Y).
\end{equation}
This generalizes the structure of the nested geodesic submanifolds according to the flag type.
\tolga{Great! flagification is useful here, no? what's the advantage? Or is this also useful for making a Dual-PGA - which I'm super excited about.} \nate{I re-worded the sentence above to emphasize that this generalized PGA. But, I'm not sure sure what the utility of this is...}
\subsection{Dual PGA}
\nate{Maybe we can translate Dual PCA to riemannian manifolds by thinking about Vidal's geometric picture for dual PCA. For example, normalize data on a manifold to live on a unit distance away from the mean of the data as pre-processing... What follows are some ideas, I'm open to suggestions!}

\paragraph{Dual PGA}
The most natural notion of a Dual PGA geodesic submanifold is a minimizer of explained variance:
\begin{equation}
    \argmin_{H \subset M} \mathbb{E} \left[ d( \mu, \pi_{H} (x_j))^q \right].
\end{equation}
Let $S_i = \text{span} ( b_1, b_2, \dots, b_i)$ and $S_b = \text{span} \left( S_{i-1} \cup \{ b\} \right)$. We can do this by finding a set of dual principal geodesic directions as minimizers of sample variance
\begin{equation}
\vb_{i} = \argmin_{\substack{ \| \vb \| = 1 \\ \vb \in S_{i-1}^\perp}} \mathbb{E} \left[ d( \mu, \pi_{H(S_\vb)} (\x_j))^q \right].
\end{equation}
For $q = 2$, we can linearize this as a minimization of the objective function in~\cref{def: linpga}. Then, the dual principal geodesic directions will be orthogonal to the principal geodesic directions, meaning that linearized Dual PGA and linearized PGA result in the same geodesic submanifolds. We may produce a novel manifold dimensionality reduction algorithm if we do exact Dual PGA or approximate the solution to the Dual PGA with $q=1$. \nate{Should we try this?} \tolga{we should!}

As we did with PCA, we can think of Dual PGA as a maximization of reconstruction error:
\begin{equation}
\vb_{i} = \argmax_{\substack{ \| \vb \| = 1 \\ \vb \in S_{i-1}^\perp}} \mathbb{E} \left[ d( x_j, \pi_{H(S_\vb)} (\hat{x}_j)) \right].
\end{equation}
Again, for a given Riemannian manifold, we are not guaranteed that minimizing explained variance and maximizing reconstruction error produce the same geodesic submanifold.


\paragraph{DPGP}
Let $\w_i = \log_{\mu}(x_i)$ and $\hat{\w}_i = \w_i/\| \w_i \|$. To remain consistent with the Euclidean definition of dual principal components, we define the Dual PGA directions as the solutions to 
\begin{equation}
    \vb_{i} = \argmin_{\substack{ \| \vb \| = 1 \\ \vb \in S_{i-1}^\perp}} \| \bv_{i-1} \|_0
\end{equation}
where the $jth$ entry of $\bv_{i-1}$ is $\langle \w_j, \vb_{i-1} \rangle.$


We approximate Dual PGA directions with the Dual Principal Geodesic Pursuit (DPGP) directions
\begin{equation}
\vb_{i} = \argmin_{\substack{ \| \vb \| = 1 \\ \vb \in S_{i-1}^\perp}} \mathbb{E} \left[ \langle  \hat{\w}_i, \pi_{S_\vb} (\hat{\w}_i) \rangle^{1/2} \right].
\end{equation}
In~\cref{prop:dpcphopes}, we showed that, in Euclidean space, this formulation is equivalent to DPCP.
\nate{think on when we have a negative number in inner product}\\


The $i$th DPGP direction can be approximated using linearized DPGP. Linearized DPGP solves
\begin{equation}
b_{i} = \argmin_{\substack{ \| b \| = 1 \\ b \in S_{i-1}^\perp}}  \sum_{j=1}^p |\langle \hat{w}_j, b \rangle|.
\end{equation}



\paragraph{Flagified Dual PGA}
\nate{Again, maybe we use the Riemannian metric tensor here?} \\
Using the same $h$ from flagifying PGA, we approximate linearized dual PGA by running DPCP-IRLS on the Euclidean embedding of the tangent space. Define $w_i$ as in~\cref{def: linpga} and re-define 
\begin{equation}
    \mathbf{H} = \left[\frac{h(w_1)}{\|h(w_1)\|}, \frac{h(w_2)}{\|h(w_2)\|}, \dots, \frac{h(w_p)}{\|h(w_p)\|}\right],
\end{equation}
and the optimization problem
\begin{equation}
[\z_1, \z_2, \dots, \z_k] = \argmin_{\B^T\B = \I} \| \mathbf{H}^T \B \|_{1,2}.
\end{equation}
This approximates the dual principle geodesic directions $\{\bu_i\}_{i=1}^k \approx \{ h^{-1}(\z_i)\}_{i=1}^k$. We can also optimize this problem over $\flag(n+1)$:
\begin{equation}
    [\![\z_1, \z_2, \dots, \z_k]\!] = \argmin_{[\![ \B ]\!] \in \flag(n+1)} \| \mathbf{H}^T \B \|_{1,2}.
\end{equation}
This generalizes DPCP-IRLS by providing an alternate structure of the nested subspaces of the tangent space and, consequently, the nested geodesic submanifolds according to the flag type.
\tolga{and what problem does this alleviate?}
\nate{ Honestly, not sure... the usefulness of flagification is still uncertain to me.}

==> content/old_versions/method_older.tex <==
\vspace{-1mm}\section{Methods}\vspace{-1mm}\label{sec:method}

\subsection{Basic Geometry of a Flag Manifold}
There are three basic representations for the flag manifold. 
\begin{enumerate}

\item Ma~\etal~\cite{ma2021flag} describe a point on the flag manifold as $[[\mathbf{A}] ]\in \flag(d+1)$ using an special orthogonal matrix $\mathbf{A} \in SO(d)$ where 
\begin{equation*}
[[\mathbf{A}]] = \left\{ \mathbf{A} \mathbf{M}  \: : \:  \mathbf{M}_i \in O(m_i), \: \prod_{i=1}^{k+1} \det (\mathbf{M}_i) = 1 \right\}
\end{equation*}
and $\mathbf{M} = \text{diag}(\mathbf{M}_{m_1}, \dots, \mathbf{M}_{m_{k+1}})$.
This amounts to the following representation for a flag manifold
\begin{equation}
    \frac{SO(d)}{S(O(m_1) \times \cdots \times O(m_{k+1}))}.
\end{equation}

\item On the other hand, ~\cite{helmke1994optimization, pitaval2013flag, nguyen2022closed} represent a flag as $[[\mathbf{B}]] \in \flag(d+1)$ using $\mathbf{B} \in St(m_k, d)$ where
\begin{equation*}
[[\mathbf{B}]] = \left\{ \mathbf{B} \mathbf{N} \: : \: \mathbf{N}_i \in O(m_i) \right\}
\end{equation*}
and $\mathbf{N} = \text{diag}(\mathbf{N}_{m_1}, \dots, \mathbf{N}_{m_{k+1}})$.
This amounts to the following representation for a flag manifold
\begin{equation}
    \frac{St(m_k, d)}{O(m_1) \times \cdots \times O(m_{k})}.
\end{equation}

\item A third representation for a flag is mentioned by~\cite{helmke1994optimization, pitaval2013flag} $[[\mathbf{C}]] \in \flag(d+1)$ where $\mathbf{C} = \text{diag}(\lambda_1 \I_{m_1}, \dots, \lambda_1 \I_{m_{k+1}})$ and 
\begin{equation*}
[[\mathbf{C}]] = \left\{ \mathbf{L}^T \mathbf{C} \mathbf{L} \: : \: \mathbf{L} \in \mathbf{O}(d) \right \}.
\end{equation*}
This \textit{should} be equivalent to $[[\mathbf{D}]] \in \flag(d+1)$ where $\mathbf{D} \in O(d)$, 
\begin{equation*}
[[\mathbf{D}]] = \left\{ \mathbf{D} \mathbf{M}  \: : \:  \mathbf{M}_i \in O(m_i)\right\},
\end{equation*}
and $\mathbf{M} = \text{diag}(\mathbf{M}_{m_1}, \dots, \mathbf{M}_{m_{k+1}})$. The intuition is the common representations of the Grassmannian using either truncated unitary matrices with $k$ columns or rank $k$ projection matrices.

This representation amounts to the following representation for a flag manifold
\begin{equation}
    \frac{O(d)}{O(m_1) \times \cdots \times O(m_{k+1})}.
\end{equation}
    
\end{enumerate}

\vspace{.2in}
All of this information is summarized in~\cref{ye2022optimization} and correspondence between all three representations is realized by introducing a projection matrix representation. Hemlke and Moore~\cite{helmke1994optimization} show that this third representation is diffeomorphic to the representation used by Nguyen~\cite{nguyen2022closed}. Ma~\etal~\cite{ma2021flag} mention that the third representation is common and claim, that the first is equivalent to the third, and the third is more useful for computations with the exponential map.



\subsection{PCA on Flags}
~\cite{pennec2018barycentric} has shown that PCA can be seen as an optimization on flag manifolds. Though, Pennec lacked an algorithm to perform this optimization. This gap has been filled by ~\cite{ye2022optimization}. 

Ye~\etal realize this PCA problem for some covariance matrix $\mathbf{M}$ as
\begin{equation}
    \argmax_{[[\Y]] \in \flag(d+1)} \tr(\Y^T \mathbf{M} \Y).
\end{equation}
Ye~\etal also mention and use their methods to solve the non-linear eigenflag problem
\begin{equation}
    \argmax_{[[\Y]] \in \flag(d+1)} \sum_{i=1}^k \tr(\Y_k^T \mathbf{M} \Y_k)^2
\end{equation}
and mention that it would be hard to solve using matrix calculus.
\textit{We should be able to solve this problem using our IRLS algorithm with different weights.}
\vspace{.2in}

\textit{We can use our methods to solve this version of ``simultaneous PCA:''
\begin{equation}
    \argmax_{[[\Y]] \in \flag(d+1)} \sum_{i=1}^k\tr(\Y_k^T \mathbf{M}_k \Y_k).
\end{equation}
Also, we can consider sums of Procrustes problems like
\begin{equation}
    \argmin_{[[\Y]] \in \flag(d+1)} \sum_{i=1}^k \|\Z_k -   \Y_k^T  \Y_k\mathbf{M} \|_F^s,
\end{equation}
\begin{equation}
    \argmin_{[[\Y]] \in \flag(d+1)} \sum_{i=1}^k \|\Z_k -   \Y_k^T \mathbf{M} \|_F^s,
\end{equation}
\begin{equation}
    \argmin_{[[\Y]] \in \flag(d+1)} \sum_{i=1}^k \|\Z -   \Y_k^T \mathbf{M}_k \|_F^s,
\end{equation}
and
\begin{equation}
    \argmin_{[[\Y]] \in \flag(d+1)} \sum_{i=1}^k \|\Z -   \Y_k^T \Y_k \mathbf{M}_k \|_F^s
\end{equation}
for $s = 1$ or $2$.}\\
\vspace{.1in}

\textit{I think we can also apply this to dictionary learning problems where we simultaneously learn multiple dictionaries at the same time. My Grassmannian average can also be applied to dictionary learning.}

\subsection{Dual PCA on Flags}
\textcolor{blue}{Nate: add background for DPCA}
Dual PCA is relaxed to DPCP-IRLS over $\R^n$ by Vidal~\etal~\cite{vidal2018dpcp}. Suppose we have a data matrix $\X = [\x_1, \x_2, \dots, \x_{d_k}] \in \R^{d \times d_k}$. The simplest realization of DPCP-IRLS optimization problem on flags is
\begin{equation}
    \argmin_{[[\Y]] \in \flag(d+1)} \| \X^T \Y \|_{1,2}.
\end{equation}
\textit{Perhaps we can solve this using an IRLS where we use~\cite{ye2022optimization} to iteratively solve the least squares problem and compare it to using~\cite{ye2022optimization} to solve the original problem.}

\subsection{PGA on Flags}
Let $\{[[\X_i]]\}_{i=1}^p \subset \flag(d+1)$ and take $[[\bm{\mu}]]$ to be a mean of these points. \cite{sommer2010manifold} define the \textbf{first principal geodesic} as the geodesic defined by $[[\bm{\mu}]]$ and the element of the tangent space at $[[\bm{\mu}]]$,  $T_{[[\bm{\mu}]]}$, which solves
\begin{equation}\label{eq:mainPGA}
\argmax_{||\mathbf{v}||=1} \sum_{i=1}^p d([[\bm{\mu}]], \pi_{S_{\mathbf{v}}}([[\X_i]]))^2.
\end{equation}
On the other hand, the \textbf{first exact principal geodesic} comes from 
\begin{equation}\label{eq:mainPGA}
\argmax_{||\mathbf{v}||=1} \sum_{i=1}^p d([[\X_i]], \pi_{S_{\mathbf{v}}}([[\X_i]]))^2.
\end{equation}

We define $S_{\mathbf{v}} = \exp_{[[\bm{\mu}]]}\mathbf{v}$ and 
\begin{equation}
    \pi_S([[\X]]) := \argmin_{[[\mathbf{Z}]]\in S} d([[\mathbf{Z}]], [[\X]]).
\end{equation}
\textit{We can solve this using a single variable, $t$!}

The main PGA optimization problem is approximated by the problem
\begin{equation}\label{eq:approxpga}
\argmax_{||\mathbf{v}|| = 1} \frac{1}{p} \sum_{i=1}^p\langle\log_{[[\bm{\mu}]]}[[\X_i]], \mathbf{v} \rangle.
\end{equation}
\textit{Ideas: 
\begin{enumerate}
    \item What if we just do this for the flag manifold with our means?
    \item What if find a way to use chordal and/or geodesic distance on the Grassmann or flag manifolds and use their respective log and exp maps? Can we do something analogous to~\cite{chakraborty2016efficient} or solve it in our own way?
\end{enumerate}}

Elaborating on (2). We can think of $Z = \{ [[\mathbf{Z}]] \in S_{\mathbf{v}} : || \mathbf{v} || = 1\}$ as the set of all points on the ``unit sphere'' from $[[\bm{\mu}]]$.

Let $d(\cdot, \cdot)$ be the chordal distance on the Grassmann or flag manifold. Then 
\begin{equation*}
    Z = \{ [[\mathbf{Z}]] : d_c([[\bm{\mu}]], [[\mathbf{Z}]]) = 1\}
\end{equation*}
Then we can rephrase 
\begin{equation*}
    \pi_S([[\X]]) \approx \argmin_{[[\mathbf{Z}]]\in Z} d_c([[\mathbf{Z}]], [[\X]]).
\end{equation*}
The PGA optimization problem seeks a set of vectors in the tangent space of a manifold. 
\begin{itemize}
    \item Grassmann manifold tangent space is a subset of skew symmetric matrices
    \item Flag manifold tangent space is a subset of skew symmetric matrices
\end{itemize} 
Also, the exp and log maps for the Grassmann and flag manifolds are in~\cite{edelman1998geometry} and~\cite{ma2021flag} respectively. 


\paragraph{Computing Flagified PCA} \nate{This method is a silly idea because it is costly and could just be accomplished by multiplying a matrix of PCs by a block diagonal matrix with $i$ blocks in $SO(m_i)$.}
We flagify PCA by finding the point on $\flag(n+1)$ that is closest to the first $n_k$ principal components of our data. This mixes the basis vectors that live in the same subspace within the flag. Specifically, we compute all the principal components and store them as the columns of $\Y$. Then we find the point on the flag manifold that is closest to $[\![\Z]\!]$ with respect to the chordal distance.
\begin{equation}\label{eq:stclosept}
    \argmin_{[\![ \Z ]\!] \in \flag(n+1)} d_c([\![\Z]\!], [\![\Y]\!])^2
\end{equation}
This has the obvious solution $[\![ \Z ]\!] = [\![\Y]\!]$. But, we seek a solution that is blind to the order of the columns of $\Z$ according to the type of $\flag(n+1)$. 

We translate $d_c(\cdot, [\![\Y]\!]):\flag(n+1) \rightarrow \R$ to a function that maps $St(n_k, n) \rightarrow \R$:
\begin{align}
    d_c([\![\Z]\!], [\![\Y]\!])^2 &= \sum_{i=1}^{k} m_i - \tr(\Z_i^T \Y_i \Y_i^T \Z_i),\\
    &= \sum_{i=1}^{k} m_i - \tr(\I_i \Z^T \Y_i \Y_i^T \Z).
\end{align}
We define $\I_i$ as
\begin{equation}
    \I_i = \begin{bmatrix}
    0 & 0 & 0  \\
    0 & \I & 0 \\
    0 & 0 & 0 \\
    \end{bmatrix}
    \in \R^{n_k \times n_k}
\end{equation}
where the center block with $\I \in R^{m_i \times m_i}$ is the $n_{i-1}+1$ to $n_i$ rows and columns. Then we solve
\begin{equation}
    \argmin_{\substack{\Z \in St(n_k, n) \\ \Z \neq \Y}} \sum_{i=1}^{k} m_i - \tr(\I_i \Z^T \Y_i \Y_i^T \Z)
\end{equation}
using RTR on $St(n_k, n)$. We approximate the constraint $\Z \neq \Y$ by initializing RTR with $\Z = \I_{:,:n_k}$. 

% We can also do this using the following algorithm:
% \begin{enumerate}
%     \item Compute a mean $[[\bm{\mu}]]$.
%     \item Generate the set of points in the tangent space: 
%     \begin{equation*}
%         \bm{v}_i := \log([[\bm{\mu}]], [[\X_i]])
%     \end{equation*}
%     \item Compute PCA of $\{ \bm{v}_i \}_{i=1}^p$.
%     \item The mean and PCA results define the various principal geodesics.
% \end{enumerate}

\subsection{Dual PGA on Flags}
Let $\bm{\Omega} \in \R^{p \times n}$ be a set of $p$ data points with $n$ features. Let us assume that this dataset in $R^n$ has a set of outliers and inliers (a.k.a. non-outliers). We seek a subspace, $\mathbf{b}^*$, that spans the subspace that is orthogonal to subspace that contains the most inliers of $\bm{\Omega}$. To do this we define
\begin{equation*}
\mathbf{b}^* := \argmin_{\mathbf{b}} || \bm{\Omega} \mathbf{b} ||_0.
\end{equation*}
Now, we seek basis, encoded in the columns of $\mathbf{B}$, for a higher dimensional subspace that is orthogonal to the subspace that contains the most inliers of $\bm{\Omega}$. This can be relaxed, then reformulated as the DPCP-IRLS optimization problem
\begin{equation*}
 \argmin_{\mathbf{B}^T \mathbf{B} = \mathbf{I}} || \bm{\Omega} \mathbf{B} ||_{1,2}.
\end{equation*}
This problem is presented and solved by Tsaskaris \etal \cite{vidal2018dpcp} using an algorithm similar to what is presented by Mankovich \etal \cite{mankovich2022flag}.

\textit{Idea: can we adapt this optimization problem to the Riemannian, Grassmann and/or flag manifold setting and solve it?}

Elaborating. Maybe we just think of this problem as 
\begin{equation*}
\argmin_{||\mathbf{v}||=1} \sum_{i=1}^p d(\bm{\mu}, \pi_{S_{\mathbf{v}}}([[\X_i]])).
\end{equation*}
Then we use a similar approximation and solve it.

\subsection{Topology Dimensionality Reduction and Flags}
\textit{Persistent Homology-based Projection Pursuit}

% \subsection{t-SNE}

\subsection{Dynamic Mode Decomposition}

\subsection{Main Questions}
\begin{enumerate}
    \item Realize PCA as an optimization problem on flag manifolds?
    \item Differentiable flag PCA?
    \item PGA on flag manifolds? Latent space as flags?
    \item Robust PGA using Weiszfeld methods maybe related to Dual PCA and DPCP?
    \item What if we do PGA and just remove the square from the optimization problem?
\end{enumerate}


\subsection{Partial Least Squares (PLS)}
\tolga{I think this is good for a follow-up but for the self-consistency of the paper we focus on PCA variations?} \nate{I agree. One thing at a time. I've moved the PLS discussion to another overleaf. But just FYI: PLS is a dimensionality reduction of two datasets simultaneously. Dual PCA and DPCP are essentially robust versions of PCA. Correctly formulating DPCP on Riemannian manifolds seems pretty hard. But I think PLS might have a simpler realization as a Riemannian manifold problem. See \url{https://digital.library.adelaide.edu.au/dspace/handle/2440/138532}}


\subsection{Applications}
\begin{enumerate}
    \item classification by distance to the first principal geodesic
\end{enumerate}

==> content/old_versions/pca_old.tex <==
\section{Generalizing PCA and Its Robust Variants}
\emph{Principal directions} are the directions where the data varies. We now review and go beyond the celebrated principal component analysis (PCA)~\cite{hotelling1933analysis} algorithm and its variants. In what follows, we present PCA in a generalizing framework, which further yields novel variants.
We consider a set of $p$ centered samples (points with a sample mean of $0$) with $n$ random variables (features) $\mathcal{X} = \{ \x_j \subset \R^n\}_{j=1}^p $ and collect these data in the matrix $\X = [\x_1,\x_2,\ldots,\x_p]$.
\begin{dfn}[PCA~\cite{hotelling1933analysis}]\label{dfn:pca}
PCA aims to linearly transform the data into a new coordinate system, specified by a set of $k < n$ orthonormal vectors $\{\bu_i \in \R^n\}_{j=1}^k$, where (most of) the variation in the data can be described with fewer dimensions than the initial data. 
The $i^\mathrm{th}$ principal direction is obtained either by maximizing variance \cref{eq: maxpca} or minimizing reconstruction error (Eq.~\eqref{eq: minpca}):
\begin{align}\label{eq: maxpca}
\mathbf{u}_{i} &= \argmax_{\substack{\mathbf{u}^T \mathbf{u} = 1, \,\mathbf{u} \in S_i^\perp }} \,\,\,\mathbb{E}_j \left[\|  \pi_{S_{\mathbf{u}}} (\x_j) \|_2^2 \right]\\
\mathbf{u}_{i} &= \argmin_{\substack{\mathbf{u}^T \mathbf{u} = 1,\, \mathbf{u} \in S_{i-1}^\perp}} \mathbb{E}_j \left[\|  \bm{\x_j} - \pi_{S_{\mathbf{u}}} (\x_j) \|_2^2 \right],\label{eq: minpca}
\end{align}
where $\pi_{S_\bu}(\x) := \bu \bu^T \x$, $S_i = \mathrm{span}\{ \bu_1, \bu_2, \ldots, \bu_i \}$, $S_i^\perp$ denotes its orthogonal complement, and $\mathbb{E}_j$ denotes expectation over $j$.
Although these objectives can be achieved jointly~\cite{wang2023max}, in this work, we focus on the more common practice specified above.
Notice that~\cref{eq: maxpca} is equivalent (up to rotation) to solving the following optimization:
\begin{equation}\label{eq: pca_opt_rot}
    \argmax_{\U^T\U = \I} \tr(\U^T \X \X^T \U)
\end{equation}
\end{dfn}
Directions of maximum variance captured by the naive PCA are known to be susceptible to outliers in data. This motivated a body of work devising more robust versions. 
\begin{dfn}[Generalized PCA]\label{dfn:pcagen}
The formulations in~\cref{dfn:pca} can be generalized by using arbitrary $L_p$-norms, $q$-powers, and weighted with real weights $\{w_1,w_2,\ldots, w_p\}$:
% Most robust PCA formulations solve for $\U^\star\in St(n,k)$ using an arbitrary $L_p$-norm via~\cref{eq: maxpca_gen,eq: mindpca_gen}~\cite{kwak2013principal}:
\begin{align}
\U^\star&=\argmax_{\mathbf{U}^T \mathbf{U} = \I} \,\,\mathbb{E}_j \left[ w_j\|  \pi_{S_{\mathbf{U}}} (\x_j) \|_p^q \right],\label{eq: maxpca_gen}\\
\U^\star&=\argmin_{\mathbf{U}^T \mathbf{U} = \I } \,\,\,\mathbb{E}_j \left[w_j\|  \bm{\x_j} - \pi_{S_{\mathbf{U}}} (\x_j) \|_p^q \right],\label{eq: minpca_gen}
\end{align}
where $\pi_{S_\U}(\x) := \U \U^T \x$. Both problems recover PCA up to a rotation when $p=q=2$. When $p \leq 2$ and $ q < 2$, a more \emph{outlier robust} version of PCA is achieved, and two formulations become different. The variance-maximizing (\cref{eq: maxpca_gen}) $q=1$ case is known as \LpRPCA~\cite{kwak2013principal}. Specifically, when $q=p=1$, it recovers \LoneRPCA~\cite{markopoulos2014optimal} and when $q=1$, $p=2$, it recovers \LtwoRPCA~\cite{polyak2017robust}. 
On the other hand, minimizing the reconstruction error  (\cref{eq: minpca_gen}) leads to $L_1$-Weiszfeld PCA (\LoneWPCA)~\cite{neumayer2020robust} for $q=p=1$ and \LtwoWPCA~\cite{ding2006r} for $q=1$, $p=2$. % \nate{There's even more literature on this stuff. Improved algorithms etc... not sure how much detail we should go into here.}
\end{dfn}



% Robust PCA-L1 (RPCA-L1)~\cite{markopoulos2014optimal} solves~\cref{eq: maxpca_gen} for $p=q=1$ and Robust Weiszfeld PCA-L1 (WPCA-L1)~\cite{neumayer2020robust} solves~\cref{eq: minpca_gen} for $p=q=1$. We also propose two new formulations RPCA-L2 and WPCA-L2 which solve ~\cref{eq: maxpca_gen} and ~\cref{eq: minpca_gen} for $p=2,q=1$ respectively.

\paragraph{Generalizing Dual-PCA}
Momentarily assume that the data matrix can be decomposed into inliers $\X_I$ and outliers $\X_O$: $\X =  [\X_I, \X_O] \mathbf{P}$, where $\mathbf{P}$ is a permutation matrix. 
\begin{dfn}[Dual-PCA~\cite{vidal2018dpcp}]\label{dfn:DPCA}
    Assuming the samples live on the unit sphere, $\{\x_i\}_{i=1}^p \in \mathbb{S}^{n-1}$, DPCA seeks a subspace $S_\ast = \mathrm{span}\{ \vb_1,  \vb_2, \ldots,  \vb_k\}$ so that $S_\ast^\perp$ contains the most inliers (e.g., columns of $\X_I$). In other words, we seek vectors $\{\vb_i\}_{i=1}^k$ that are \emph{as orthogonal as possible} to the span of the inliers. This is formalized in the iterative optimization problem
    \begin{equation}~\label{eq: dualpca}
        \vb_{i} =  \argmin_{\| \vb \| = 1, \: \vb \in S_{i-1}^\perp} \| \X^T \vb \|_0.
    \end{equation}    
    When we re-write the maximum variance formulation of the \PCA~optimization in~\cref{eq: maxpca_gen} as the minimization
    (e.g., $\vb_{i} =  \argmin_{\| \vb \| = 1, \: \bu \in S_{i-1}^\perp} \| \X^T \vb \|_2^2$) we see that Dual-\PCA~minimizes a similar objective that is robustified by considering a $0$-norm.
\end{dfn}
\begin{dfn}[Dual Principal Component Pursuit (DPCP)]\label{dfn:DPCP}
Relaxing the $L_0$-norm sparse problem into an $L_1$-norm one turns the DPCA problem into \LoneDPCP~\cite{vidal2018dpcp}. When solved via an $L_2$-relaxed scheme, we recover \LtwoDPCP~ (referred to as DPCP-IRLS by~\cite{vidal2018dpcp}). 
\end{dfn}
\begin{dfn}[Dual PCA Generalizations]\label{dfn: genDualPCA}
In general, we can think of~\cref{dfn:DPCA,dfn:DPCP} as variance-minimizing (\cref{eq: mindpca_gen}) and reconstruction-error-maximizing (\cref{eq: maxdpca_gen}), respectively: %optimizations~\cref{eq: mindpca_gen,eq: maxdpca_gen}:
\begin{align}\label{eq: mindpca_gen}
\B^\star&=\argmin_{\B^T \B = \I} \,\mathbb{E}_j \left[\|  \pi_{S_{\B}} (\x_j) \|_p^q \right]\\
\B^\star&=\argmax_{\B^T \B = \I } \mathbb{E}_j \left[\|  \bm{\x_j} - \pi_{S_{\B}} (\x_j) \|_p^q \right].\label{eq: maxdpca_gen}
\end{align}
Using~\cref{eq: mindpca_gen}, we recover \LoneDPCP~with $p=q=1$ and \LtwoDPCP~with $p=2$ and $q=1$.
\end{dfn}

\begin{remark}[New DPCP Variants]
    Two other possibilities optimize~\cref{eq: maxdpca_gen} when $p=q=1$ and $p=2,q=1$. We call these methods $L_p$-Weiszfeld DPCPs (WDPCPs), specifically, \LoneWDPCP~and \LtwoWDPCP~for different $p$ values.
\end{remark}

\paragraph{Extension to Riemannian manifolds}
%\tolga{Write about PGA, RPGA, DPGA, DPGP, WDPGP and etc.} 
Principal geodesic analysis (PGA)~\cite{fletcher2004principal} generalizes 
PCA for describing the variability of data $\{\x_i\in\Man\}_{i=1}^p$ on a Riemannian manifold $\Man$, induced by the \emph{geodesic distance} $d(\cdot, \cdot):\Man\times\Man\to\R_+$. To this end, PGA first requires a manifold-mean:
\begin{equation}\label{eq: manifold_mean}
    \bmu = \argmin_{\y \in \Man} \mathbb{E}_j \left[ d(\x_j, \y)^2 \right],
\end{equation}
where the local minimizer is called the \emph{Karcher mean} and if there is a global minimizer, it is called the \emph{Fr\'echet mean}. A more robust version of the Karcher mean is the \emph{Karcher median} which minimizes $\mathbb{E}_j \left[ d(\x_j, \y) \right]$ and can be estimated by running a Weiszfeld-type algorithm~\cite{aftab2014generalized}.
Next, PGA 
% defines the 
uses geodesics rather than lines, locally the shortest path between two points, as one-dimensional subspaces.
\begin{dfn}[PGA~\cite{fletcher2003statistics,sommer2010manifold}]
The $i^\mathrm{th}$ principal geodesic for (exact) PGA is defined as $\gamma_i(t) = \Exp_{\bmu}(\bu_i t)$
%the unique geodesic starting at the mean with the tangent vector 
constructed either by maximizing variance (\cref{eq:pga_max}) or by minimizing reconstruction error (or unexplained variance) (\cref{eq:pga_min}):
\begin{align}
\bu_{i} &= \argmax_{ \| \bu \| = 1,\, \: \bu \in S_{i-1}^\perp} \mathbb{E}_j \left[ d( \bmu, \pi_{\SubMan(S_\bu)} (\x_j))^2 \right]\label{eq:pga_max}\\
\bu_{i} &= \argmin_{ \| \bu \| = 1,\, \: \bu \in S_{i-1}^\perp} \mathbb{E}_j \left[ d(\x_j, \pi_{\SubMan(S_\bu)} (\x_j))^2 \right],\label{eq:pga_min} 
\end{align}
where $S_\bu = \mathrm{span}\{ \bu\}$, the $i^\mathrm{th}$ subspace of $\TmuM$, and
\begin{equation}
    S_i = \mathrm{span}\{ \bu_1, \bu_2, \ldots, \bu_i \}.
\end{equation}
The projection operator onto $\SubMan \in \Man$, the geodesic submanifold of $S \subset \TmuM$, is \footnote{$\pi_{H}$ can use any monotonically increasing function of distance on $\Man$.}
\begin{equation}\label{eq:projdef}
\pi_{\SubMan}(\x) = \argmin_{\z \in \SubMan } d(\z, \x).
\end{equation}
where $\SubMan(S) = \{ \Exp_{\bmu}(\bv) : \bv \in S\}$.
\end{dfn}
\begin{remark}
    In contrast to PCA, PGA needs to explicitly define $\SubMan(S)$ because the tangent space and manifold are distinct. While in Euclidean space, maximizing variances is equivalent to minimizing residuals,~\cref{eq:pga_max} and~\cref{eq:pga_min} are not equivalent on Riemannian manifolds~\cite{sommer2010manifold}. PGA results in a flag of subspaces of the tangent space of type $(1,2,\ldots,k; \text{\emph{dim}}(T_{\bmu}(\Man))$ in~\cref{eq: tangent_flag} along with an increasing sequence of geodesic submanifolds in~\cref{eq:subman_flag}
    \begin{align}
        &S_1 \subset S_2 \subset \cdots \subset S_k \subset T_{\bmu}(\Man),\label{eq: tangent_flag}\\
        &\SubMan(S_1) \subset \SubMan(S_2) \subset \cdots \subset \SubMan(S_k) \subset \Man.\label{eq:subman_flag}
    \end{align} 
    Additionally, a set of principal directions, $\{\bu_i\}_{i=1}^k$, form a (totally) geodesic submanifold $\SubMan(S_k) \subseteq \Man$ as long as geodesics in $\SubMan(S_k)$ are carried to geodesics in $\Man$~\cite{tabaghi2023principal}.
\end{remark}

\noindent Similar to~\cref{dfn:pcagen}, we now generalize PGA.
\begin{dfn}[PGA Generalizations]\label{dfn:pgagen}
Let $\{w_j\}_{j=1}^p \subset \R$ denote a set of weights. The weighted principle geodesic is $\gamma_i(t) = \Exp_{\bmu}(\bu_it)$ where $\bu_i$ maximizes / minimizes:
\begin{align}
\bu_{i} &= \argmax_{\substack{ \| \bu \| = 1,\, \bu \in S_{i-1}^\perp}} \mathbb{E}_j \left[ w_jd( \bmu, \pi_{\SubMan(S_\bu)} (\x_j))^q \right]\label{eq:wt_pga_max}\\
\bu_{i} &= \argmin_{\substack{ \| \bu \| = 1,\, \bu \in S_{i-1}^\perp}} \mathbb{E}_j \left[ w_jd(\x_j, \pi_{\SubMan(S_\bu)} (\x_j))^q \right],\label{eq:wt_pga_min} 
\end{align}
This recovers PGA when $q=2$ and $w_j = 1$ for all $j$.
%\tolga{I really like using Tabaghi~\etal~\cite{tabaghi2023principal} to write them thru the geodesic submanifolds. Can we do this?} \nate{ I think you mean just to add geodesic submanifolds to the definition. I did that, taking the definition from~\cite{tabaghi2023principal}. I also mentioned an increasing sequence of submanifolds in the remark.}
\end{dfn}

\begin{remark}[Tangent-PCA (\TPCA)~\cite{fletcher2004principal}]\label{rem:TPCA}
    PGA is known to be computationally expensive to compute except on a few simple manifolds~\cite{tabaghi2023principal,said2007exact}. 
    As a remedy, Fletcher~\etal~\cite{fletcher2004principal} leverage the Euclidean-ness of the tangent space to define principal geodesics as $\gamma(t) = \Exp_{\bmu}(t\bu_i)$ where $\{\bu_i\}_{i=1}^k$ are the principal components of $\{\Log_{\bmu} \x_j \}_{j=1}^p$. This approximation, known as \emph{Tangent-PCA}, and we will later
    %can be 
    approximately invert it to reconstruct data on $\Man$ by (i) using principal directions to reconstruct the data on $T_{\bmu}(\Man)$, then (ii) mapping the reconstruction to $\Man$ using $\Exp_{\bmu}(\cdot)$. 
\end{remark}

% Again, we can formulate weighted versions of these algorithms with weights $\{w_j\}_{j=1}^p \in \R$. For example, weighted PGA solves \tolga{We never formulated this for PCA.}
% \begin{equation}\label{eq:wt_pga_max}
% \bu_{i} = \argmax_{\substack{ \| \bu \| = 1 \\ \bu \in S_{i-1}^\perp}} \mathbb{E} \left[ w_j d( \mu, \pi_{H(S_\bu)} (x_j))^q \right]
% \end{equation}
% Using the minimize distortion definition~\cref{eq:pga_min} and inspiration from Tabaghi~\etal~\cite{tabaghi2023principal}, we say PGA finds a geodesic submanifold of $M$ at $\mu$
% \begin{equation}
%     H_\ast = \argmax_{H \subset M} \mathbb{E} \left[ d( \mu, \pi_{H} (x_j))^2 \right].
% \end{equation}
% Similarly, the maximizing variance definition~\cref{eq:pga_max} results in
% \begin{equation}
%     H_\ast = \argmin_{H \subset M} \mathbb{E} \left[ d( x_j, \pi_{H} (x_j))^2 \right].
% \end{equation}

\begin{prop}[Robust PGAs (RPGA \& WPGA)]
    Setting $1\leq q<2$, gives us novel, robust formulations of the PGA problem (RPGA and WPGA) defined in~\cref{dfn:pgagen}, which we will solve in the unifying flag framework we provide.     
    While general robust manifold-optimizers such as \emph{robust median-of-means}~\cite{lin2020robust} can be used to implement RPGA and WPGA, to be consistent with \TPCA, we will approximate these problems by performing RPCA and WPCA in the tangent space of the robust Karcher median (removing the square in~\cref{eq: manifold_mean}).
    %Karcher mean (replacing the square in~\cref{eq: manifold_mean} by $q$) or Karcher median. 
    We will refer to these tangent space versions as tangent \RPCA~ (\TRPCA) and tangent \WPCA~ (\TWPCA). 
\end{prop}

% \noindent \tolga{What about Weiszfeld algorithms on manifolds as in~\cite{aftab2014generalized}?} \nate{I've added this to manuscipt.}
\noindent We are now ready to formulate novel, dual versions of PGA.
\begin{prop}[Dual PGA (DPGA)]
    Given a dataset on a Riemannian manifold, we define dual robust principal directions, analogous to DPCA (\cref{dfn: genDualPCA}):
    \begin{align}\label{eq:dpga_min}
\vb_{i} &= \argmin_{\substack{ \| \vb \| = 1 \,,\, \vb \in S_{i-1}^\perp}} \mathbb{E}_j \left[ w_j d( \bmu, \pi_{H(S_\vb)} (\x_j))^q \right]\\
\vb_{i} &= \argmax_{\substack{ \| \vb \| = 1 \,,\, \vb \in S_{i-1}^\perp}} \mathbb{E}_j \left[ w_j d( \x_j, \pi_{H(S_\vb)} (\x_j))^q \right].\label{eq:dpga_max} 
\end{align}
We refer to these novel principal directions as \DPGP~ (\cref{eq:dpga_min}) and \WDPGP~ (\cref{eq:dpga_max}). Again, we can approximate these problems by performing DPCP and WDPCP in the tangent space, resulting in the tractable algorithms of tangent DPCP (\TDPCP) and tangent WDPCP (\TWDPCP).
\end{prop}

\begin{remark}[Normalization]
    Classical DPCA works with datasets normalized to the unit sphere. Our tangent formulations of DPCP variations do not perform this preprocessing on the tangent space.
\end{remark}
{We summarize all the PCA methods as well as our extensions in~\cref{tab:pca_summary}.}



==> content/old_versions/related_work_old.tex <==
\section{Related Work}\label{sec:related}
Our work will heavily combine PCA with flag manifolds.

% \paragraph{Averaging in computer vision}
\paragraph{PCA and its variants}
Although there are many variants of PCA~\cite{hotelling1933analysis, scholkopf1997kernel, vidal2005generalized, candes2011robust, arenas2013kernel}, we focus on forms of Robust PCA (RPCA)~\cite{kwak2008principal, markopoulos2014optimal, neumayer2020robust} and Dual PCA (DPCA)~\cite{vidal2018dpcp}. 
%Given a dataset in $\R^n$, RPCA seeks to find the directions that maximize explained variance. 
As opposed to RPCA, DPCA finds directions orthogonal to RPCA and is
%, is a more robust dimensionality reduction algorithm which is 
designed to work on datasets with outliers by minimizing a $0$-norm problem~\cite{vidal2018dpcp}.
%scholkopf1997kernel,

%It finds directions orthogonal to the subspace that contains most of the inliers of the dataset. 

%Dual PCA, on the other hand, operates on the paradigm that our dataset contains many inliers and few outliers by finding directions orthogonal to the subspace that contains most of the inliers of the dataset. This essentially addresses the opposite problem of PCA by minimizing functions of the explained variance. 


%\paragraph{PCA on manifolds} 
We also consider the generalization of PCA to Riemannian manifolds, Principal Geodesic Analysis (PGA), which finds geodesic submanifolds that best represent the data~\cite{fletcher2004principal} and has been applied to the manifold of SPD matrices on ``real-world'' datasets~\cite{harandi2014manifold, smith2022data}. Though, exact PGA is hard to compute~\cite{sommer2010manifold, sommer2014optimization}.
Principal Curves~\cite{hastie1989principal} finds curves passing through the mean of a dataset which maximize variance and have seen their own enhancements~\cite{laparra2012nonlinearities}. 
Linearized (tangent) versions of PGA perform PCA on the tangent space to the mean of the data~\cite{abboud2020robust, awate2014kernel}.
Geodesic PCA (GPCA) removes the mean requirement \cite{huckemann2006principal, huckemann2010intrinsic}. 
Barycentric Subspace Analysis (BSA) realizes PCA on more classes of manifolds than just Riemannian manifolds by generalizing geodesic subspaces using weighted means of reference points~\cite{pennec2018barycentric}.
Recent years have witnessed further generalizations~\cite{pennec2020advances,rabenoro2022geometric,buet2023flagfolds} as we will mention later.
%when necessary.

%Pennec has continued investigating generalizations PCA while using flags~\cite{pennec2020advances}. Buet~\etal generalized varifolds to flagifolds to understand the eigenvalues (explained variances) from PCA along with the flag structure of the principal components in order to model multi-dimensional shapes~\cite{buet2023flagfolds}. Rabenoro~\etal offered a method for hypothesis testing and confidence regions for PCA, all within the context of flag manifolds \cite{rabenoro2022geometric}.

\paragraph{Flag manifolds}
Besides being mathematically interesting objects~\cite{wiggerman1998fundamental,donagi2008glsms,alekseevsky1997flag}, flags and flag manifolds have been explored by a series of works by Nishimori~\etal addressing subspace independent component analysis (ICA) via Riemannian optimization~\cite{nishimori2006riemannian0,nishimori2006riemannian1,nishimori2007flag, nishimori2008natural,nishimori2007flag}. Several works have also addressed averaging on flag manifolds or producing flags as subspace averages~\cite{draper2014flag,Mankovich_2023_ICCV,mankovich2023subspace}. Nested sequences of subspaces (e.g. flags) appear in principal directions,
%canonical algorithms like 
%the PCA weights, 
the numerous manifold variants of PCA \cite{pennec2018barycentric,pennec2020advances,ye2022optimization}, and the result of a wavelet transform \cite{kirby2001geometric}.



==> content/old_versions/results_lessold.tex <==
\vspace{-3mm}\section{Results}\label{sec:results}
\vspace{-3mm}
\paragraph{Baselines}
Our algorithm results in a family of novel \PCA/\TPCA~algorithms (\cf~\cref{tab:pca_summary} in blue). We compare these to their known versions using state-of-the-art implementations. In particular, we use the bit-flipping algorithm of~\cite{markopoulos2017efficient} for \LoneRPCA, the alternating scheme of~\cite{wang2017ell} for \LtwoWPCA, and the iteratively reweighted algorithm of~\cite{vidal2018dpcp} (DPCP-IRLS) for \LtwoDPCP. Finally, we use the Pymanopt~\cite{townsend2016pymanopt} implementations for Stiefel CGD and Riemannian Trust Region (RTR) methods on flag manifolds~\cite{nguyen2023operator} to directly optimize the objectives in~\cref{prop:fPCA_all}. 

\paragraph{Implementation details}
We always initialize~\cref{alg: flagified pca} randomly and determine convergence either if we reach a maximum number of iterations (max. iters. of 50) or meet at least one of $\left| f([\![\U^{(m)}]\!]) - f([\![\U^{(m+1)}]\!]) \right| < 10^{-9}$ or $d_c([\![\U^{(m)}]\!],[\![\U^{(m+1)}]\!]) < 10^{-9}$ where $d_c(\cdot, \cdot)$ is the chordal distance on $\flag(n+1)$~\cite{pitaval2013flag}. Karcher's mean / median convergence parameter is $10^{-8}$, and step size is $0.05$. 
All algorithms are run on a $2020$ M$1$ MacBook Pro.


\paragraph{Outlier detection}
Euclidean formulations of PCA yield the residuals of $\|\x_j - \U \U^T \x_j \|_2$ (for \WPCA, \RPCA, and \PCA) and $\| \B \x_j\|_2$ (for \DPCP). To predict labels for outliers, we normalize these residuals between $[0,1]$ and decide on a threshold during AUC computation. Non-Euclidean versions, (\fTWPCA, \fTRPCA, and \TPCA), given $k$ flattened principal directions $\U = [\bu_1,\dots, \bu_k]$ at a base point $\x \in \Man$, we compute $\pi_{\U}(x_j) = \U \U^T \x_j$ and reshape it into $\bv_j \in \TxM$.
The predicted label is then obtained from the reconstruction error for $\x_j$ by thresholding the manifold distance $d(\x_j, \hat{\x}_j)$, where $\hat{\x}_j = \Exp_{\x}(\bv_j)$. The predictions for \fTDPCP~follows a slightly different scheme which uses flattened estimations for the dual principal directions in $\B = [\vb_1, \dots, \vb_k]$ and the data in the tangent space $\{\bv_j\}$. The predicted label for point $j$ is obtained by thresholding $\| \B \bv_j\|_2$.
%similar projection scheme which uses flattened estimations for the dual principal directions in $\B = [\vb_1, \dots, \vb_k]$ to form $\pi_{\B}(x_j)$ that we reshape into $\w_j \in \TxM$. Then we estimate the explained variance on the manifold for $\x_j$ as $d(\x, \overline{\x}_j)$ where $\overline{\x}_j = \Exp_{\x}(\w_j)$. % We normalize each prediction vector by its maximum value for predictions between $[0,1]$. 

% We then compute $\hat{\x}_j = \Exp_{\x}(\bv_j)$ and the predicted label as the reconstruction error for $\x_j$ as the manifold distance $d(\x_j, \hat{\x}_j)$. Finally, we compute the predictions for \fTDPCP~using a similar projection scheme which uses flattened estimations for the dual principal directions in $\B = [\vb_1, \dots, \vb_k]$ to form $\pi_{\B}(x_j)$ that we reshape into $\w_j \in \TxM$. Then we estimate the explained variance on the manifold for $\x_j$ as $d(\x, \overline{\x}_j)$ where $\overline{\x}_j = \Exp_{\x}(\w_j)$. We normalize each prediction vector by its maximum value for predictions between $[0,1]$. 

% Euclidean formulations of \WPCA, \RPCA, and \PCA~use $\|\x_j - \U \U^T \x_j \|_2$ and \DPCP~uses $\| \B \x_j\|_2$ as the predicted labels for outliers. For the manifold formulations \fTWPCA, \fTRPCA, and \TPCA~we use a different label estimation scheme. Given $k$ flattened principal directions at a center point $\x \in \Man$ stored in the matrix $\U = [\bu_1,\dots, \bu_k]$, we compute $\pi_{\U}(x_j) = \U \U^T \x_j$. We reshape $\pi_{\U}(x_j)$ into the proper tangent space dimensions and call it $\bv_j \in \TxM$. Then compute $\hat{\x}_j = \Exp_{\x}(\bv_j)$ and the predicted label as the reconstruction error for $\x_j$ as the manifold distance $d(\x_j, \hat{\x}_j)$. Finally, we compute the predictions for \fTDPCP~using a similar projection scheme which uses flattened estimations for the dual principal directions in $\B = [\vb_1, \dots, \vb_k]$ to form $\pi_{\B}(x_j)$ that we reshape into $\w_j \in \TxM$. Then we estimate the explained variance on the manifold for $\x_j$ as $d(\x, \overline{\x}_j)$ where $\overline{\x}_j = \Exp_{\x}(\w_j)$. We normalize each prediction vector by its maximum value for predictions between $[0,1]$. 

\subsection{Evaluating Euclidean Principal Directions}
\label{sec:eucPD}
%We first assess the qualities of our method in flat spaces.
\noindent\textbf{Can flagified PCAs recover specified algorithms?}
% Code in Euclidean/sanity_check.ipynb
To ensure that our robust algorithms in~\cref{alg: flagified pca} can recover traditional, specific PCA variants, we compare \foneRPCA~to \LoneRPCA, \ftwoWPCA~to \LtwoWPCA, and \ftwoDPCP~to \LtwoDPCP~in~\cref{tab:compare} (with $200$ max. iters.) by computing the first $k=2$ principal directions of $\{ \x_i\}_{i=1}^{100} \in \R^{5}$ where $\x_i\sim\mathcal{U}[0,1)$ is sampled uniformly. % over $[0,1)$. %Flag variants are found using~\cref{alg: flagified pca} and other algorithms are implemented using~\cite{markopoulos2017efficient,wang2017ell,vidal2018dpcp} respectively.
As seen, our algorithms converge to similar objective values as the baselines 
% \LoneRPCA~and \LtwoWPCA~converge to more optimal objective values and 
while \LtwoWPCA~and \LtwoDPCP~run faster than the flag versions. Yet, the novel \foneRPCA~is much faster than \LoneRPCA~and \ftwoDPCP~converges to a more optimal objective albeit being initialized randomly, as opposed to SVD-initialization of \LtwoDPCP. %~is initialized with the SVD, whereas~\cref{alg: flagified pca} is initialized randomly.
% So our general~\cref{alg: flagified pca} for finding flagified robust \PCA~recovers
%is competitive with the robust \PCA~specific algorithms.


% \begin{table}[t!]
%     \centering
%     \begin{tabular}{c @{\:}c|| c |c}
%         & Algorithm & Obj. Val. & Time \\ 
%         \toprule
%         \multirow{2}{*}{$\uparrow$} & \LoneRPCA & $\mathbf{54.69}$ & $70.66$ \\ 
%         & \foneRPCA & $54.66$          & $\mathbf{0.19}$ \\ 
%         \midrule
%         \multirow{2}{*}{$\downarrow$} & \LtwoWPCA & $\mathbf{42.89}$ & $\mathbf{0.24}$ \\ 
%         & \ftwoWPCA & $42.92$          & $0.45$ \\ 
%         \midrule
%         \multirow{2}{*}{$\downarrow$} & \LtwoDPCP & $34.83$          & $\mathbf{0.26}$ \\ 
%         & \ftwoDPCP & $\mathbf{34.66}$ & $0.38$ \\ 
%     \end{tabular}
%     \caption{Objective function values and run times for robust \PCA variants. The general~\cref{alg: flagified pca} is comparable to the baseline algorithms. Run times on $2020$ MacBook Pro with M$1$ Chip. \tolga{transpose the table.}}
%     % \label{tab:compare}
% \end{table}

\begin{table}[t!]
    \centering
    \begin{tabular}{l@{\:}c@{\:}|@{\:}c|c@{\:}|@{\:}c|c@{\:}|@{\:}c}
        & \multicolumn{2}{c}{\LoneRPCA} & \multicolumn{2}{c}{\LtwoWPCA} & \multicolumn{2}{c}{\LtwoDPCP} \\
        \cmidrule{2-7}
        & Obj.$\uparrow$ & Time & Obj.$\downarrow$ & Time & Obj.$\downarrow$ & Time \\
        \midrule
        Baseline\,\,\, & $\mathbf{54.69}$ & $70.66$ & $\mathbf{42.89}$ & $\mathbf{0.24}$ & $34.83$ & $\mathbf{0.26}$\\
        %\hline
        Flag (\cref{alg: flagified pca}) & $54.66$ & $\mathbf{0.19}$ & $42.92$ & $0.45$ & $\mathbf{34.66}$ & $0.38$\\
        \bottomrule
    \end{tabular}
    \caption{Objective function values and run times comparing \foneRPCA/ \ftwoWPCA/ \ftwoDPCP~found with~\cref{alg: flagified pca} to baselines \LoneRPCA/ \LtwoWPCA/ \LtwoDPCP~respectively.\vspace{-1mm}}
    \label{tab:compare}
\end{table}



\vspace{0.3mm}
\noindent\textbf{Is our algorithm advantageous to direct optimization on manifolds?}
% Code in Euclidean/convergence_tests.ipynb
We compare~\cref{alg: flagified pca} to direct optimization with Stiefel CGD and Flag RTR on data $\{ \x_i\}_{i=1}^{30} \in \R^{4}$ where $\x_i \sim \mathcal{U}[0,1)$.~\cref{fig:pymanopt_compare_fl} presents run times and objective values attained when computing the first $k=2$ principal directions via \foneRPCA, \foneWPCA, and \foneDPCP~with $20$ random initializations. Our algorithms converge faster and to more optimal objective values than naive Stiefel-CGD and Flag-RTR.
\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{figures/cgd_comparison_st.pdf}
    \caption{\cref{alg: flagified pca} converges faster to more optimal cost values compared to Stiefel CGD or Flagg RTR.}
    \label{fig:pymanopt_compare}
\end{figure}
\end{comment}

\begin{figure}
    \centering\vspace{-3mm}
    \includegraphics[width = \linewidth]{figures/cgd_comparison_fl.pdf}
    \caption{\cref{alg: flagified pca} converges faster to more optimal cost values compared to Stiefel CGD or Flag RTR.\vspace{-3mm}}
    \label{fig:pymanopt_compare_fl}
\end{figure}

\paragraph{Impact of flag-type on cluster detection} % Code in Euclidean/flag_type_classification.py
To assess the impact of flag-type, we generate a 
%specific 
dataset $\{\x_j\}_{j=1}^{300} \subset \R^{10}$ with $3$ clusters ($C_1,C_2,C_3$) in which we curate the flag type corresponding to the data structure: $\flag(2,5,7; 10)$.
We then compute $2$ sets of $k=7$ principal directions by running \fWPCA~with flag type $(2,5,7;10)$ (\fWPCA$(2,5,7)$) and \ftwoWPCA~using~\cref{alg: flagified pca} with $200$ max. iters. Both of these methods result in a flag representative $\U = [\U_1, \U_2, \U_3] \in \R^{10\times 7}$ where $\U_1 \in \R^{10 \times 2}$, $\U_2 \in \R^{10 \times 3}$, and $\U_3 \in \R^{10 \times 2}$. We compute the reconstruction error for point $j$ against each $\U_i$ as $\sum_{j=1}^p \|\x_j - \U_i \U_i^T \x_j\|_2$. These errors are used for $3$ classification tasks, predicting $C_i$ using $\U_i$ for $i=1,2,3$. 
% We sample data $\{\x_j\}_{j=1}^{300} \subset \R^{10}$ with $3$ clusters ($C_1,C_2,C_3$) that satisfy $\text{dim}(C_2) = 2$, $\text{dim}(C_3) = 3$, and $\text{dim}(C_1) = 2$. The details of generating this dataset is in the supplementary. The clustered structure of this dataset is optimal for running flagified versions of robust PCA optimizing over the flag corresponding to the data structure: $\flag(2,5,7; 10)$. To validate this, we compute $2$ sets of $k=7$ principal directions by running \fWPCA~with flag type $(2,5,7)$ (\fWPCA$(2,5,7)$) and \ftwoWPCA~using~\cref{alg: flagified pca} with $200$ max. iters. Both of these methods result in a flag representative $\U = [\U_1, \U_2, \U_3] \in \R^{10\times 7}$ where $\U_1 \in \R^{10 \times 2}$, $\U_2 \in \R^{10 \times 3}$, and $\U_3 \in \R^{10 \times 2}$. We the compute the reconstruction error for point $j$ with each $\U_i$ as $\sum_{j=1}^p \|\x_j - \U_i \U_i^T \x_j\|_2.$ These errors are used for $3$ classification experiments: predict $C_i$ with $\U_i$ for $i=1,2,3$. 
%For example, in experiment $i=1$, the true labels for class $1$ are $0$ for points $i=1,\dots,150$ and $1$ otherwise. 
The corresponding AUC values are in~\cref{tab:fl_type}.
\fWPCA$(2,5,7)$ produces higher AUCs 
%for each cluster 
because it is optimized over a more optimal flag type, respecting the subspace structure of the data.
\begin{table}[t!]
    \centering
    \begin{tabular}{l@{\:}||@{\:}c@{\:}|@{\:}c@{\:}|@{\:}c@{\:}|@{\:}c@{\:}|@{\:}c@{\:}|@{\:}c}
         & \multicolumn{2}{c}{Cluster $1$} & \multicolumn{2}{c}{Cluster $2$} & \multicolumn{2}{c}{Cluster $3$}\\
         \toprule
        \fWPCA$(\cdot)$ & $(7)$ & $(2,5,7)$ & $(7)$ & $(2,5,7)$ & $(7)$ & $(2,5,7)$ \\
        \hline
        AUC $\uparrow$ & $0.72$ & $\mathbf{0.73}$ & $0.48$ & $\mathbf{1.00}$ & $0.43$ & $\mathbf{0.49}$
    \end{tabular}
    \caption{AUC for cluster classification using  \fWPCA. We see higher AUCs when we match the flag type for \fWPCA~with the cluster dimensions (e.g., $(2,5,7)$).\vspace{-1mm}}
    \label{tab:fl_type}
\end{table}

% \paragraph{}
\vspace{-2mm}
\subsection{Evaluating Non-Euclidean Extensions}\label{sec: exp-noneuc}
\vspace{-2mm}
We now evaluate flagified tangent-PCA and its robust variants starting with a synthetic evaluation of the sphere and Grassmannian before moving to real datasets.

\paragraph{Convergence on $4$-sphere}
To sample a dataset of inliers and outliers on the $4$-sphere $\mathbb{S}^4 = \left \{ \x \in \R^5 : \| \x \|_2 = 1 \right\}$, we first sample a random center $\x \in \mathbb{S}^4$, and then sample $100$ inlier tangent vectors from $\mathcal{U}[0,.01)$. Another $20$ outlier tangent vectors $\bv$, have entries $v_1, v_2 \sim \mathcal{U}[0,.01)$ and $v_3, v_4, v_5 \sim \mathcal{U}[0,.1)$. We wrap these vectors to have our dataset, $\{\Exp_{\x}(\bv)\}$. Then we compute the first $k=2$ principal directions of \foneTRPCA, \foneTWPCA, and \foneTDPCP~with $50$ random initializations and plot objective values
as Euclidean optimizations in the tangent space of the Karcher median at each iteration of~\cref{alg: flagified pca} in~\cref{fig: all_convergence}. All methods converge in fewer than $7$ iterations, while the spread of objective function values due to initializations decreases.


\begin{figure}[t]
    \centering
    \includegraphics[width =\linewidth]{figures/all_convergence.pdf}
    \caption{$50$ random initializations of \fTPCA~ variations. The blue line is the mean and the shaded region is the standard deviation. The $x$-axis of this plot is the number of iterations of~\cref{alg: flagified pca} performed in the tangent space.\vspace{-3mm}}
    \label{fig: all_convergence}
\end{figure}

\paragraph{Outlier detection on $Gr(2,4)$}
To compare between different flag type realizations of flagified robust PCAs, we now synthesize data with inliers and outliers on $Gr(2,4)$, the set of all $2$-planes in $\R^4$ represented as $Gr(2,4) = \left \{ [\X]: \X \in \R^{4 \times 2} \text{ and }\X^T \X = \I  \right \}$~\cite{edelman1998geometry}. To do so, consider two random points $[\X],[\Y] \in Gr(2,4)$ acting as centroids for inliers and outliers, respectively.  
Inliers are sampled as $\Exp_{[\X]}(a\V_i)$ where $a \sim \mathcal{U}[0,1)$, $\V_1, \V_2 \in \mathcal{T}_{[\X]}(Gr(2,4))$ are two random tangent vectors and $\Exp_{[\X]}$ is the exp-map of $Gr(2,4)$. We randomly choose $i\in \{1,2\}$. 
Outliers are sampled similarly as $\Exp_{[\Y]}(b\V)$ where $b \sim \mathcal{U}[0,0.1)$ and gradually added to the dataset.
~\cref{fig:out_auc_gr24_man} plots the AUCs for outlier detection using the first $k=2$ principal directions. \foneTDPCP~produces the highest AUC and is more stable to the presence of outliers. We also found that Euclidean \PCA~variants with the same data produce lower AUC (see supplementary).

% $Gr(2,4)$ is parameterized by the set of all $2$-planes in $\R^4$~\cite{edelman1998geometry} and can be represented as $Gr(2,4) = \left \{ [\X] : \X \in \R^{4 \times 2} \text{ and }\X^T \X = \I  \right \}$.
% We sample data on $Gr(2,4)$ with inliers and outliers, and compare between different flag type realizations of flagified robust PCAs. We generate inlier data by sampling a random point $[\X] \in Gr(2,4)$ and two random tangent vectors $\V_1, \V_2 \in \mathcal{T}_{[\X]}(Gr(2,4))$. Inliers are sampled as $\Exp_{[\X]}(a\V_i)$ where $a \sim \mathcal{U}[0,1)$ and we randomly choose $i\in \{1,2\}$. Outliers are sampled from tangent vectors at a different center $[\Y] \in Gr(2,4)$, sampling $\V \in \mathcal{T}_{[\X]}(Gr(2,4))$. Then an outlier is $\Exp_{[\Y]}(b\V)$ where $b \sim \mathcal{U}[0,.1)$. 
% We gradually add outliers to a dataset and plot the AUCs for outlier detection in~\cref{fig:out_auc_gr24} using the first $k=2$ principal directions. For this plot we call Tangent \PCA~variants the ``Manifold'' method. 


\begin{figure}[t]
    \centering
    \includegraphics[width =\linewidth, trim=0mm 2mm 0mm 3mm, clip]{figures/gr_outlier_detection_man.pdf}
    \caption{AUC of different algorithms for outlier detection using the first $k=2$ principal directions of outlier-contaminated data on $Gr(2,4)$. All iterative variants are optimized with $100$ max. iters.}
    \label{fig:out_auc_gr24_man}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width =\linewidth]{figures/outlier_detection.pdf}
%     \caption{AUC of different algorithms for outlier detection using the first $k=2$ principal directions of outlier-contaminated data on $Gr(2,4)$. The ``Manifold'' plot corresponds to tangent space ($\mathcal{T}$) formulations. All algorithms other than PCA are optimized using~\cref{alg: flagified pca,alg: tPDs} with $100$ max. iters.\nate{change title of manifold to Riemannian or Non-Euclidean (Tangent)}. \tolga{move the manifold to fig. 4 and move euclidean to supp.}}
%     \label{fig:out_auc_gr24}
% \end{figure}



% \paragraph{Reconstruction and outlier Detection on Kendall (pre-shape) space}

\paragraph{Outlier detection and reconstruction on Kendall pre-shape space}
% New hands experiment
We use an outlier-contaminated version of the 2D Hands~\cite{stegmann2002} to probe the performance on a real dataset. We represent the $44$ total inlier Procrustes-aligned hands
%(\url{https://github.com/msrepo/statistical_shape_model}) 
and added outliers in the Kendall pre-shape space~\cite{kendall1984shape}: $\Sigma_2^{56} := \left \{ \X \in \R^{56 \times 2} \: : \: \| \X\|_F = 1 \text{ and } \sum_{i=1}^{56} \x_i = 0 \right \}$.
We sample outliers as open ellipses with axes sampled from $\mathcal{N}(.4,.5)$, centers from $\mathcal{N}(0,.1)$, and a hole that is $\approx 6.8\%$ of the entire ellipse. We project these outliers onto $\Sigma_2^{56}$ by normalization and mean-centering. % Our supplementary contains experiments involving hand reconstruction in the presence of more ``extreme'' outliers.
~\cref{fig: hand_pred_ablation} reports the AUC on outlier detection as we gradually add outliers. \fTDPCP~has the best outlier detections for both flag variants followed by \fTRPCA, \fTWPCA, and \TPCA~with flag type $(1,2,\dots,k)$ producing different AUC than $\flag(k)$ (\cf~\cref{tab:pca_summary}). All algorithms in these experiments are initialized with the SVD.
\begin{figure}[t]
    \centering
    \includegraphics[width = \linewidth]{figures/hand_outlier_resFeb.pdf}
    \caption{Mean AUC for outlier predictions using the first $k=4$ principal directions where we gradually add outlier ellipses to the $2$D Hands dataset. The mean is over $20$ trials of adding outliers.\vspace{-3mm}}
    \label{fig: hand_pred_ablation}
\end{figure}
We further consider a dataset with $30$ outliers to isolate the hands (inliers). We run \TPCA~with $k=2$ principal directions to reconstruct the first hand in~\cref{fig:rec_with_out_removal}. In a slight abuse of notation, we reconstruct a hand $\x \in \Sigma_2^{56}$ using $k=2$ principal tangent directions $\{\bu_1, \bu_2\} \in \mathcal{T}_{\bm{\mu}}\left(\Sigma_2^{56}\right)$ as $\hat{\x} = \Log_{\mu} \left( \U \U^T \Exp_{\mu}(\x) \right)$ where $\U = [\bu_1, \bu_2]$. Since \foneTDPCP~and \ftwoTDPCP~almost perfectly detect all the outliers, they produce the best reconstructions.
\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{figures/hand_qualFeb.pdf}
    \caption{Reconstructions using a \PCA~of the inliers detected by variants of \fTWPCA, \fTRPCA, \fTDPCP~and \TPCA~on a the $2$D Hands dataset with $28$ hands and $16$ ellipses. The reconstruction error is reported inside each hand.}\label{fig:rec_with_out_removal}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
% Old hands experiment
% \textcolor{blue}{Nate: Re-do these}


% We use an outlier-contaminated version of the 2D Hands~\cite{stegmann2002} to probe the performance on a real dataset. We represent the $40$ inlier hands and added outliers in the Kendall pre-shape space~\cite{kendall1984shape}: $\Sigma_2^{56} := \left \{ \X \in \R^{56 \times 2} \: : \: \| \X\|_F = 1 \text{ and } \sum_{i=1}^{56} \x_i = 0 \right \}$.
% We sample outliers as open ellipses with axes sampled from $\mathcal{N}(.4,.5)$, centers from $\mathcal{N}(0,.1)$, and a hole that is $\approx 6.8\%$ of the entire ellipse. We project these outliers onto $\Sigma_2^{56}$ by normalization and mean-centering. % Our supplementary contains experiments involving hand reconstruction in the presence of more ``extreme'' outliers.
% ~\cref{fig: hand_pred_ablation} reports the AUC on outlier detection as we gradually add outliers. \fTDPCP~has the best outlier detections for both flag variants followed by \fTRPCA, \fTWPCA, and \TPCA~with flag type $(1,2,\dots,k)$ producing higher AUC than $\flag(k)$ because $(1,2,\dots, k)$ is a ``more robust'' type than $(k)$ corresponding to $L_1$. (\cf~\cref{tab:pca_summary}).
% \begin{figure}[t]
%     \centering
%     \includegraphics[width = \linewidth]{figures/hand_outlier_res.pdf}
%     \caption{Mean AUC for outlier predictions using the first $k=2$ principal directions where we gradually add outlier ellipses to the $2$D Hands dataset. The mean is over $5$ trials of adding outliers.\vspace{-3mm}}
%     \label{fig: hand_pred_ablation}
% \end{figure}
% We further consider a dataset with $30$ outliers to isolate the hands (inliers). We run \TPCA~with $k=2$ principal directions to reconstruct the first hand in~\cref{fig:rec_with_out_removal}. In a slight abuse of notation, we reconstruct a hand $\x \in \Sigma_2^{56}$ using $k=2$ principal tangent directions $\{\bu_1, \bu_2\} \in \mathcal{T}_{\bm{\mu}}\left(\Sigma_2^{56}\right)$ as $\hat{\x} = \Log_{\mu} \left( \U \U^T \Exp_{\mu}(\x) \right)$ where $\U = [\bu_1, \bu_2]$. Since \foneTDPCP~and \ftwoTDPCP~almost perfectly detect all the outliers, they produce the best reconstructions.
% \begin{figure}
%     \centering
%     \includegraphics[width = \linewidth]{figures/hand_qual.pdf}
%     \caption{Reconstructions of the $0$th hand using a \PCA~of the inliers detected by variants of \fTWPCA, \fTRPCA, \fTDPCP~and \TPCA~on a the $2$D Hands dataset with $30$ outliers. The reconstruction error is reported inside each hand.}\label{fig:rec_with_out_removal}
% \end{figure}



% \section{After this is not structured...}

% We run experiments on synthetic data to probe the properties of \cref{alg: flagified pca,alg: tPDs} and the novelty of flagified \PCA~variants with non-trivial flag types. Then we compare \fRPCA, \fWPCA, and \fDPCP~to \fTRPCA, \fTWPCA, and \fTDPCP~for outlier detection on $Gr(2,4)$. More importantly, we investigate the practical value of \fTRPCA, \fTWPCA, and \fTDPCP~on hand pose data for hand reconstruction with outlier-contaminated data and for outlier classification.




% \tolga{One common remark about experimentation: We proposed many new algorithms as highlighted in~\cref{tab:pca_summary}. Do some of these work better at any of the experiments? Or are they completely useless? I think both t-fWPCA and fDPCP work well in certain experiments. This means that developing new algorithms thru the flag perspective gives us new reduction algorithms that can be of practical value?} \nate{so just summarize the practical utility of these algorithms in this section?}

% \subsection{Metrics}
% \begin{itemize}
% \item Angles (T)
% \item Euclidean reconstruction error
% \item Manifold reconstruction error
% \item Euclidean explained variance
% \end{itemize}

% \subsection{Synthetic Data}
% We compare the performance of~\cref{alg: flagified pca} to state of the art methods, investigate convergence, determine the novelty of flag types between those which recover $L_2$ and $L_1$ robust \PCA ($(k;n)$ and $(1,2,\dots,k;n)$ respectively), and (iii) evaluate flagified robust \PCA and \TPCA variants for outlier detection in $\R^n$ and $Gr(2,4)$.

% All Euclidean principal directions in this section other than \PCA are optimized using~\cref{alg: flagified pca} and all manifold principal directions are optimized using~\cref{alg: tPDs} unless otherwise stated.

% \begin{table}[t!]
%     \centering
%     \begin{tabular}{c@{\:}|c@{\:}|@{\:}c@{\:}|@{\:}c@{\:}|@{\:}c@{\:}|@{\:}c@{\:}|@{\:}c}
%         Alg. & \multicolumn{2}{c}{\LoneRPCA $\uparrow$} & \multicolumn{2}{c}{\LtwoWPCA $\downarrow$} & \multicolumn{2}{c}{\LtwoDPCP $\downarrow$} \\
%         & \cite{markopoulos2017efficient} & \cref{alg: flagified pca} & \cite{wang2017ell} & \cref{alg: flagified pca} & \cite{vidal2018dpcp} & \cref{alg: flagified pca} \\
%         \toprule
%         Obj. Val. & $\mathbf{54.69}$ & $54.66$ & $\mathbf{42.89}$ & $42.92$ & $34.83$ & $\mathbf{34.66}$ \\
%         Time (s) & $70.66$  & $\mathbf{0.19}$ & $\mathbf{0.24}$ & $0.45$ & $\mathbf{0.26}$ & $0.38$
%     \end{tabular}
%     \caption{Objective function values and run times for flagified algorithms and their counterparts. Flagified algorithms are generally comparable to the baseline algorithms. Flag \LoneRPCA~ is much faster than the algorithm from~\cite{markopoulos2017efficient}. Run times are on $2020$ MacBook Pro with M$1$ Chip.}
%     \label{tab:compare}
% \end{table}

% \paragraph{\cref{alg: flagified pca} v.s. Stiefel CGD}


% \paragraph{Flag Types in $\R^{10}$} 


% \paragraph{Convergence on $4$-Sphere}




\begin{comment}
\paragraph{Outlier Detection on Gr(2,4)}
$Gr(2,4)$ is parameterized by the set of all $2$-planes in $\R^4$~\cite{edelman1998geometry} and can be represented as
\begin{equation*}
    Gr(2,4) = \left \{ [\X] : \X \in \R^{4 \times 2} \text{ and }\X^T \X = \I  \right \}.
\end{equation*}
We sample data on $Gr(2,4)$ with inliers and outliers and compare different flag type realizations of flagified robust PCAs. We generate inlier data by sampling a random point $[\X] \in Gr(2,4)$ and two random tangent vectors $\V_1, \V_2 \in \mathcal{T}_{[\X]}(Gr(2,4))$. Inliers are sampled as $\Exp_{[\X]}(a\V_i)$ where $a \sim \mathcal{U}[0,1)$ and we randomly choose $i\in \{1,2\}$. Outliers are sampled from tangent vectors at a different center $[\Y] \in Gr(2,4)$, sampling $\V \in \mathcal{T}_{[\X]}(Gr(2,4))$. Then an outlier is $\Exp_{[\Y]}(b\V)$ where $b \sim \mathcal{U}[0,.1)$. 

We gradually add outliers to a dataset and plot the AUCs for outlier detection in~\cref{fig:out_auc_gr24} using the first $k=2$ principal directions. For this plot we call Tangent \PCA~variants the ``Manifold'' method. 

Euclidean formulations of \WPCA, \RPCA, and \PCA~use $\|\x_j - \U \U^T \x_j \|_2$ and \DPCP~uses $\| \B \x_j\|_2$ as the predicted labels for outliers. For the manifold formulations \fTWPCA, \fTRPCA, and \TPCA~we use a different label estimation scheme. Given $2$ flattened principal directions at a center point $\x \in \Man$ stored in the matrix $\U = [\bu_1, \bu_2]$, we compute $\pi_{\U}(x_j) = \U \U^T \x_j$. We reshape $\pi_{\U}(x_j)$ into the proper tangent space dimensions and call it $\bv_j \in \TxM$. Then compute $\hat{\x}_j = \Exp_{\x}(\bv_j)$ and the predicted label as the reconstruction error for $\x_j$ as the manifold distance $d(\x_j, \hat{\x}_j)$. Finally, we compute the predictions for \fTDPCP~using a similar projection scheme, which uses flattened estimations for the dual principal directions in $\B = [\vb_1, \vb_2]$ to form $\pi_{\B}(x_j)$ that we reshape into $\w_j \in \TxM$. Then we estimate the explained variance on the manifold for $\x_j$ as $d(\x, \overline{\x}_j)$ where $\overline{\x}_j = \Exp_{\x}(\w_j)$. We normalize each prediction vector by its maximum value for predictions between $[0,1]$. 


Looking at~\cref{fig:out_auc_gr24}, we see that manifold and Euclidean \fDPCP~produce the highest AUCs for outlier detection. In fact, novel \foneTDPCP~produces the highest AUC and is more stable as we add more outliers. Other than that, manifold versions of these algorithms are slightly better at detecting outliers than their Euclidean counterparts and \RPCA~variants outpreform \PCA.  
\begin{figure}[t]
    \centering
    \includegraphics[width =\linewidth]{figures/outlier_detection.pdf}
    \caption{AUC of different algorithms for outlier detection using the first $k=2$ principal directions of outlier-contaminated data on $Gr(2,4)$. The ``Manifold'' plot corresponds to tangent space ($\mathcal{T}$) formulations. All algorithms other than PCA are optimized using~\cref{alg: flagified pca,alg: tPDs} with $100$ max. iters.\nate{change title of manifold to Riemannian or Non-Euclidean (Tangent)}. \TB{move the manifold to fig. 4 and move Euclidean to supp.}}
    \label{fig:out_auc_gr24}
\end{figure}
\end{comment}



% \begin{figure}[t]
%     \centering
%     \includegraphics[width =\linewidth]{figures/WPCAvPCA.png}
%     \caption{fWPCA($2,5,9$) (right) places higher variance in Cluster $3$ (green points) for the $8$th and $9$th PCs. Blue points are in cluster 1 and orange points are in cluster 2.}
%     \label{fig: fWPCAvPCA}
% \end{figure}





% \paragraph{Online Principle Directions}
% Take a dataset that can be seperated into two subsets of samples. Samples until time $t$ and samples from time $t+1$ to $T$. Then run each of the four algorithms: PCA, PGA, DPCP-IRLS, DPGP-IRLS with Stiefel and flagified versions on each of the two datasets. Use flag averaging to get estimation of PCs for the whole dataset. For example \url{http://proceedings.mlr.press/v33/goes14.pdf}.



% We evaluate our flagified \PCA~and flagified \TPCA~formulations on 

%We use two types of outliers for our dataset (visualized in~\cref{fig:outlier_qual}): ``Hairballs'' in hand reconstruction and ``Open Ellipses'' in outlier detection. We use two different datasets in these experiments in order to separate between the different \PCA~variants.



%max iterations for gradient descent is 1000
% \begin{itemize}
%  \item \url{https://github.com/msrepo/statistical_shape_model}
%  \item \url{https://github.com/DrewLazar/RobustManifold/tree/master/HandShape/RawData}
%  \item \url{https://link.springer.com/chapter/10.1007/978-3-540-76725-1_35}
% \end{itemize}


==> content/old_versions/results_old.tex <==
\section{Results}\label{sec:results}
\begin{comment}
    I offer more ideas of applications with cool data on Earth and climate here: 1) http://dx.doi.org/10.1109/JSTSP.2015.2417833 2) http://dx.doi.org/10.1109/MSP.2013.2250591 3) https://doi.org/10.1109/TGRS.2020.2969813
\end{comment}

\subsection{Synthetic}
% \nate{Maybe we do one figure for this subsection with just one plot of the ratio of inliers to outliers for 3 manifolds: sphere, psd, and rotations. We'd have to visualie the standard deviation of the ratio for this.}

\paragraph{Robust Flagified PCA}
We begin with $100$ inliers in $\R^{8}$ samples from $\mathcal{N}(0,1)$. We compute $5$ components using PCA and Robust Flagified PCA for the dataset of inliers. Then outliers are sampled as $\x \in \R^8$ with $\x_j \sim \mathcal{N}(0,1)$ for $j=1,2,\dots,5$ and $\x_j \sim \mathcal{N}(0,10)$ for $j=6,7,8$. We compute $5$ components using PCA and Robust Flagified PCA on the dataset with inliers and outliers and measure the chordal distance on $\flag(1,2,\dots,5;8)$ between components and the inlier components. We do $10$ random data sets for each trial. The results are in~\cref{fig:synthetic_flag_pca}. All the Robust Flagified PCA methods are more robust to outliers with respect to the chordal distance on $\flag(1,2,3,4,5;8)$. Specifically, $\flag(1,2,3,4,5;8)$ has the lowest variance across flag types.

\begin{figure}[H]
    \centering
    \includegraphics[width =\linewidth]{figures/flag_type_pca.pdf}
    \caption{Robust Flag PCA are the colored lines the shaded region is one standard deviation away from the mean from $10$ random datasets. $[3,5]$ corresponds to $\flag(3,5;8)$.}
    \label{fig:synthetic_flag_pca}
\end{figure}
\nate{Do geodesic distance. Add in random guess.}


$\X = [\x_1,\dots, \x_5] \in \R^{10 \times 5}$
\[
\sum_{i=1}^5  \theta(\x_i, \y_i)
\]
\[
\argmin_{\y} \sum_{i=1}^5  \theta(\x_i, \y) \neq \argmin_{\y} \sum_{i=1}^5  \sin\theta(\x_i, \y)
\]

\paragraph{Robust Flagified DPCP-IRLS}
We begin with $100$ inliers in $\R^{8}$ samples from $\mathcal{N}(0,1)$. We compute $4$ components using DPCP-IRLS and Robust Flagified DPCP-IRLS for the dataset of inliers. Then outliers are sampled as $\x \in \R^8$ with $\x_j \sim \mathcal{N}(0,1)$ for $j=1,2,3,4$ and $\x_j \sim \mathcal{N}(0,10j)$ for $j=5,6,7,8$. We compute $4$ components using DPCP-IRLS and Robust Flagified DPCP-IRLS on the dataset with inliers and outliers and measure the chordal distance on $\flag(1,2,\dots,4;8)$ between components and the inlier components. We do $20$ random data sets for each trial. The results are in~\cref{fig:synthetic_flag_dpcp}. Robust Flagified DPCP-IRLS methods are more robust to outliers with respect to the chordal distance on $\flag(1,2,3,4;8)$.

\begin{figure}[H]
    \centering
    \includegraphics[width =\linewidth]{figures/flag_type_dpcp.pdf}
    \caption{Robust Flag DPCP-IRLS are the colored lines the shaded region is one standard deviation away from the mean from $20$ random datasets.}
    \label{fig:synthetic_flag_dpcp}
\end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[width =\linewidth]{figures/flag_tangent.pdf}
    \caption{Robust Flagified-Tangent-PCA are the colored lines the shaded region is one standard deviation away from the mean from $10$ random datasets. \tolga{Is this really $0.2\%$ outliers? If so, it is almost nothing. I'm also surprised that the standard PCA methods are so robust to outliers... There seems to be a small bug somewhere?.}}
    \label{fig:synthetic_flag_tangent}
\end{figure}



\nate{You're right. It's proportion of outliers. So like 20\%. Should I do more? This is the distance between the PC weights with no outliers and the PC weights as we add more outliers. In general, the lower the chordal distance, the more robust to outliers.}

\begin{figure}[H]
    \centering
    \includegraphics[width =\linewidth]{figures/flag_tangent_dpcp.pdf}
    \caption{Robust Flagified-Tangent-DPCP-IRLS are the colored lines the shaded region is one standard deviation away from the mean from $10$ random datasets. \nate{increase the amount of outliers}}
    \label{fig:synthetic_flag_tangent_dpcp}
\end{figure}



% \paragraph{Sphere Example}
% \tolga{An immediate example I thought of: Generate points on the sphere with outilers, synthetically, where we know the ground truth. You can then put all of the methods at test, from PCA to Dual PGA. You can run the PCA treating that the points follow a Euclidean structure. The Dual PGA would be both outlier and manifold aware. So I expect the best results with that one. What do you think?}\\
% \nate{Great idea! I tried this with the Sphere and got bad results. But it did work with PSD matrices. See below.}


% We do $100$ random trials where we sample $1000$ inliers and $100$ outliers on the Riemannian manifold of $10$-dimensional rank-$1$ Positive Semi-definite Matrices (PSD). The inliers live on the same geodesic sub-manifold spanned by $9$ tangent vectors and the outliers are randomly sampled from a $1$-dimensional geodesic submanifold. PCA and Tangent PCA do not show any separation between inliers and outliers so we run DPCP-IRLS and DPGP-IRLS on these data to distinguish between the inliers and outliers. 

% The mean absolute correlation between the first dual principal component and the data are in~\cref{fig:synthetic_psd1}. 

% \begin{figure}[H]
%     \centering
%     \includegraphics[width =\linewidth]{figures/synthetic_psd1.pdf}
%     \caption{Our manifold-informed implementation of DPCP-IRLS has higher correlation with outliers and lower correlation with inliers than the Euclidean version.}
%     \label{fig:synthetic_psd1}
% \end{figure}


% We do $100$ random trials where we sample $1000$ inliers and $100$ outliers on the $9$-sphere. The inliers live on the same geodesic sub-manifold spanned by $8$ tangent vectors and the outliers are randomly sampled. PCA and Tangent PCA do not show any separation between inliers and outliers so we run DPCP-IRLS and DPGP-IRLS on these data to distinguish between the inliers and outliers. 

% The mean absolute correlation between the first $2$ dual principal components and the data are in~\cref{tab:sphere_ex1}. For DPGP-IRLS, we use the Euclidean mean for the manifold mean and compute correlations between the tangent vector data representations. DPGP-IRLS treats the data as living on the $9$-sphere and DPCP-IRLS uses a Euclidean space representation, e.g., $\R^{10}$. Notice $0.0048/ 0.0602 < 0.0360 /0.4504$ which implies that the manifold informed algorithm, DPGP-IRLS, improves outlier detection over the Euclidean version, DPCP-IRLS. 

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{c|cc}
%                  & Inliers       & Outliers \\
%                  \hline
%         DPGP-IRLS     & $ 0.0048 \pm 0.0012 $ & $ 0.0602 \pm 0.0054 $\\
%         DPCP-IRLS     & $ 0.0360 \pm 0.0159 $ & $ 0.4504 \pm 0.0261 $
%     \end{tabular}
%     \caption{$1000$ inliers and $100$ outliers on the $9$-sphere. The inliers live on a geodesic submanifold spanned by $8$ tangent vectors and the outliers are randomly sampled. Entries are mean absolute correlations between the first $2$ dual PCs and the data.}
%     \label{tab:sphere_ex1}
% \end{table}

% \paragraph{PSD Example}
% Consider data samples on the manifold of $10$-dimensional rank-$1$ Positive Semidefinite Matrices (PSD). We run the same sampling methodology as the previous sphere example. For DPGP-IRLS we use the Karcher mean~\cite{karcher1977riemannian}.

% The results of this PSD example are in~\cref{tab:psd_ex1}. Again, outlier detection is improved by our manifold-aware DPCP-IRLS (called DPGP-IRLS). Also, notice there is a much smaller variance in the correlation with the inliers for DPGP-IRLS.

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{c|cc}
%                  & Inliers       & Outliers \\
%                  \hline
%         DPGP-IRLS     & $ 0.0249 \pm 0.0041 $ & $ 0.4879 \pm 0.0302$\\
%         DPCP-IRLS     & $ 0.0355 \pm 0.0150 $ & $ 0.5077 \pm 0.0290 $
%     \end{tabular}
%     \caption{$1000$ inliers and $100$ outliers on the manifold of rank-$1$ $10$-dimensional PSD matrices. The inliers live on a geodesic submanifold spanned by $8$ tangent vectors and the outliers are randomly sampled. Entries are mean absolute correlations between the first $2$ dual PCs and the data.}
%     \label{tab:psd_ex1}
% \end{table}


\paragraph{DPCP-IRLS: Euclidean vs Manifold}
Compare inlier correlation/ outlier correlation for sphere, PSD matrices, and rotations.

\paragraph{Compare all Methods}
Compare plots of first two PCs for a dataset of two clusters with all 4 methods. Get first 2 PCs by looking at orthogonal complement of the last $n-1$ PCs for DPCP-IRLS.

Or compare correlations with inliers and outliers for principle directions for each of the methods.

\paragraph{Robustness of Flag Versions}
Gradually add outliers and compare vanilla (Stiefel) algorithms to flag versions.

\paragraph{Online Principle Directions}
Take a dataset that can be seperated into two subsets of samples. Samples until time $t$ and samples from time $t+1$ to $T$. Then run each of the four algorithms: PCA, PGA, DPCP-IRLS, DPGP-IRLS with Stiefel and flagified versions on each of the two datasets. Use flag averaging to get estimation of PCs for the whole dataset. For example \url{http://proceedings.mlr.press/v33/goes14.pdf}.


\subsection{Real Data}
\paragraph{Anomaly Detection}
Do anomaly detection on satellite images with $n$ spectral bands and $p$ pixels. We some (or just one) of the images from~\cite{padron2021unsupervised}. Each pixel $\x^{(l)} \in \R^n$ is a data point. Generate $\X^{(l)} = \x^{(l)} {\x^{(l)}}^T$ as SPD matrix. Do dual PGA on $\{\X^{(l)} \}_{l=1}^p$ to find outlier pixels. This was done for one image from Padron~\etal. DPCP-IRLS does a poor job at detecting the outlier pixels and the manifold method does not significantly improve those results.

\nate{I tried this with PCA vs flagified pca and saw simila, poor results. I also tried change detection. But saw even worse results.}

\begin{figure}[H]
    \centering
    \includegraphics[width =\linewidth]{figures/AD_Example.pdf}
    \caption{Anomaly detection using Flagified PCA and PCA. AUC for $5$ components is $0.70$ and $0.72$ respectively. AUC for $25$ components is $0.76$ and $0.75$ respectively.\tolga{maybe show many images?}}
    \label{fig:AD}
\end{figure}
%We can also generate a kernel SPD matrix by doing $\X^{(l)}_{i,j} = e^{|x^{(l)}_i-x^{(l)}_j|^2/\sigma}$ or another kernel. This doesnt work because the matrix is not guaranteed to be positive definite.


\paragraph{Online Principle Directions}
Suppose we have too many data points (samples) so we can't store the matrix in memory. Or, suppose we have a big timeseries dataset. Then we do something like we did in the ICCV submission. Averaging flags of principal components, dual principal components, principal tangent vectors, and dual principal tangent vectors but with a ``non-trivial'' flag type like (1,3,10). %\nate{I'm not sure what we're looking to find here... but maybe there a good reason to do this? Maybe we work with a spatial, temporal, or spatio-temporal dataset with many, many samples.}


\paragraph{Classification}
Classification by nearest geodesic subspace. Or using variants of principal directions for classification. \nate{Ideas for datasets here?}

\paragraph{Occlusion Data and More!}
\tolga{we need a lot of ideas here. my gut tells me that we should first demonstrate (even synthetically) the effect of our principal directions on existing manifold datasets. so weather data is probably one. but also 'rotations' can be interesting too - rotation clustering? for example we use a Principal Component Analysis (PCA) on the quaternion hypotheses in this paper: ~\cite{manhardt2019explaining}. Though, we should definitely start from datasets used in PGA and DualPCA.}  \\
\nate{In response to~\cite{manhardt2019explaining}: \\ -How are you thinking of doing rotation clustering here?\\ -My idea: We could use Tangent/linearized PGA instead of PCA in Algorithm 1 of the Supplementary. For this, we need to come up with a new thresholding that controls the inner if statement. Then we compare performance between algorithms. \\ -Another thought is to use Dual PCA and Dual PGA for a similar task of controlling the if statement. But, in this case, we would need to think of another analogous if statement for these dimensionality reduction algorithms. \\ -I'm just spitballing here... I like the idea of using these data... do you have any other specific thoughts about what we can do with it???}


\paragraph{Spectral Clustering}
Try spectral clustering with the top vectors from out versions of PCA. I'm not sure which datasets make the most sense here...



\begin{comment}
Suppose we have two sets of basis vectors in either $\R^n$ or $T_{\mu}(\Man)$: $\{\bu_i\}_{i=1}^k$ and $\{\bv_i\}_{i=1}^k$ . Let $\theta ( \bu_i, \bv_i)$ denote the smallest angle between $\bu_i$ and $\bv_i$. We compare the angles between the basis vectors using the mean angle
\begin{equation}
    \Delta T = \frac{1}{k}\sum_{i=1}^k \theta ( \bu_i, \bv_i).
\end{equation}

We have three ways to compare a baseline embedding of data $\widehat{\X}_b = \U_b^T \X$ and another embedding $\widehat{\X} = \U^T \X$.

Compute the Euclidean distance matrix under $\| \cdot \|_2$ of the embedded data sets as $\mathbf{D}_b$ and $\mathbf{D}$ respectively.
\begin{equation}
    \Delta D = \frac{\|\mathbf{D}_b - \mathbf{D}\|_F}{\|\mathbf{D}_b\|_F}.
\end{equation}

We compare the angles between the basis vectors using
\begin{align}
\begin{aligned}
    \Delta T &= \sqrt{\sum_{i=1}^k \theta ( {\U_b}_i, {\U}_i)^2},\\
             &= \sqrt{ \sum_{i=1}^k \arccos^2 \left( |{\U_b}_i^T {\U}_i |  \right)}.
\end{aligned}
\end{align}
\nate{sum absolute values of angles. also careful with what we're summing over.}

Finally, we compare the explained variances using
\begin{equation}
    \Delta V = \left|\frac{\|\U_b^T \X\|_F^2 - \|\U^T \X\|_F^2}{\|\U_b^T \X\|_F^2}\right|.
\end{equation}
\end{comment}


\begin{comment}
We use $20$ datasets sampled with $30$ points in the same clusters as described above. For each dataset we sample $15$ points in Cluster 1, $5$ in Cluster $2$, and $10$ in Cluster 3. We run flagified versions of PCA optimized over $\flag(2,5,9;10)$ on each dataset with a maximum of $100$ iterations. We check the resulting principal directions by checking the objective function values of $20$ randomly sampled points near them. Given a set of principal directions in $\U \in \R^{9 \times 10}$ we sample a checking point as the first $9$ columns of $\mathbf{Q}$ from the $QR$ decomposition of $\U + \Delta$ where $\Delta \sim \mathcal{U}[0,0.01)$. We find that fRPCA and fWPCA always converge whereas fDPCP converges for $80\%$ trials. The means and standard deviations of the run times are in~\cref{tab:fPCAvarTimes}.

\begin{table}[h]
    \centering
    \begin{tabular}{c|c}
        Algorithm & Run Time (sec) \\
        \hline
        fRPCA & $20.17\pm9.24$\\
        fWPCA & $33.57 \pm 27.08$\\
        fDPCP & $467.03\pm271.28$
    \end{tabular}
    \caption{Run times of flagified PCA variants optimized over $\flag(2,5,9;10)$. \nate{ I need to re-run this and cite the machine that I'm running it on... this probably goes in supplementary material}}
    \label{tab:fPCAvarTimes}
\end{table}

We preform vanilla PCA and compare it to fRPCA($2,5,9$) and fWPCA($2,5,9$). Optimizing over $\flag(2,5,9,10)$ results in high variance in cluster $3$ (green points) when we look at the $8$th and $9$th principal components. The results for fRPCA and fWPCA are in~\cref{fig: fRPCAvfWPCAvPCA} respectively.
\begin{figure}[t]
    \centering
    \includegraphics[width =\linewidth]{figures/ScatterPCAs.pdf}
    \caption{fRPCA($2,5,9$) and fWPCA($2,5,9$)(right) places higher variance in C$3$ for the $8$th and $9$th PCs. \nate{Remove this. do quantitiative evaluation.}}
    \label{fig: fRPCAvPCA}
\end{figure}
\end{comment}


\subsection{Hand Data}
We represent the $40$ hands on $SO(2)^{56}$ as relative rotations about the positive $x$-axis. We run our PCA variants to produce compressed representations of the shapes. We report the reconstruction error of our algorithms in 



%max iterations for gradient descent is 1000
% \begin{itemize}
%  \item \url{https://github.com/msrepo/statistical_shape_model}
%  \item \url{https://github.com/DrewLazar/RobustManifold/tree/master/HandShape/RawData}
%  \item \url{https://link.springer.com/chapter/10.1007/978-3-540-76725-1_35}
% \end{itemize}
We preform Procrustes alignment on the hands dataset (from \url{https://github.com/msrepo/statistical_shape_model}) with $40$ hands. Then we generate a dataset with these aligned hands and $10$ different outlier ellipses and we normalize each data point to obtain a dataset on $S^{111}$. We run t-PGA variations on (1) only the hands and (2) the whole dataset (including outliers). Then we compare various dimensionality reduction schemes in~\cref{tab:hand_res}.
\begin{table}
\centering
\begin{tabular}{c@{\:}c@{\:}c@{\:}l@{\:}|ccc}
\toprule
& & &  Algorithm & $\Delta D$ & $\Delta T$ & $\Delta V$\\
\midrule
\multirow{10}{*}{\rotatebox{90}{Primal}} & \multirow{5}{*}{\rotatebox{90}{Euc.}} & \multirow{3}{*}{\rotatebox{90}{Var.}}& PCA & 0.0456 & 1.5414 & \textbf{3.3944} \\
& & & fRPCA(5) & 0.0452 & 1.5321 & 3.4019\\
& & & fRPCA(1,...,5) & 0.0502 & 1.4875 & 3.4052\\
& & \multirow{2}{*}{\rotatebox{90}{Rec.}} & fWPCA(5) & 0.0470 & 1.5150 & 3.3957\\
& & & fWPCA(1,...,5) & 0.0461 & 1.3845 & 3.4026 \\
\cline{4-7}
 & \multirow{5}{*}{\rotatebox{90}{Man.}} & \multirow{3}{*}{\rotatebox{90}{Var.}}& t-PCA & 0.0453 & 1.5420 & 3.4019 \\
& & & t-fRPCA(5) & \textbf{0.0442} & 1.5673 & 3.4248\\
& & & t-fRPCA(1,...,5) & 0.0690 & \textbf{1.0056} & 3.4252\\
& & \multirow{2}{*}{\rotatebox{90}{Rec.}}& t-fWPCA(5) & 0.0459 & 1.5340 & 3.4184\\
& & & t-fWPCA(1,...,5) & \textbf{0.0442} & 1.3960 & 3.4331\\
\hline
\hline
\multirow{4}{*}{\rotatebox{90}{Dual}}& \multirow{2}{*}{\rotatebox{90}{Euc.}} & \multirow{4}{*}{\rotatebox{90}{Var.}} & fDPCP(5) & 0.4244 & 0.5667 & \textbf{0.0484}\\
& & & fDPCP(1,...,5) & 0.4244 & 0.5667 & \textbf{0.0484}\\
\cline{4-7}
& \multirow{2}{*}{\rotatebox{90}{Man.}} & & t-fDPCP(5) & 0.5515 & 0.2358 & 0.7570\\
& & & t-fDPCP(1,...,5) & \textbf{0.3541} & \textbf{0.1247} & 0.6143\\
\bottomrule
\end{tabular}
\caption{Hand Results}
\label{tab:hand_res}
\end{table}

\begin{table}[H]
\centering
\begin{tabular}{c@{\:}c@{\:}c@{\:}l@{\:}|ccc}
\toprule
& & &  Algorithm & $D$ & $T$ & $V$\\
\midrule
\multirow{10}{*}{\rotatebox{90}{Primal}} & \multirow{5}{*}{\rotatebox{90}{Euc.}} & \multirow{3}{*}{\rotatebox{90}{Var.}} & PCA & 0.0454 & 1.5525 & 3.6406 \\
& & & fWPCA(5) & 0.0461 & 1.5119 & 3.6429 \\
& & & fWPCA(1,...,5) & 0.0460 & 1.3840 & 3.6505 \\
& & \multirow{2}{*}{\rotatebox{90}{Rec.}} & fRPCA(5) & 0.0449 & 1.5378 & 3.6496 \\
& & & fRPCA(1,...,5) & 0.1088 & 1.5600 & \textbf{3.6070} \\
\cline{4-7}
 & \multirow{5}{*}{\rotatebox{90}{Man.}} & \multirow{3}{*}{\rotatebox{90}{Var.}} & t-PCA & 0.0451 & 1.5530 & 3.6483 \\
& & & t-fWPCA(5) & 0.0462 & 1.4981 & 3.6671 \\
& & & t-fWPCA(1,...,5) & 0.0451 & 1.2852 & 3.6758 \\
& & \multirow{2}{*}{\rotatebox{90}{Rec.}} & t-fRPCA(5) & \textbf{0.0439} & 1.5685 & 3.6752 \\
& & & t-fRPCA(1,...,5) & 0.1197 & \textbf{1.1027} & 3.6382 \\
\hline
\hline
\multirow{4}{*}{\rotatebox{90}{Dual}}& \multirow{2}{*}{\rotatebox{90}{Euc.}} & \multirow{4}{*}{\rotatebox{90}{Var.}} & fDPCP(5) & 0.4872 & 0.5345 & \textbf{0.2311} \\
& & & fDPCP(1,...,5) & 0.4872 & 0.5345 & \textbf{0.2311} \\
\cline{4-7}
& \multirow{2}{*}{\rotatebox{90}{Man.}} & & t-fDPCP(5) & \textbf{0.3968} & 0.1657 & 0.5545 \\
& & & t-fDPCP(1,...,5) & 0.4756 & \textbf{0.1500} & 0.7140 \\
\bottomrule
\end{tabular}
\caption{Hand Results}
\label{tab:hand_res}
\end{table}




\subsection{Indian Pines}
%max iterations for gradient descent is 1000
These data are represented as rank $20$ symmetric positive definite matrices using the algorithm from~\cite{fang2018new}. We generate a dataset with $80$ examples of crop type $3$ and $20$ examples of crop type $4$. We run t-PGA variations on (1) only class $3$ data and (2) the whole dataset. Then we compare various dimensionality reduction schemes in~\cref{tab:ip_res}

\begin{table}
\centering
\begin{tabular}{c@{\:}c@{\:}c@{\:}l@{\:}|ccc}
\toprule
& & &  Algorithm & $D$ & $T$ & $ V$\\
\midrule
\multirow{10}{*}{\rotatebox{90}{Primal}} & \multirow{5}{*}{\rotatebox{90}{Euc.}} & \multirow{3}{*}{\rotatebox{90}{Var.}}& PCA & 0.0589 & 1.1895 & 0.0067 \\
& & & fRPCA(3) & 0.0595 & 0.4214 & 0.0061\\
& & & fRPCA(1,2,3) & 0.1376 & 0.9473 & 0.0148 \\
& & \multirow{2}{*}{\rotatebox{90}{Rec.}} & fWPCA(3) & 0.0763 & 0.4034 & 0.0040\\
& & & fWPCA(1,2,3) & 0.0752 & 0.2821 & \textbf{0.0022} \\
\cline{4-7}
 & \multirow{5}{*}{\rotatebox{90}{Man.}} & \multirow{3}{*}{\rotatebox{90}{Var.}}& t-PCA & \textbf{0.0579} & 1.1626 & 0.0071 \\
& & & t-fRPCA(3) & 0.0590 & 1.0505 & 0.0062\\
& & & t-fRPCA(1,2,3) & 0.1082 & 1.4823 & 0.0309 \\
& & \multirow{2}{*}{\rotatebox{90}{Rec.}}& t-fWPCA(3) & 0.0769 & 0.9770 & 0.0046\\
& & & t-fWPCA(1,2,3) & 0.0742 & \textbf{0.0566} & 0.0026 \\
\hline
\hline
\multirow{4}{*}{\rotatebox{90}{Dual}}& \multirow{2}{*}{\rotatebox{90}{Euc.}} & \multirow{4}{*}{\rotatebox{90}{Var.}} & fDPCP(3) & 0.7121 & 0.2474 & 0.8906\\
& & & fDPCP(1,2,3) & \textbf{0.2280} & \textbf{0.0627} & \textbf{0.2870} \\
\cline{4-7}
& \multirow{2}{*}{\rotatebox{90}{Man.}} & & t-fDPCP(3) & 0.6827 & 0.2228 & 0.8453\\
& & & t-fDPCP(1,2,3) & 0.9075 & 0.1851 & 1.8928 \\

\bottomrule
\end{tabular}
\caption{Indian Pines Results}
\label{tab:ip_res}
\end{table}

==> content/relatedwork.tex <==
\section{Related Work}\label{sec:related}

% \paragraph{Averaging in computer vision}

\paragraph{PCA and Dual PCA}
Although there are many variants of Principal Component Analysis (PCA)~\cite{hotelling1933analysis, scholkopf1997kernel, vidal2005generalized, candes2011robust, arenas2013kernel}, we focus on forms of Robust PCA (RPCA)~\cite{kwak2008principal, markopoulos2014optimal, neumayer2020robust} and Dual PCA (DPCA)~\cite{vidal2018dpcp}. Given a dataset in $\R^n$, RPCA seeks to find the directions that maximize explained variance. DPCA, on the other hand, is a more robust dimensionality reduction algorithm which is designed to work on datasets with outliers by minimizing a $0$-norm problem~\footnote{Kernelized PCA~\cite{scholkopf1997kernel} is sometimes refered to as Dual PCA but we will refer to Dual PCA as the outlier robust dimensionality reduction suggested by Vidal~\etal.}. 

%It finds directions orthogonal to the subspace that contains most of the inliers of the dataset. 

%Dual PCA, on the other hand, operates on the paradigm that our dataset contains many inliers and few outliers by finding directions orthogonal to the subspace that contains most of the inliers of the dataset. This essentially addresses the opposite problem of PCA by minimizing functions of the explained variance. 


\paragraph{PCA on manifolds} Principal Curves~\cite{hastie1989principal} finds curves passing through the mean of a dataset which maximize variance and have seen their own enhancements~\cite{laparra2012nonlinearities}.  Although it it doesn't strictly work on a manifold, it provides a framework for true manifold dimensionality reduction algorithms. Fletcher~\etal was one of the first to generalize PCA to Riemannian manifolds using Principal Geodesic Analysis (PGA), which finds geodesic submanifolds that best represent the data~\cite{fletcher2004principal}. They adapt ideas from Principal Curves by approximating PGA with lineralized (a.k.a. tangent) PGA which performs PCA on the tangent space to the mean of the data. Linearized principal geodesic analysis has been applied to the manifold of SPD matrices on ``real-world'' datasets~\cite{harandi2014manifold, smith2022data}. Variants of PCA, like RPCA and kPCA, have seen adaptations to manifolds using linearized PGA~\cite{abboud2020robust, awate2014kernel}. Exact PGA better approximates the PGA optimization problem without the tangent space approximation~\cite{sommer2010manifold, sommer2014optimization}. Another formulation of PCA on manifolds that removes the mean requirement is Geodesic PCA (GPCA) \cite{huckemann2006principal, huckemann2010intrinsic}. PCA was also generalized to spheres and shape spaces with principal nested spheres~\cite{jung2012analysis} and principal nested shape spaces~\cite{dryden2019principal} respectively. A kernal version of principal nested spheres have also been considered~\cite{awate2016robust}. Barycentric Subspace Analysis (BSA) realizes PCA on more classes of manifolds than just Riemannian manifolds by generalizing geodesic subspaces using weighted means of reference points~\cite{pennec2018barycentric}. Although flags and PCA have been linked previously, Pennec uses flags throughout his discussion to describe nested subspace relations. 
\tolga{Mention Tabaghi~\cite{tabaghi2023principal}, nested spheres and hyperboloids~\cite{fan2022nested}}

In recent years, Pennec has continued investigating generalizations PCA while using flags~\cite{pennec2020advances}. Buet~\etal generalized varifolds to flagifolds to understand the eigenvalues (explained variances) from PCA along with the flag structure of the principal components in order to model multi-dimensional shapes~\cite{buet2023flagfolds}. Rabenoro~\etal offered a method for hypothesis testing and confidence regions for PCA, all within the context of flag manifolds \cite{rabenoro2022geometric}.

\paragraph{Flag manifolds}
Besides being mathematically interesting objects~\cite{wiggerman1998fundamental,donagi2008glsms,alekseevsky1997flag}, flags and flag manifolds have been explored by a series of works from Nishimori~\etal addressing subspace independent component analysis (ICA) via Riemannian optimization~\cite{nishimori2006riemannian0, nishimori2006riemannian1, nishimori2007flag, nishimori2008natural,nishimori2007flag,nishimori2006riemannian}. A number of works have also addressed averaging on flag manifolds or producing flags as subspace averages~\cite{draper2014flag,Mankovich_2023_ICCV,mankovich2023subspace}. Nested sequences of subspaces (e.g. flags) appear in 
%canonical algorithms like 
the weights in principal component analysis (PCA), the numerous manifold variants of PCA \cite{pennec2018barycentric,pennec2020advances,ye2022optimization} and the result of a wavelet transform \cite{kirby2001geometric}.




% \nate{mention DU NGUYEN here...}


% \paragraph{Flag manifolds in computer vision} The utilization of flag manifolds in computer vision is a recent development. Ma~\etal~\cite{ma2021flag} employ nested subspace methods to compare large datasets. Additionally, they port self-organizing mappings to work on flag manifolds, enabling parameterization of a set of flags of a fixed type. This method was applied to hyper-spectral image data analysis~\cite{ma2022self}. Ye~\etal~\cite{ye2022optimization} derive closed-form analytic expressions for the set of operators required for Riemannian optimization algorithms on the flag manifold, while Nguyen~\cite{nguyen2022closed, nguyen2023operator} provides an alternative framework for Riemannian optimization on flag manifolds. Szwagier~\etal offer a re-framing of the logarithm map on the flag manifold as a Procrustes problem between orthogonal matrices while simultaneously offering an efficient method for computing geodesics, and consequently distance \cite{szwagier2023rethinking}.


% Marrinan~\etal~\cite{marrinan2014finding} investigate the averaging of Grassmanians into flags, demonstrating that flag means behave more like medians and are therefore more robust to the presence of outliers among the subspaces being averaged. Building on this work, they utilize flag averages to improve the detection of chemical plumes in hyperspectral videos~\cite{marrinan2016flag}. Finally, Mankovich~\etal~\cite{mankovich2022flag} also average Grassmannians into flags by providing the median as a flag and an algorithm to compute it. 
%\tolga{Have a look :)}

% \paragraph{Why PCA?}
% Use conclusion of \cite{pennec2018barycentric}. 

% \paragraph{Other}

%Finally, Mankovich~\etal~\cite{mankovich2022flag} provide a robust algorithm for median computations.

% The use of flag manifolds~\cite{monk1959geometry} in computer vision is only recent. Ma~\etal~\cite{ma2021flag} use nested subspace methods, utilizing flag manifolds to compare large sets of data. Same authors also ported self-organizing mappings to work on flag manifolds in order to parameterize a set of flags of a fixed type~\cite{ma2022self}. Their method was applied to hyper-spectral image data analysis. Ye~\etal~\cite{ye2022optimization} derive closed-form analytic expressions for the set of operators required for Riemannian optimization algorithms on the flag manifold. Nguyen~\cite{nguyen2022closed} provided closed-form expressions for logarithms and geodesics on flag manifolds.
% Marrinan~\etal~\cite{marrinan2014finding} investigate averaging Grassmanians into flags and find out that flag means behave more like medians and are therefore more robust to the presence of outliers among the subspaces being averaged. 
% Marrinan~\etal~\cite{marrinan2016flag} use flag averages to improve detection of chemical plumes in hyperspectral videos.
% Mankovich~\etal~\cite{mankovich2022flag} provided robustified algorithms for centroid computations. 

==> preamble.tex <==

\usepackage{iccv}
\usepackage{times}
\usepackage{epsfig}
\usepackage[utf8]{inputenc}
\usepackage{color}
\usepackage{bm}
\usepackage{amsfonts,mathtools,amsmath,amsthm}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{mwe}
\usepackage{makecell}
\usepackage{booktabs}
\usepackage{enumitem}
\usepackage{float} %Nate added this
\usepackage{graphicx} %Nate added this
\graphicspath{{images/}} %Nate added this
\usepackage[ruled,vlined]{algorithm2e} %Nate added this
\usepackage[pagebackref=true,breaklinks=true,colorlinks,bookmarks=false]{hyperref}
\usepackage{setspace}
\usepackage[table]{xcolor}
\usepackage{comment}
% \usepackage{todonotes}
\usepackage[capitalize]{cleveref}
\providecommand\algorithmname{algorithm}
% \usepackage[thmmarks, amsmath, thref, amsthm]{ntheorem}

\def\iccvPaperID{3293} % *** Enter the ICCV Paper ID here
\def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}

% Pages are numbered in submission mode, and unnumbered in camera-ready
\ificcvfinal\pagestyle{empty}\fi

\title{Fun with Flags: Robust Principal Directions via Flag Manifolds -- Author Feedback}
\usepackage[dvipsnames]{xcolor}
\usepackage{enumitem}

%\newcommand{\Rone}{{\textcolor{Blue}{\textbf{R1}}}}
%\newcommand{\Rtwo}{{\textcolor{RoyalBlue}{\textbf{R2}}}}
%\newcommand{\Rthree}{{\textcolor{TealBlue}{\textbf{R3}}}}
\newcommand{\Rone}[0]{\textcolor{teal}{\textbf{sJxc}}}
\newcommand{\Rtwo}[0]{\textcolor{cyan}{\textbf{ZkmG}}}
\newcommand{\Rthree}[0]{\textcolor{magenta}{\textbf{3dqZ}}}


\input{defs.tex}
\renewcommand{\paragraph}[1]{{\vspace{0.5mm}\noindent \bf #1}.}
\newcommand{\parahead}[1]{\vspace{0.5mm}\noindent\textbf{#1}.\ }

==> preamble_rebuttal.tex <==

\usepackage{cvpr}
\usepackage{times}
\usepackage{epsfig}
\usepackage[utf8]{inputenc}
\usepackage{color}
\usepackage{bm}
\usepackage{amsfonts,mathtools,amsmath, amsthm}
\usepackage{graphicx}
%\usepackage{subcaption}
\usepackage{mwe}
\usepackage{makecell}
\usepackage{booktabs}
\usepackage{enumitem}
\usepackage{float} %Nate added this
\usepackage{graphicx} %Nate added this
\graphicspath{{images/}} %Nate added this

\usepackage[ruled,vlined]{algorithm2e} %Nate added this

\definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
\usepackage[pagebackref,breaklinks,colorlinks,citecolor=cvprblue]{hyperref}

\usepackage{color}
\usepackage{xcolor}
\usepackage{flushend}
\usepackage{setspace}
% \usepackage[table]{xcolor}
%\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{comment}
% \usepackage{todonotes}
\usepackage[capitalize]{cleveref}
\usepackage{multirow}
\providecommand\algorithmname{algorithm}
% \usepackage[thmmarks, amsmath, thref, amsthm]{ntheorem}

%\iccvfinalcopy
\def\paperID{824} % *** Enter the Paper ID here
\def\confName{CVPR}
\def\confYear{2024}

% \def\iccvPaperID{824} % *** Enter the ICCV Paper ID here
\def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}

%%%%%%%%% TITLE
\title{Fun with Flags: Robust Principal Directions via Flag Manifolds}

\renewcommand{\paragraph}[1]{{\vspace{0.5mm}\noindent \bf #1}.}
\newcommand{\paragraphnoper}[1]{{\vspace{0.5mm}\noindent \bf #1}}

\newcommand{\Rone}[0]{\textcolor{teal}{\textbf{sJxc}}}
\newcommand{\Rtwo}[0]{\textcolor{cyan}{\textbf{ZkmG}}}
\newcommand{\Rthree}[0]{\textcolor{magenta}{\textbf{3dqZ}}}

\newcommand{\PCA}{PCA}
\newcommand{\RPCA}{RPCA}
\newcommand{\WPCA}{WPCA}
\newcommand{\DPCP}{DPCP}
\newcommand{\WDPCP}{WDPCP}
\newcommand{\LtwoRPCA}{$L_2$-RPCA}
\newcommand{\LoneRPCA}{$L_1$-RPCA}
\newcommand{\LpRPCA}{$L_p$-RPCA}
\newcommand{\LtwoWPCA}{$L_2$-WPCA}
\newcommand{\LoneWPCA}{$L_1$-WPCA}
\newcommand{\OPCA}{$\perp$PCA}
\newcommand{\LtwoDPCP}{$L_2$-DPCP}
\newcommand{\LtwoWDPCP}{$L_2$-WDPCP}
\newcommand{\LoneDPCP}{$L_1$-DPCP}
\newcommand{\LoneWDPCP}{$L_1$-WDPCP}
\newcommand{\fPCA}{fPCA}
\newcommand{\fOPCA}{f$\perp$PCA}
\newcommand{\fRPCA}{fRPCA}
\newcommand{\fWPCA}{fWPCA}
\newcommand{\fDPCP}{fDPCP}
\newcommand{\fWDPCP}{fWDPCP}
\newcommand{\ftwoRPCA}{fRPCA$(k)$}
\newcommand{\ftwoWPCA}{fWPCA$(k)$}
\newcommand{\ftwoDPCP}{fDPCP$(k)$}
\newcommand{\foneRPCA}{fRPCA$(1,...,k)$}
\newcommand{\foneWPCA}{fWPCA$(1,...,k)$}
\newcommand{\foneDPCP}{fDPCP$(1,...,k)$}
